UMI-Live for In-The-Wild Bimanual Robotics Data Collection

Universal Manipulation Interface (UMI) devices allow human experts to demonstrate tasks for robot learning without teleoperating physical robots. Using these demonstrations as training data still requires a consistent hardware setup, calibration, and data processing. We present UMI-Live, a full-stack open-source bimanual UMI system for in-the-wild data collection. We design our custom UMI-Live hardware to integrate camera and LiDAR--inertial sensing, onboard compute, and power, without external tracking equipment or calibration within the collection environment. We implement a simple user interface for recording data while an asynchronous pipeline performs parallel SLAM reconstruction and publishes training-ready datasets. We also release software that supports dual-YAM teleoperation and VLA policy training and inference. We validate UMI-Live data quality by fine-tuning $\pi_{0.5}$ and MolmoAct2, achieving success rates of 10/10 and 8/10, respectively on a bimanual pick-and-place task. Furthermore, we release 40 hours of UMI-Live data across three tasks, and complete hardware designs, software, and reproduction guides at our $\href{https://umi-live.github.io/}{\text{project website}}$.

==> figures/pipeline/pipeline-geometry.tex <==
%% Native TikZ geometry transcribed from the supplied PDF.
% Reference curve 0
\path[fill=pipelineteal!5,draw=pipelineborder,line width=.48bp,
  rounded corners=3.2bp]
  (.4,.4) rectangle (395.6,103.6);
% Reference curve 1
\path[draw={rgb,1:red,0.78432;green,0.78432;blue,0.76471},line width=0.34870bp] (6.00000,18.20301)
  -- (6.00000,58.56306)
  .. controls (6.00000,59.22581) and (6.53725,59.76307) .. (7.20000,59.76307)
  -- (80.80011,59.76307)
  .. controls (81.46284,59.76307) and (82.00010,59.22581) .. (82.00010,58.56306)
  -- (82.00010,18.20301)
  .. controls (82.00010,17.54026) and (81.46284,17.00302) .. (80.80011,17.00302)
  -- (7.20000,17.00302)
  .. controls (6.53725,17.00302) and (6.00000,17.54026) .. (6.00000,18.20301)
  -- cycle;
% Reference curve 2
\path[fill={rgb,1:red,0.13725;green,0.62354;blue,0.65099}] (31.63004,42.81301)
  -- (27.83000,42.81301)
  .. controls (27.22247,42.81301) and (26.72998,43.30550) .. (26.72998,43.91302)
  -- (26.72998,47.71307)
  .. controls (26.72998,48.32058) and (27.22247,48.81307) .. (27.83000,48.81307)
  -- (31.63004,48.81307)
  .. controls (32.23755,48.81307) and (32.73006,48.32058) .. (32.73006,47.71307)
  -- (32.73006,43.91302)
  .. controls (32.73006,43.30550) and (32.23755,42.81301) .. (31.63004,42.81301)
  -- cycle;
% Reference curve 3
\path[fill={rgb,1:red,0.89804;green,0.50195;blue,0.27843}] (63.34009,44.80302)
  -- (59.54004,44.80302)
  .. controls (58.93253,44.80302) and (58.44003,45.29553) .. (58.44003,45.90304)
  -- (58.44003,49.70307)
  .. controls (58.44003,50.31060) and (58.93253,50.80310) .. (59.54004,50.80310)
  -- (63.34009,50.80310)
  .. controls (63.94760,50.80310) and (64.44010,50.31060) .. (64.44010,49.70307)
  -- (64.44010,45.90304)
  .. controls (64.44010,45.29553) and (63.94760,44.80302) .. (63.34009,44.80302)
  -- cycle;
% Reference curve 4
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (106.00014,22.90302)
  -- (106.00014,42.10305)
  .. controls (106.00014,42.60010) and (106.40308,43.00305) .. (106.90013,43.00305)
  -- (136.60016,43.00305)
  .. controls (137.09723,43.00305) and (137.50017,42.60010) .. (137.50017,42.10305)
  -- (137.50017,22.90302)
  .. controls (137.50017,22.40597) and (137.09723,22.00302) .. (136.60016,22.00302)
  -- (106.90013,22.00302)
  .. controls (106.40308,22.00302) and (106.00014,22.40597) .. (106.00014,22.90302)
  -- cycle;
% Reference curve 5
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (106.00014,45.90305)
  -- (106.00014,65.10308)
  .. controls (106.00014,65.60014) and (106.40308,66.00308) .. (106.90013,66.00308)
  -- (136.60016,66.00308)
  .. controls (137.09723,66.00308) and (137.50017,65.60014) .. (137.50017,65.10308)
  -- (137.50017,45.90305)
  .. controls (137.50017,45.40600) and (137.09723,45.00305) .. (136.60016,45.00305)
  -- (106.90013,45.00305)
  .. controls (106.40308,45.00305) and (106.00014,45.40600) .. (106.00014,45.90305)
  -- cycle;
% Reference curve 6
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (139.50017,22.90302)
  -- (139.50017,42.10305)
  .. controls (139.50017,42.60010) and (139.90312,43.00305) .. (140.40018,43.00305)
  -- (170.10020,43.00305)
  .. controls (170.59726,43.00305) and (171.00021,42.60010) .. (171.00021,42.10305)
  -- (171.00021,22.90302)
  .. controls (171.00021,22.40597) and (170.59726,22.00302) .. (170.10020,22.00302)
  -- (140.40018,22.00302)
  .. controls (139.90312,22.00302) and (139.50017,22.40597) .. (139.50017,22.90302)
  -- cycle;
% Reference curve 7
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (139.50017,45.90305)
  -- (139.50017,65.10308)
  .. controls (139.50017,65.60014) and (139.90312,66.00308) .. (140.40018,66.00308)
  -- (170.10020,66.00308)
  .. controls (170.59726,66.00308) and (171.00021,65.60014) .. (171.00021,65.10308)
  -- (171.00021,45.90305)
  .. controls (171.00021,45.40600) and (170.59726,45.00305) .. (170.10020,45.00305)
  -- (140.40018,45.00305)
  .. controls (139.90312,45.00305) and (139.50017,45.40600) .. (139.50017,45.90305)
  -- cycle;
% Reference curve 8
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (179.00023,22.90302)
  -- (179.00023,42.10305)
  .. controls (179.00023,42.60010) and (179.40318,43.00305) .. (179.90024,43.00305)
  -- (209.60027,43.00305)
  .. controls (210.09732,43.00305) and (210.50026,42.60010) .. (210.50026,42.10305)
  -- (210.50026,22.90302)
  .. controls (210.50026,22.40597) and (210.09732,22.00302) .. (209.60027,22.00302)
  -- (179.90024,22.00302)
  .. controls (179.40318,22.00302) and (179.00023,22.40597) .. (179.00023,22.90302)
  -- cycle;
% Reference curve 9
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (179.00023,45.90305)
  -- (179.00023,65.10308)
  .. controls (179.00023,65.60014) and (179.40318,66.00308) .. (179.90024,66.00308)
  -- (209.60027,66.00308)
  .. controls (210.09732,66.00308) and (210.50026,65.60014) .. (210.50026,65.10308)
  -- (210.50026,45.90305)
  .. controls (210.50026,45.40600) and (210.09732,45.00305) .. (209.60027,45.00305)
  -- (179.90024,45.00305)
  .. controls (179.40318,45.00305) and (179.00023,45.40600) .. (179.00023,45.90305)
  -- cycle;
% Reference curve 10
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (212.50027,22.90302)
  -- (212.50027,42.10305)
  .. controls (212.50027,42.60010) and (212.90321,43.00305) .. (213.40027,43.00305)
  -- (243.10030,43.00305)
  .. controls (243.59737,43.00305) and (244.00030,42.60010) .. (244.00030,42.10305)
  -- (244.00030,22.90302)
  .. controls (244.00030,22.40597) and (243.59737,22.00302) .. (243.10030,22.00302)
  -- (213.40027,22.00302)
  .. controls (212.90321,22.00302) and (212.50027,22.40597) .. (212.50027,22.90302)
  -- cycle;
% Reference curve 11
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (212.50027,45.90305)
  -- (212.50027,65.10308)
  .. controls (212.50027,65.60014) and (212.90321,66.00308) .. (213.40027,66.00308)
  -- (243.10030,66.00308)
  .. controls (243.59737,66.00308) and (244.00030,65.60014) .. (244.00030,65.10308)
  -- (244.00030,45.90305)
  .. controls (244.00030,45.40600) and (243.59737,45.00305) .. (243.10030,45.00305)
  -- (213.40027,45.00305)
  .. controls (212.90321,45.00305) and (212.50027,45.40600) .. (212.50027,45.90305)
  -- cycle;
% Reference curve 12
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (252.00034,22.90302)
  -- (252.00034,42.10305)
  .. controls (252.00034,42.60010) and (252.40327,43.00305) .. (252.90033,43.00305)
  -- (282.60036,43.00305)
  .. controls (283.09743,43.00305) and (283.50037,42.60010) .. (283.50037,42.10305)
  -- (283.50037,22.90302)
  .. controls (283.50037,22.40597) and (283.09743,22.00302) .. (282.60036,22.00302)
  -- (252.90033,22.00302)
  .. controls (252.40327,22.00302) and (252.00034,22.40597) .. (252.00034,22.90302)
  -- cycle;
% Reference curve 13
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (252.00034,45.90305)
  -- (252.00034,65.10308)
  .. controls (252.00034,65.60014) and (252.40327,66.00308) .. (252.90033,66.00308)
  -- (282.60036,66.00308)
  .. controls (283.09743,66.00308) and (283.50037,65.60014) .. (283.50037,65.10308)
  -- (283.50037,45.90305)
  .. controls (283.50037,45.40600) and (283.09743,45.00305) .. (282.60036,45.00305)
  -- (252.90033,45.00305)
  .. controls (252.40327,45.00305) and (252.00034,45.40600) .. (252.00034,45.90305)
  -- cycle;
% Reference curve 14
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (285.50037,22.90302)
  -- (285.50037,42.10305)
  .. controls (285.50037,42.60010) and (285.90330,43.00305) .. (286.40038,43.00305)
  -- (316.10040,43.00305)
  .. controls (316.59746,43.00305) and (317.00040,42.60010) .. (317.00040,42.10305)
  -- (317.00040,22.90302)
  .. controls (317.00040,22.40597) and (316.59746,22.00302) .. (316.10040,22.00302)
  -- (286.40038,22.00302)
  .. controls (285.90330,22.00302) and (285.50037,22.40597) .. (285.50037,22.90302)
  -- cycle;
% Reference curve 15
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (285.50037,45.90305)
  -- (285.50037,65.10308)
  .. controls (285.50037,65.60014) and (285.90330,66.00308) .. (286.40038,66.00308)
  -- (316.10040,66.00308)
  .. controls (316.59746,66.00308) and (317.00040,65.60014) .. (317.00040,65.10308)
  -- (317.00040,45.90305)
  .. controls (317.00040,45.40600) and (316.59746,45.00305) .. (316.10040,45.00305)
  -- (286.40038,45.00305)
  .. controls (285.90330,45.00305) and (285.50037,45.40600) .. (285.50037,45.90305)
  -- cycle;
% Reference curve 16
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (325.00043,22.90302)
  -- (325.00043,42.10305)
  .. controls (325.00043,42.60010) and (325.40337,43.00305) .. (325.90044,43.00305)
  -- (355.60046,43.00305)
  .. controls (356.09752,43.00305) and (356.50046,42.60010) .. (356.50046,42.10305)
  -- (356.50046,22.90302)
  .. controls (356.50046,22.40597) and (356.09752,22.00302) .. (355.60046,22.00302)
  -- (325.90044,22.00302)
  .. controls (325.40337,22.00302) and (325.00043,22.40597) .. (325.00043,22.90302)
  -- cycle;
% Reference curve 17
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (325.00043,45.90305)
  -- (325.00043,65.10308)
  .. controls (325.00043,65.60014) and (325.40337,66.00308) .. (325.90044,66.00308)
  -- (355.60046,66.00308)
  .. controls (356.09752,66.00308) and (356.50046,65.60014) .. (356.50046,65.10308)
  -- (356.50046,45.90305)
  .. controls (356.50046,45.40600) and (356.09752,45.00305) .. (355.60046,45.00305)
  -- (325.90044,45.00305)
  .. controls (325.40337,45.00305) and (325.00043,45.40600) .. (325.00043,45.90305)
  -- cycle;
% Reference curve 18
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (358.50046,22.90302)
  -- (358.50046,42.10305)
  .. controls (358.50046,42.60010) and (358.90341,43.00305) .. (359.40047,43.00305)
  -- (389.10050,43.00305)
  .. controls (389.59755,43.00305) and (390.00050,42.60010) .. (390.00050,42.10305)
  -- (390.00050,22.90302)
  .. controls (390.00050,22.40597) and (389.59755,22.00302) .. (389.10050,22.00302)
  -- (359.40047,22.00302)
  .. controls (358.90341,22.00302) and (358.50046,22.40597) .. (358.50046,22.90302)
  -- cycle;
% Reference curve 19
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (358.50046,45.90305)
  -- (358.50046,65.10308)
  .. controls (358.50046,65.60014) and (358.90341,66.00308) .. (359.40047,66.00308)
  -- (389.10050,66.00308)
  .. controls (389.59755,66.00308) and (390.00050,65.60014) .. (390.00050,65.10308)
  -- (390.00050,45.90305)
  .. controls (390.00050,45.40600) and (389.59755,45.00305) .. (389.10050,45.00305)
  -- (359.40047,45.00305)
  .. controls (358.90341,45.00305) and (358.50046,45.40600) .. (358.50046,45.90305)
  -- cycle;
% Reference curve 26
\path[fill={rgb,1:red,.98431;green,.92549;blue,.95294},
  draw={rgb,1:red,.89804;green,.69804;blue,.78431},
  line width=.48bp,rounded corners=3.2bp]
  (.3,112.3) rectangle (269.7,241.7);
% Reference curve 27
\path[draw=pipelineteal!35,line width=0.34870bp,fill=pipelineteal!12] (41.00005,127.00318)
  -- (41.00005,229.00329)
  .. controls (41.00005,230.10787) and (41.89548,231.00330) .. (43.00006,231.00330)
  -- (262.00034,231.00330)
  .. controls (263.10492,231.00330) and (264.00035,230.10787) .. (264.00035,229.00329)
  -- (264.00035,127.00318)
  .. controls (264.00035,125.89858) and (263.10492,125.00315) .. (262.00034,125.00315)
  -- (43.00006,125.00315)
  .. controls (41.89548,125.00315) and (41.00005,125.89858) .. (41.00005,127.00318)
  -- cycle;
% Reference curve 28
\path[draw=pipelineteal!45,line width=0.34870bp,fill=pipelineteal!6] (38.50003,129.50317)
  -- (38.50003,231.50327)
  .. controls (38.50003,232.60787) and (39.39546,233.50330) .. (40.50006,233.50330)
  -- (259.50032,233.50330)
  .. controls (260.60490,233.50330) and (261.50034,232.60787) .. (261.50034,231.50327)
  -- (261.50034,129.50317)
  .. controls (261.50034,128.39858) and (260.60490,127.50315) .. (259.50032,127.50315)
  -- (40.50006,127.50315)
  .. controls (39.39546,127.50315) and (38.50003,128.39858) .. (38.50003,129.50317)
  -- cycle;
% Reference curve 29
\path[draw=pipelineborder,line width=0.39850bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (36.00005,132.00318)
  -- (36.00005,234.00329)
  .. controls (36.00005,235.10789) and (36.89546,236.00330) .. (38.00006,236.00330)
  -- (257.00032,236.00330)
  .. controls (258.10492,236.00330) and (259.00034,235.10789) .. (259.00034,234.00329)
  -- (259.00034,132.00318)
  .. controls (259.00034,130.89860) and (258.10492,130.00317) .. (257.00032,130.00317)
  -- (38.00006,130.00317)
  .. controls (36.89546,130.00317) and (36.00005,130.89860) .. (36.00005,132.00318)
  -- cycle;
% Reference curve 30
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (41.00005,151.70320)
  -- (41.00005,169.57322)
  .. controls (41.00005,170.07028) and (41.40298,170.47321) .. (41.90005,170.47321)
  -- (69.60008,170.47321)
  .. controls (70.09714,170.47321) and (70.50008,170.07028) .. (70.50008,169.57322)
  -- (70.50008,151.70320)
  .. controls (70.50008,151.20614) and (70.09714,150.80320) .. (69.60008,150.80320)
  -- (41.90005,150.80320)
  .. controls (41.40298,150.80320) and (41.00005,151.20614) .. (41.00005,151.70320)
  -- cycle;
% Reference curve 31
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (73.00009,151.70320)
  -- (73.00009,169.57322)
  .. controls (73.00009,170.07028) and (73.40303,170.47321) .. (73.90009,170.47321)
  -- (101.60011,170.47321)
  .. controls (102.09718,170.47321) and (102.50012,170.07028) .. (102.50012,169.57322)
  -- (102.50012,151.70320)
  .. controls (102.50012,151.20614) and (102.09718,150.80320) .. (101.60011,150.80320)
  -- (73.90009,150.80320)
  .. controls (73.40303,150.80320) and (73.00009,151.20614) .. (73.00009,151.70320)
  -- cycle;
% Reference curve 32
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.54794bp] (107.50012,151.70320)
  -- (107.50012,169.57322)
  .. controls (107.50012,170.07028) and (107.90308,170.47321) .. (108.40013,170.47321)
  -- (136.10016,170.47321)
  .. controls (136.59721,170.47321) and (137.00017,170.07028) .. (137.00017,169.57322)
  -- (137.00017,151.70320)
  .. controls (137.00017,151.20614) and (136.59721,150.80320) .. (136.10016,150.80320)
  -- (108.40013,150.80320)
  .. controls (107.90308,150.80320) and (107.50012,151.20614) .. (107.50012,151.70320)
  -- cycle;
% Reference curve 33
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.54794bp] (139.50017,151.70320)
  -- (139.50017,169.57322)
  .. controls (139.50017,170.07028) and (139.90312,170.47321) .. (140.40018,170.47321)
  -- (168.10020,170.47321)
  .. controls (168.59726,170.47321) and (169.00020,170.07028) .. (169.00020,169.57322)
  -- (169.00020,151.70320)
  .. controls (169.00020,151.20614) and (168.59726,150.80320) .. (168.10020,150.80320)
  -- (140.40018,150.80320)
  .. controls (139.90312,150.80320) and (139.50017,151.20614) .. (139.50017,151.70320)
  -- cycle;
% Reference curve 34
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.39850bp] (41.00005,172.77322)
  -- (41.00005,174.27322)
  -- (102.50012,174.27323)
  -- (102.50012,172.77323);
% Reference curve 35
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.39850bp] (107.50012,172.77322)
  -- (107.50012,174.27322)
  -- (169.00021,174.27323)
  -- (169.00021,172.77323);
% Reference curve 56
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=1.4bp] (6,118.5) rectangle (28,129.5);
% Reference curve 57
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=1.4bp] (6,130.5) rectangle (28,141.5);
% Reference curve 58
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=1.4bp] (6,142.5) rectangle (28,153.5);
% Reference curve 59
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=1.4bp] (6,154.5) rectangle (28,165.5);
% Reference curve 60
\path[draw=pipelineteal,line width=0.59776bp,fill=pipelineteal] (17.00002,115.65981)
  .. controls (17.05904,115.44395) and (17.39356,114.49505) .. (17.75760,113.90200)
  -- (16.24244,113.90200)
  .. controls (16.60648,114.49505) and (16.94100,115.44395) .. (17.00002,115.65981)
  -- cycle;
% Reference curve 61
\path[draw=pipelineteal,line width=0.59776bp,fill=pipelineteal] (33.65671,159.00320)
  .. controls (33.44085,158.94418) and (32.49195,158.60966) .. (31.89890,158.24562)
  -- (31.89890,159.76078)
  .. controls (32.49195,159.39674) and (33.44085,159.06222) .. (33.65671,159.00320)
  -- cycle;
% Reference curve 62
\path[fill=pipelineyellow,draw=pipelinegold,line width=.48bp,
  rounded corners=3.2bp]
  (278.3,112.3) rectangle (395.7,241.7);
% Reference curve 63
\path[draw=pipelineborder,line width=0.39850bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (284.00037,140.00320)
  -- (284.00037,176.00321)
  .. controls (284.00037,177.10780) and (284.89580,178.00323) .. (286.00040,178.00323)
  -- (388.00050,178.00323)
  .. controls (389.10509,178.00323) and (390.00052,177.10780) .. (390.00052,176.00321)
  -- (390.00052,140.00320)
  .. controls (390.00052,138.89860) and (389.10509,138.00318) .. (388.00050,138.00318)
  -- (286.00040,138.00318)
  .. controls (284.89580,138.00318) and (284.00037,138.89860) .. (284.00037,140.00320)
  -- cycle;
% Reference curve 64
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=2bp] (284,188) rectangle (390,203);
% Reference curve 65
\path[draw=pipelineborder,line width=.39850bp,fill=white,
  rounded corners=2bp] (284,209) rectangle (390,238);
% Reference curve 66
\path[draw=pipelineteal,line width=0.49814bp,fill=pipelineteal] (321.95041,185.86011)
  .. controls (322.00458,185.66265) and (322.31160,184.79473) .. (322.64571,184.25228)
  -- (321.25511,184.25228)
  .. controls (321.58922,184.79473) and (321.89624,185.66265) .. (321.95041,185.86011)
  -- cycle;
% Reference curve 67
\path[draw=pipelineteal,line width=0.49814bp,fill=pipelineteal] (377.00050,207.86014)
  .. controls (377.05467,207.66268) and (377.36169,206.79476) .. (377.69580,206.25231)
  -- (376.30520,206.25231)
  .. controls (376.63931,206.79476) and (376.94633,207.66268) .. (377.00050,207.86014)
  -- cycle;
% Reference curve 68
\path[draw=pipelineteal,line width=0.59776bp,fill=pipelineteal] (281.65704,158.00320)
  .. controls (281.44118,157.94418) and (280.49228,157.60966) .. (279.89923,157.24562)
  -- (279.89923,158.76078)
  .. controls (280.49228,158.39674) and (281.44118,158.06222) .. (281.65704,158.00320)
  -- cycle;
% Reference line 0
\path[draw={rgb,1:red,0.78432;green,0.78432;blue,0.76471},line width=0.34870bp] (138.50017,66.80308)
  -- (138.50017,89.50310);
% Reference line 1
\path[draw={rgb,1:red,0.78432;green,0.78432;blue,0.76471},line width=0.34870bp] (211.50027,66.80308)
  -- (211.50027,89.50310);
% Reference line 2
\path[draw={rgb,1:red,0.78432;green,0.78432;blue,0.76471},line width=0.34870bp] (284.50037,66.80308)
  -- (284.50037,89.50310);
% Reference line 3
\path[draw={rgb,1:red,0.78432;green,0.78432;blue,0.76471},line width=0.34870bp] (357.50046,66.80308)
  -- (357.50046,89.50310);
% Reference line 4
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (110.42012,89.50310)
  -- (391.19050,89.50310);
% Reference line 5
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (110.42012,89.50310)
  -- (110.42012,91.00309);
% Reference line 6
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (166.58022,89.50310)
  -- (166.58022,91.00309);
% Reference line 7
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (222.73027,89.50310)
  -- (222.73027,91.00309);
% Reference line 8
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (278.88036,89.50310)
  -- (278.88036,91.00309);
% Reference line 9
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (335.04042,89.50310)
  -- (335.04042,91.00309);
% Reference line 10
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.34870bp] (391.19050,89.50310)
  -- (391.19050,91.00309);
% Reference line 11
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (60.16008,211.60328)
  -- (60.16008,231.00330);
% Reference line 12
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (74.97008,211.60328)
  -- (74.97008,231.00330);
% Reference line 13
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (89.78010,211.60328)
  -- (89.78010,231.00330);
% Reference line 14
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (104.59012,211.60328)
  -- (104.59012,231.00330);
% Reference line 15
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (119.39014,211.60328)
  -- (119.39014,231.00330);
% Reference line 16
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (134.20015,211.60328)
  -- (134.20015,231.00330);
% Reference line 17
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (149.01018,211.60328)
  -- (149.01018,231.00330);
% Reference line 18
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (163.82020,211.60328)
  -- (163.82020,231.00330);
% Reference line 19
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.29887bp] (53.50006,214.00327)
  -- (169.00021,214.00327);
% Reference line 20
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.29887bp] (53.50006,221.50327)
  -- (169.00021,221.50327);
% Reference line 21
\path[draw={rgb,1:red,0.604;green,0.604;blue,0.604},line width=0.29887bp] (53.50006,229.00330)
  -- (169.00021,229.00330);
% Reference line 22
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (60.16008,212.00327)
  -- (60.16008,216.00327);
% Reference line 23
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (74.97008,212.00327)
  -- (74.97008,216.00327);
% Reference line 24
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (89.78010,212.00327)
  -- (89.78010,216.00327);
% Reference line 25
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (104.59012,212.00327)
  -- (104.59012,216.00327);
% Reference line 26
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (119.39014,212.00327)
  -- (119.39014,216.00327);
% Reference line 27
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (134.20015,212.00327)
  -- (134.20015,216.00327);
% Reference line 28
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (149.01018,212.00327)
  -- (149.01018,216.00327);
% Reference line 29
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (163.82020,212.00327)
  -- (163.82020,216.00327);
% Reference line 30
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (69.91008,227.00329)
  -- (69.91008,231.00330);
% Reference line 31
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (114.33014,227.00329)
  -- (114.33014,231.00330);
% Reference line 32
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.49814bp] (158.75020,227.00329)
  -- (158.75020,231.00330);
% Reference line 33
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (202.67026,225.29328)
  -- (177.00023,204.26325);
% Reference line 34
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (211.22026,218.28327)
  -- (185.56024,197.25326);
% Reference line 35
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (219.78029,211.27328)
  -- (194.11024,190.25324);
% Reference line 36
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (228.33029,204.26325)
  -- (202.67026,183.24323);
% Reference line 37
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (236.89030,197.25326)
  -- (211.22026,176.23322);
% Reference line 38
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (245.44030,190.25324)
  -- (219.78029,169.22320);
% Reference line 39
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (254.00034,183.24323)
  -- (228.33029,162.21320);
% Reference line 40
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (202.67026,225.29328)
  -- (254.00034,183.24323);
% Reference line 41
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (194.11024,218.28327)
  -- (245.44030,176.23322);
% Reference line 42
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (185.56024,211.27328)
  -- (236.89030,169.22320);
% Reference line 43
\path[draw={rgb,1:red,0.855;green,0.855;blue,0.839},line width=0.29887bp] (177.00023,204.26325)
  -- (228.33029,162.21320);
% Reference line 44
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (201.20024,181.87322)
  -- (204.45026,175.32322);
% Reference line 45
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (201.20024,181.87322)
  -- (208.01025,185.69325);
% Reference line 46
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (201.20024,181.87322)
  -- (203.44026,179.78323);
% Reference line 47
\path[draw={rgb,1:red,0.784;green,0.255;blue,0.294},line width=0.54794bp] (201.20024,181.87322)
  -- (204.45026,175.32322);
% Reference line 48
\path[draw={rgb,1:red,0.243;green,0.604;blue,0.322},line width=0.54794bp] (201.20024,181.87322)
  -- (208.01025,185.69325);
% Reference line 49
\path[draw={rgb,1:red,0.18;green,0.427;blue,0.706},line width=0.54794bp] (201.20024,181.87322)
  -- (203.44026,179.78323);
% Reference line 50
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (237.16031,170.35322)
  -- (231.84029,164.57320);
% Reference line 51
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (237.16031,170.35322)
  -- (242.48030,165.25321);
% Reference line 52
\path[draw={rgb,1:red,1.0;green,1.0;blue,1.0},line width=1.69366bp] (237.16031,170.35322)
  -- (234.87030,171.92321);
% Reference line 53
\path[draw={rgb,1:red,0.784;green,0.255;blue,0.294},line width=0.54794bp] (237.16031,170.35322)
  -- (231.84029,164.57320);
% Reference line 54
\path[draw={rgb,1:red,0.243;green,0.604;blue,0.322},line width=0.54794bp] (237.16031,170.35322)
  -- (242.48030,165.25321);
% Reference line 55
\path[draw={rgb,1:red,0.18;green,0.427;blue,0.706},line width=0.54794bp] (237.16031,170.35322)
  -- (234.87030,171.92321);
% Reference line 56
\path[draw=pipelineteal,line width=0.59776bp] (17.00002,104.40312)
  -- (17.00002,113.90200);
% Reference line 57
\path[draw=pipelineteal,line width=0.59776bp] (29.20001,159.00320)
  -- (31.89890,159.00320);
% Reference line 58
\path[draw=pipelineteal,line width=0.49814bp] (321.95041,178.80323)
  -- (321.95041,184.25228);
% Reference line 59
\path[draw=pipelineteal,line width=.49814bp,
  rounded corners=.8bp]
  (377.00050,178.80323) -- (377.00050,183) -- (393,183)
  -- (393,206) -- (377.00050,206) -- (377.00050,206.25231);
% Reference line 60
\path[draw=pipelineteal,line width=0.59776bp] (265.20033,158.00320)
  -- (279.89923,158.00320);

% Timeline markers are painted after their horizontal grid lines.
% Reference curve 36
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (60.96008,221.50327)
  .. controls (60.96008,221.06146) and (60.60190,220.70327) .. (60.16008,220.70327)
  .. controls (59.71825,220.70327) and (59.36008,221.06146) .. (59.36008,221.50327)
  .. controls (59.36008,221.94511) and (59.71825,222.30330) .. (60.16008,222.30330)
  .. controls (60.60190,222.30330) and (60.96008,221.94511) .. (60.96008,221.50327)
  -- cycle;
% Reference curve 37
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (75.77010,221.50327)
  .. controls (75.77010,221.06146) and (75.41191,220.70327) .. (74.97008,220.70327)
  .. controls (74.52826,220.70327) and (74.17007,221.06146) .. (74.17007,221.50327)
  .. controls (74.17007,221.94511) and (74.52826,222.30330) .. (74.97008,222.30330)
  .. controls (75.41191,222.30330) and (75.77010,221.94511) .. (75.77010,221.50327)
  -- cycle;
% Reference curve 38
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (90.58011,221.50327)
  .. controls (90.58011,221.06146) and (90.22194,220.70327) .. (89.78010,220.70327)
  .. controls (89.33827,220.70327) and (88.98010,221.06146) .. (88.98010,221.50327)
  .. controls (88.98010,221.94511) and (89.33827,222.30330) .. (89.78010,222.30330)
  .. controls (90.22194,222.30330) and (90.58011,221.94511) .. (90.58011,221.50327)
  -- cycle;
% Reference curve 39
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (105.39012,221.50327)
  .. controls (105.39012,221.06146) and (105.03195,220.70327) .. (104.59012,220.70327)
  .. controls (104.14828,220.70327) and (103.79012,221.06146) .. (103.79012,221.50327)
  .. controls (103.79012,221.94511) and (104.14828,222.30330) .. (104.59012,222.30330)
  .. controls (105.03195,222.30330) and (105.39012,221.94511) .. (105.39012,221.50327)
  -- cycle;
% Reference curve 40
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (120.19016,221.50327)
  .. controls (120.19016,221.06146) and (119.83197,220.70327) .. (119.39014,220.70327)
  .. controls (118.94832,220.70327) and (118.59013,221.06146) .. (118.59013,221.50327)
  .. controls (118.59013,221.94511) and (118.94832,222.30330) .. (119.39014,222.30330)
  .. controls (119.83197,222.30330) and (120.19016,221.94511) .. (120.19016,221.50327)
  -- cycle;
% Reference curve 41
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (135.00015,221.50327)
  .. controls (135.00015,221.06146) and (134.64198,220.70327) .. (134.20015,220.70327)
  .. controls (133.75833,220.70327) and (133.40015,221.06146) .. (133.40015,221.50327)
  .. controls (133.40015,221.94511) and (133.75833,222.30330) .. (134.20015,222.30330)
  .. controls (134.64198,222.30330) and (135.00015,221.94511) .. (135.00015,221.50327)
  -- cycle;
% Reference curve 42
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (149.81018,221.50327)
  .. controls (149.81018,221.06146) and (149.45201,220.70327) .. (149.01018,220.70327)
  .. controls (148.56834,220.70327) and (148.21017,221.06146) .. (148.21017,221.50327)
  .. controls (148.21017,221.94511) and (148.56834,222.30330) .. (149.01018,222.30330)
  .. controls (149.45201,222.30330) and (149.81018,221.94511) .. (149.81018,221.50327)
  -- cycle;
% Reference curve 43
\path[fill={rgb,1:red,0.0;green,0.0;blue,0.0}] (164.62021,221.50327)
  .. controls (164.62021,221.06146) and (164.26204,220.70327) .. (163.82020,220.70327)
  .. controls (163.37837,220.70327) and (163.02020,221.06146) .. (163.02020,221.50327)
  .. controls (163.02020,221.94511) and (163.37837,222.30330) .. (163.82020,222.30330)
  .. controls (164.26204,222.30330) and (164.62021,221.94511) .. (164.62021,221.50327)
  -- cycle;
% Reference curve 44
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (60.96008,229.00330)
  .. controls (60.96008,228.56147) and (60.60190,228.20330) .. (60.16008,228.20330)
  .. controls (59.71825,228.20330) and (59.36008,228.56147) .. (59.36008,229.00330)
  .. controls (59.36008,229.44512) and (59.71825,229.80331) .. (60.16008,229.80331)
  .. controls (60.60190,229.80331) and (60.96008,229.44512) .. (60.96008,229.00330)
  -- cycle;
% Reference curve 45
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (75.77010,229.00330)
  .. controls (75.77010,228.56147) and (75.41191,228.20330) .. (74.97008,228.20330)
  .. controls (74.52826,228.20330) and (74.17007,228.56147) .. (74.17007,229.00330)
  .. controls (74.17007,229.44512) and (74.52826,229.80331) .. (74.97008,229.80331)
  .. controls (75.41191,229.80331) and (75.77010,229.44512) .. (75.77010,229.00330)
  -- cycle;
% Reference curve 46
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (90.58011,229.00330)
  .. controls (90.58011,228.56147) and (90.22194,228.20330) .. (89.78010,228.20330)
  .. controls (89.33827,228.20330) and (88.98010,228.56147) .. (88.98010,229.00330)
  .. controls (88.98010,229.44512) and (89.33827,229.80331) .. (89.78010,229.80331)
  .. controls (90.22194,229.80331) and (90.58011,229.44512) .. (90.58011,229.00330)
  -- cycle;
% Reference curve 47
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (105.39012,229.00330)
  .. controls (105.39012,228.56147) and (105.03195,228.20330) .. (104.59012,228.20330)
  .. controls (104.14828,228.20330) and (103.79012,228.56147) .. (103.79012,229.00330)
  .. controls (103.79012,229.44512) and (104.14828,229.80331) .. (104.59012,229.80331)
  .. controls (105.03195,229.80331) and (105.39012,229.44512) .. (105.39012,229.00330)
  -- cycle;
% Reference curve 48
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (120.19016,229.00330)
  .. controls (120.19016,228.56147) and (119.83197,228.20330) .. (119.39014,228.20330)
  .. controls (118.94832,228.20330) and (118.59013,228.56147) .. (118.59013,229.00330)
  .. controls (118.59013,229.44512) and (118.94832,229.80331) .. (119.39014,229.80331)
  .. controls (119.83197,229.80331) and (120.19016,229.44512) .. (120.19016,229.00330)
  -- cycle;
% Reference curve 49
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (135.00015,229.00330)
  .. controls (135.00015,228.56147) and (134.64198,228.20330) .. (134.20015,228.20330)
  .. controls (133.75833,228.20330) and (133.40015,228.56147) .. (133.40015,229.00330)
  .. controls (133.40015,229.44512) and (133.75833,229.80331) .. (134.20015,229.80331)
  .. controls (134.64198,229.80331) and (135.00015,229.44512) .. (135.00015,229.00330)
  -- cycle;
% Reference curve 50
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (149.81018,229.00330)
  .. controls (149.81018,228.56147) and (149.45201,228.20330) .. (149.01018,228.20330)
  .. controls (148.56834,228.20330) and (148.21017,228.56147) .. (148.21017,229.00330)
  .. controls (148.21017,229.44512) and (148.56834,229.80331) .. (149.01018,229.80331)
  .. controls (149.45201,229.80331) and (149.81018,229.44512) .. (149.81018,229.00330)
  -- cycle;
% Reference curve 51
\path[draw={rgb,1:red,0.0;green,0.0;blue,0.0},line width=0.32877bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (164.62021,229.00330)
  .. controls (164.62021,228.56147) and (164.26204,228.20330) .. (163.82020,228.20330)
  .. controls (163.37837,228.20330) and (163.02020,228.56147) .. (163.02020,229.00330)
  .. controls (163.02020,229.44512) and (163.37837,229.80331) .. (163.82020,229.80331)
  .. controls (164.26204,229.80331) and (164.62021,229.44512) .. (164.62021,229.00330)
  -- cycle;


==> figures/pipeline/plots/bimanual-trajectories.tex <==
% Exact reference trace vertices, rendered with native TikZ paths.
% Reference trace 52
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.49814bp] (194.11024,208.05328)
  -- (194.15024,207.96328)
  -- (194.23024,207.90325)
  -- (194.27025,207.96328)
  -- (194.27025,207.92326)
  -- (194.34024,207.93325)
  -- (194.21025,207.96328)
  -- (194.20024,207.92326)
  -- (194.28024,207.94326)
  -- (194.32025,207.83326)
  -- (194.28024,207.69328)
  -- (194.32025,207.76327)
  -- (194.25024,207.86326)
  -- (194.38025,207.91326)
  -- (194.09024,207.74326)
  -- (194.70024,207.63326)
  -- (195.99025,206.68325)
  -- (197.77025,203.31324)
  -- (199.90025,198.55325)
  -- (203.24026,196.02325)
  -- (208.16028,196.15324)
  -- (208.56027,196.22325)
  -- (208.44026,195.31324)
  -- (209.04025,191.58325)
  -- (210.31026,186.56324)
  -- (211.86026,183.51322)
  -- (213.53026,182.17323)
  -- (214.83028,181.93322)
  -- (216.48027,182.17323)
  -- (217.04027,182.35323)
  -- (217.21028,182.76322)
  -- (217.20027,183.48322)
  -- (217.14027,183.78324)
  -- (217.21028,183.71324)
  -- (216.89027,183.75323)
  -- (216.30028,184.63323)
  -- (215.89027,184.96325)
  -- (216.11028,185.26322)
  -- (216.36028,185.27325)
  -- (216.10028,185.33323)
  -- (215.98027,185.62322)
  -- (215.90027,185.98324)
  -- (216.00027,186.13323)
  -- (215.48027,187.54324)
  -- (216.20026,188.61324)
  -- (216.05028,188.66323)
  -- (216.38028,189.47325)
  -- (216.34027,189.46324)
  -- (216.32028,189.56324)
  -- (215.78027,188.44323)
  -- (214.92027,187.46324)
  -- (210.67027,184.42323)
  -- (207.56027,182.54322)
  -- (204.26025,181.17323)
  -- (201.20024,181.87322)
  -- (199.80026,186.07325)
  -- (199.32027,190.78324)
  -- (200.11024,193.50324)
  -- (201.80026,194.37324)
  -- (202.61026,195.02325)
  -- (201.98026,196.09326)
  -- (202.06026,196.69326)
  -- (202.58026,196.71325)
  -- (202.91025,196.67326)
  -- (203.35027,196.80326)
  -- (203.76025,197.07327)
  -- (203.92026,197.48324)
  -- (204.49026,197.78326)
  -- (204.99026,197.80326)
  -- (205.39026,197.64324)
  -- (206.02026,197.31324)
  -- (206.61026,196.36326)
  -- (206.86026,195.32325)
  -- (207.18027,195.31324)
  -- (206.88026,195.88325)
  -- (206.44026,196.02325)
  -- (205.98026,196.45326)
  -- (205.76025,197.08325)
  -- (206.27026,196.55325)
  -- (206.29027,196.47326)
  -- (206.21027,196.46325)
  -- (206.18027,196.50324)
  -- (206.28026,196.55325)
  -- (206.47026,196.54324)
  -- (206.78027,196.60327)
  -- (207.12025,196.51324)
  -- (208.72026,195.89326)
  -- (208.62025,195.85325)
  -- (208.44026,195.94325)
  -- (208.36028,195.91325)
  -- (208.37025,195.54324)
  -- (208.10027,194.04324)
  -- (207.37025,192.12324)
  -- (206.80028,189.83325)
  -- (204.44026,188.32325)
  -- (203.03026,189.02323)
  -- (203.25026,189.15322)
  -- (203.48026,188.98324)
  -- (203.74026,188.68322)
  -- (204.70026,187.05325)
  -- (204.38026,186.36324)
  -- (203.86026,187.39323)
  -- (203.80026,187.59323)
  -- (203.53026,187.76324)
  -- (202.62024,188.74325)
  -- (202.44025,188.88323)
  -- (202.39026,189.01324)
  -- (202.44025,189.18324)
  -- (202.56026,188.72325)
  -- (203.21027,187.84323)
  -- (203.68025,185.20323)
  -- (202.44025,185.86323)
  -- (201.85027,187.47325)
  -- (201.93024,187.59323)
  -- (201.95024,188.09324)
  -- (201.81026,188.85325)
  -- (199.34026,188.67324)
  -- (199.67026,188.22323)
  -- (199.28024,186.45324)
  -- (197.67026,184.99323)
  -- (197.46025,185.91323)
  -- (197.41025,188.36324)
  -- (198.13025,190.72325)
  -- (199.66025,192.36324)
  -- (200.75024,192.61324)
  -- (201.52026,191.69325)
  -- (202.09026,190.14324)
  -- (202.11024,188.22323)
  -- (202.43025,186.58325)
  -- (202.93024,184.99323)
  -- (203.21027,184.70323)
  -- (203.38026,184.44323)
  -- (203.47026,184.03323)
  -- (203.42024,183.84323)
  -- (203.31024,183.79322)
  -- (203.19026,184.66323)
  -- (203.45026,184.87324)
  -- (203.66026,184.36323)
  -- (203.36026,184.26322)
  -- (203.53026,184.53323)
  -- (204.25026,184.64323)
  -- (204.57027,184.89324)
  -- (204.30026,185.31323)
  -- (203.65025,186.64323)
  -- (203.07027,187.49325)
  -- (203.03026,187.28323)
  -- (202.92026,187.26322)
  -- (202.65025,187.41325)
  -- (202.52026,187.27325)
  -- (203.27026,186.42323)
  -- (203.78026,184.82324)
  -- (203.89026,184.67324)
  -- (202.81026,186.42323)
  -- (201.85027,187.78324)
  -- (201.59026,187.63325)
  -- (201.41026,187.14324)
  -- (200.97026,184.79322)
  -- (199.68024,182.18322)
  -- (199.18025,181.54322)
  -- (198.46025,181.42323)
  -- (197.15024,181.80323)
  -- (197.19025,183.17323)
  -- (197.82025,184.62322)
  -- (198.90024,186.29324)
  -- (198.90024,186.53323)
  -- (199.04024,186.00324)
  -- (199.38026,185.38325)
  -- (200.19026,184.69325)
  -- (201.52026,183.92323)
  -- (203.14026,182.55323)
  -- (204.68025,180.66323)
  -- (205.40025,179.33322)
  -- (204.94026,179.63323)
  -- (204.12025,181.63323)
  -- (204.16026,182.16323)
  -- (204.35027,182.06323)
  -- (204.87025,181.35323)
  -- (204.82027,180.77323)
  -- (204.98026,181.92323)
  -- (204.82027,181.85323)
  -- (205.34026,182.09323)
  -- (204.54025,183.19323)
  -- (203.74026,184.52323)
  -- (203.60027,184.90322)
  -- (203.77026,185.09324)
  -- (204.03026,184.96325)
  -- (204.48026,184.08323)
  -- (205.16026,182.93322)
  -- (206.34026,182.96324)
  -- (206.03026,183.46324)
  -- (204.10027,185.51322)
  -- (203.62024,185.75323)
  -- (202.43025,186.00324)
  -- (202.38026,184.79322)
  -- (201.71025,180.62321)
  -- (200.41026,178.39323)
  -- (198.65025,179.31321)
  -- (197.80026,182.93322)
  -- (198.44025,187.40322)
  -- (199.46025,191.16325)
  -- (200.56026,193.54324)
  -- (201.67026,194.60327)
  -- (202.22025,195.31324)
  -- (202.97026,196.56326)
  -- (203.24026,197.25326)
  -- (203.68025,197.88325)
  -- (204.34026,198.45326)
  -- (205.02026,199.32327)
  -- (205.52026,199.51324)
  -- (205.82027,199.41326)
  -- (206.13026,199.19325)
  -- (206.46027,199.08325)
  -- (206.08026,198.88325)
  -- (205.27026,198.62324)
  -- (204.99026,198.70324)
  -- (205.50026,200.09326)
  -- (205.42026,202.14326)
  -- (205.31026,202.58326)
  -- (205.14026,202.42324)
  -- (205.22026,201.84324)
  -- (205.57027,201.05326)
  -- (206.07027,200.14326)
  -- (206.74026,199.13325)
  -- (207.03026,197.90324)
  -- (207.18027,196.22325)
  -- (207.41026,195.06324)
  -- (207.97026,194.50324)
  -- (209.06026,193.78324)
  -- (209.57027,193.32325)
  -- (209.86026,193.26324)
  -- (209.50026,193.48324)
  -- (209.15025,194.07325)
  -- (209.40025,194.20324)
  -- (209.95026,194.14324)
  -- (210.32028,194.18324)
  -- (210.75026,194.38325)
  -- (210.94028,194.40324)
  -- (210.46027,194.32325)
  -- (208.23026,194.23324)
  -- (206.95026,194.26324)
  -- (206.76025,193.90324)
  -- (206.43025,193.77325)
  -- (205.82027,193.75324)
  -- (205.66026,194.22325)
  -- (206.35027,195.21325)
  -- (207.06026,195.83325)
  -- (207.30026,196.17324)
  -- (207.08026,196.10325)
  -- (206.82027,196.28324)
  -- (206.51025,196.35325)
  -- (205.77026,196.35325)
  -- (204.87025,196.63325)
  -- (203.45026,195.39324)
  -- (202.76025,195.19325)
  -- (201.98026,195.59324)
  -- (201.50026,196.39324)
  -- (201.16026,197.15324)
  -- (200.90025,198.07327)
  -- (201.00026,198.27326)
  -- (201.13025,198.33325)
  -- (201.35025,198.22325)
  -- (201.41026,198.14326)
  -- (201.38026,197.94326)
  -- (201.68025,197.63326)
  -- (202.20024,196.68324)
  -- (202.77026,196.29325)
  -- (203.56026,196.54324)
  -- (204.51025,197.56326)
  -- (204.74026,197.63326)
  -- (204.90025,197.73324)
  -- (204.93025,198.03326)
  -- (204.27026,199.41326)
  -- (204.23026,199.62324)
  -- (204.35027,199.56326)
  -- (204.51025,199.59324)
  -- (205.30026,199.99326)
  -- (206.06026,200.57325)
  -- (206.29027,200.87325)
  -- (206.27026,201.10327)
  -- (205.60028,201.67326)
  -- (204.63026,202.40324)
  -- (204.45026,202.37325)
  -- (205.16026,201.89326)
  -- (205.63026,201.69326)
  -- (206.32027,201.49326)
  -- (206.91026,201.50326)
  -- (206.94026,201.65325)
  -- (206.20026,201.56326)
  -- (205.43025,201.76325)
  -- (204.77026,202.00326)
  -- (204.57027,202.23326)
  -- (204.60027,202.51324)
  -- (204.73026,202.67326)
  -- (205.18025,202.85327)
  -- (205.32027,202.84326)
  -- (205.32027,202.92326)
  -- (204.98026,203.25326)
  -- (204.70026,203.40324)
  -- (205.34026,203.11324)
  -- (205.49026,203.10327)
  -- (205.73026,203.22325)
  -- (205.67026,203.38326)
  -- (205.61026,203.31324)
  -- (205.75026,203.21327)
  -- (206.19026,203.12325)
  -- (206.59026,203.28326)
  -- (206.80028,203.67326)
  -- (206.68025,204.16326)
  -- (206.41026,204.37325)
  -- (206.11026,204.30326)
  -- (205.84026,204.12325)
  -- (205.70026,203.77326)
  -- (205.69028,203.34326)
  -- (205.81026,203.05326)
  -- (205.93025,202.81326)
  -- (206.01025,202.82325)
  -- (206.05026,203.04325)
  -- (205.93025,203.34326)
  -- (205.77026,203.52326)
  -- (205.86026,203.31324)
  -- (206.10027,203.19326)
  -- (206.87027,202.98326)
  -- (206.82027,202.69326)
  -- (206.70026,202.68325)
  -- (207.10027,202.92326)
  -- (207.00027,202.94326)
  -- (206.35027,202.85327)
  -- (205.82027,202.87325)
  -- (205.16026,202.78326)
  -- (203.89026,202.51324)
  -- (203.29025,202.50326)
  -- (202.58026,202.52326)
  -- (201.55025,202.67326)
  -- (200.52026,202.87325)
  -- (199.54025,203.11324)
  -- (199.01025,203.53326)
  -- (198.61024,205.17326)
  -- (198.12025,206.11326)
  -- (198.35025,206.11326)
  -- (198.56026,206.04325)
  -- (198.52026,206.08326)
  -- (198.59024,206.19326)
  -- (198.47026,206.45326)
  -- (198.59024,206.41326)
  -- (198.69026,206.29327)
  -- (198.52026,206.51325)
  -- (198.59024,206.43325)
  -- (198.48024,206.46327)
  -- (198.39024,206.56326)
  -- (198.53024,206.58328)
  -- (198.59024,206.45326);
% Reference trace 53
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.49814bp] (234.01030,180.45323)
  -- (233.91030,180.36323)
  -- (233.98030,180.27323)
  -- (233.97029,180.39323)
  -- (234.07031,180.42321)
  -- (234.07031,180.34323)
  -- (233.95029,180.39323)
  -- (233.66030,180.64323)
  -- (233.26028,180.76322)
  -- (232.80031,180.53323)
  -- (231.91030,180.57324)
  -- (230.54028,181.88323)
  -- (229.53029,184.92323)
  -- (229.93028,188.00324)
  -- (230.78030,190.80325)
  -- (231.17029,193.15324)
  -- (231.61029,194.34324)
  -- (231.93028,194.56324)
  -- (231.90028,195.11324)
  -- (231.58030,195.40324)
  -- (230.90028,195.42324)
  -- (230.38031,195.52325)
  -- (230.28029,195.44325)
  -- (230.78030,194.88325)
  -- (230.74030,194.84324)
  -- (230.82030,194.08325)
  -- (230.81029,192.45324)
  -- (230.68028,190.80325)
  -- (230.47030,189.74325)
  -- (230.53029,188.90324)
  -- (230.46030,188.03324)
  -- (230.29030,187.23324)
  -- (229.79028,186.12322)
  -- (229.69030,185.40322)
  -- (229.63030,184.18324)
  -- (229.63030,184.12322)
  -- (229.84029,184.40322)
  -- (229.68028,184.75323)
  -- (229.71030,184.66323)
  -- (230.56030,183.90322)
  -- (230.57030,183.60325)
  -- (230.17029,183.69325)
  -- (229.54028,184.04322)
  -- (228.96030,184.44323)
  -- (228.16030,184.37322)
  -- (227.56029,184.52323)
  -- (226.96030,184.82324)
  -- (226.80030,184.70323)
  -- (226.81029,184.56324)
  -- (226.78029,184.77323)
  -- (226.94029,184.78324)
  -- (227.07030,184.85323)
  -- (227.06029,185.09324)
  -- (227.25029,185.82324)
  -- (227.53029,186.52323)
  -- (227.97029,187.04322)
  -- (228.65028,187.32325)
  -- (228.85030,186.51322)
  -- (228.94029,185.85325)
  -- (229.35030,185.96325)
  -- (230.17029,185.86323)
  -- (230.92029,186.79322)
  -- (231.26028,188.09324)
  -- (231.11029,188.34324)
  -- (230.76030,187.58325)
  -- (230.22029,186.82324)
  -- (229.15028,186.63325)
  -- (228.29030,187.04322)
  -- (228.10030,187.34324)
  -- (228.49031,187.65324)
  -- (228.98030,187.79322)
  -- (229.24030,187.63325)
  -- (229.29030,188.04322)
  -- (229.95029,188.87324)
  -- (229.86029,189.39324)
  -- (229.20029,189.71324)
  -- (228.58029,190.15322)
  -- (226.84029,191.80325)
  -- (226.26028,192.58325)
  -- (225.41030,193.59324)
  -- (224.74030,194.29325)
  -- (224.02028,195.51324)
  -- (223.17027,196.29325)
  -- (221.80030,197.29325)
  -- (220.13028,198.26324)
  -- (218.98029,199.21327)
  -- (218.82028,199.81326)
  -- (218.71028,199.84324)
  -- (217.36028,199.47326)
  -- (217.30028,199.36326)
  -- (217.82028,199.04324)
  -- (218.58029,198.77325)
  -- (218.92027,198.84324)
  -- (218.98029,198.74326)
  -- (219.77028,199.11324)
  -- (219.93027,199.35325)
  -- (220.28027,199.66325)
  -- (220.69029,199.57325)
  -- (221.28027,199.51324)
  -- (222.10030,199.56326)
  -- (222.76028,199.54325)
  -- (223.28029,199.60327)
  -- (223.81029,199.52326)
  -- (224.20027,199.53324)
  -- (224.36029,199.71325)
  -- (224.78029,199.53324)
  -- (225.48029,199.48324)
  -- (225.74030,199.95324)
  -- (224.97029,199.87325)
  -- (223.78029,199.91325)
  -- (222.37027,199.51324)
  -- (221.01027,198.99325)
  -- (218.43027,197.53324)
  -- (217.77028,197.71325)
  -- (218.07030,197.87325)
  -- (219.07030,197.58326)
  -- (219.91028,196.90324)
  -- (220.57028,196.65325)
  -- (220.67029,197.30325)
  -- (220.24028,198.05326)
  -- (218.84027,197.90324)
  -- (217.92027,197.89326)
  -- (217.75027,197.97325)
  -- (217.37027,197.89326)
  -- (216.85028,197.90324)
  -- (216.73027,197.74326)
  -- (216.45027,197.71325)
  -- (215.93027,197.48324)
  -- (215.65027,197.59324)
  -- (215.47028,197.72325)
  -- (215.49028,197.67326)
  -- (215.93027,197.73324)
  -- (216.31027,198.09326)
  -- (216.49028,198.12325)
  -- (216.62027,198.01324)
  -- (216.71028,198.06324)
  -- (216.47028,198.03326)
  -- (216.09027,197.76325)
  -- (215.89027,197.68324)
  -- (216.42027,197.88325)
  -- (216.67027,198.22325)
  -- (216.73027,198.68324)
  -- (216.58028,198.94326)
  -- (216.12027,198.37324)
  -- (215.86028,197.48324)
  -- (216.40027,196.68324)
  -- (218.19028,194.85325)
  -- (218.41028,194.44325)
  -- (218.31027,194.41325)
  -- (218.10028,194.72325)
  -- (218.12027,194.90324)
  -- (218.32028,194.92324)
  -- (217.61028,195.06324)
  -- (217.53027,195.18325)
  -- (217.56027,195.63325)
  -- (217.31027,195.63325)
  -- (217.26027,195.57325)
  -- (217.74028,195.79324)
  -- (217.60030,195.85325)
  -- (217.42027,195.82325)
  -- (216.89027,195.27326)
  -- (216.71028,195.38326)
  -- (216.48027,195.25324)
  -- (216.55028,195.27326)
  -- (216.48027,195.29325)
  -- (216.77028,195.43324)
  -- (216.78027,195.63325)
  -- (216.63028,195.70324)
  -- (216.23027,195.48324)
  -- (215.97028,195.47326)
  -- (215.94028,195.55325)
  -- (216.52028,195.87325)
  -- (216.42027,195.95324)
  -- (216.31027,195.92324)
  -- (215.25027,194.73324)
  -- (215.56027,193.84324)
  -- (216.09027,193.15324)
  -- (216.41028,192.91323)
  -- (217.00029,193.23324)
  -- (216.94028,193.29324)
  -- (217.09029,193.42324)
  -- (217.42027,193.52325)
  -- (217.30028,193.37324)
  -- (217.42027,193.31324)
  -- (217.42027,193.24325)
  -- (217.56027,193.51324)
  -- (217.53027,193.54324)
  -- (217.42027,193.52325)
  -- (217.47028,193.54324)
  -- (217.51027,193.47325)
  -- (217.51027,193.30325)
  -- (217.75027,192.62324)
  -- (217.95027,192.40322)
  -- (218.02028,192.42324)
  -- (218.02028,192.91323)
  -- (217.90027,193.73324)
  -- (218.02028,193.89324)
  -- (217.53027,193.72325)
  -- (216.92027,193.63325)
  -- (216.80030,193.71325)
  -- (216.88028,194.04324)
  -- (217.20027,194.48324)
  -- (217.04027,194.31324)
  -- (216.99028,194.18324)
  -- (216.58028,193.85325)
  -- (216.48027,193.21325)
  -- (217.27028,192.21325)
  -- (218.85028,191.48324)
  -- (220.68027,191.30325)
  -- (221.93027,192.19325)
  -- (222.20027,193.49325)
  -- (222.10030,194.34324)
  -- (222.12029,195.11324)
  -- (222.34029,196.32325)
  -- (221.99028,196.68324)
  -- (222.05030,196.28324)
  -- (223.34029,195.91325)
  -- (223.41030,195.55325)
  -- (223.44028,194.62324)
  -- (223.35028,192.91323)
  -- (222.79028,191.29324)
  -- (222.19028,189.91323)
  -- (220.76028,188.75323)
  -- (219.39027,188.86323)
  -- (218.27030,189.65324)
  -- (216.83028,190.14324)
  -- (215.28027,191.40322)
  -- (214.40025,192.73324)
  -- (214.02026,192.95324)
  -- (213.78027,193.32325)
  -- (213.53026,193.83325)
  -- (213.48027,193.73324)
  -- (213.87027,193.96325)
  -- (213.97028,194.48324)
  -- (213.08028,194.97325)
  -- (212.29027,195.70324)
  -- (212.09027,195.95324)
  -- (212.25027,195.85325)
  -- (212.49028,195.34324)
  -- (212.86026,195.00326)
  -- (212.98027,194.73324)
  -- (212.49028,193.73324)
  -- (212.37027,193.63325)
  -- (212.48027,194.00326)
  -- (212.76027,194.28324)
  -- (212.85028,194.15324)
  -- (213.15025,194.26324)
  -- (213.19028,194.21325)
  -- (213.14027,193.96325)
  -- (213.04025,193.79324)
  -- (213.34027,193.39324)
  -- (214.26027,191.97325)
  -- (217.06027,185.25324)
  -- (220.21028,179.89323)
  -- (224.79028,174.86321)
  -- (229.58030,171.64321)
  -- (233.68028,170.14321)
  -- (236.38031,169.54320)
  -- (238.10031,169.48321)
  -- (239.21031,169.34321)
  -- (239.83030,168.61321)
  -- (239.66031,168.30322)
  -- (238.65030,167.77322)
  -- (235.47030,167.72321)
  -- (230.56030,168.92321)
  -- (224.48029,171.96322)
  -- (218.98029,176.20321)
  -- (215.75027,180.46324)
  -- (214.23027,184.59323)
  -- (213.32028,188.18324)
  -- (212.48027,190.56324)
  -- (211.90027,192.04324)
  -- (211.46027,193.47325)
  -- (210.76027,194.93324)
  -- (210.30026,195.16325)
  -- (210.33026,195.68324)
  -- (210.10027,194.89326)
  -- (209.71027,192.85325)
  -- (209.80028,189.13323)
  -- (211.21028,183.78324)
  -- (214.80028,178.08323)
  -- (219.85030,173.34321)
  -- (224.83029,170.44322)
  -- (228.98030,169.00321)
  -- (232.18030,169.04320)
  -- (234.29030,170.02322)
  -- (235.94030,170.88322)
  -- (236.95030,171.32322)
  -- (237.31029,171.03321)
  -- (237.16031,170.35322)
  -- (236.25030,169.21322)
  -- (234.01030,167.82320)
  -- (230.42029,167.37321)
  -- (226.12029,168.32322)
  -- (222.46028,170.59321)
  -- (219.39027,173.62321)
  -- (216.35028,177.38323)
  -- (213.80028,181.22323)
  -- (212.49028,184.63323)
  -- (210.68025,190.54324)
  -- (210.39026,190.64323)
  -- (210.04025,190.96325)
  -- (209.81026,191.54324)
  -- (209.46027,191.67324)
  -- (209.79025,191.81324)
  -- (209.73026,191.47325)
  -- (209.69028,190.65324)
  -- (210.61028,190.89324)
  -- (211.62025,192.10325)
  -- (211.32028,192.28324)
  -- (210.77026,193.52325)
  -- (210.52028,196.33325)
  -- (211.08026,198.86324)
  -- (210.14027,198.08325)
  -- (209.15025,196.37324)
  -- (208.50026,194.82325)
  -- (208.54027,193.13325)
  -- (209.50026,193.30325)
  -- (209.73026,195.03324)
  -- (209.14027,195.06324)
  -- (208.65027,195.37324)
  -- (208.25027,195.49326)
  -- (208.20026,195.57325)
  -- (208.48026,195.60327)
  -- (208.43025,195.58326)
  -- (208.43025,195.62324)
  -- (208.84026,195.46325)
  -- (208.90025,195.33325)
  -- (208.77026,195.13325)
  -- (209.03027,194.90324)
  -- (208.88026,194.09324)
  -- (209.11026,193.62324)
  -- (209.31026,193.87324)
  -- (209.33026,194.09324)
  -- (209.03027,194.15324)
  -- (208.47028,194.55325)
  -- (207.90025,194.66325)
  -- (207.53026,194.87324)
  -- (207.54025,195.03324)
  -- (207.71027,195.13325)
  -- (207.42026,195.25324)
  -- (207.38028,195.32325)
  -- (207.34026,195.21325)
  -- (207.41026,195.34324)
  -- (207.70026,195.56324)
  -- (207.81026,195.59324)
  -- (207.96028,195.49326)
  -- (207.93025,194.89326)
  -- (208.08026,192.91323)
  -- (209.27028,188.83325)
  -- (212.21028,183.13323)
  -- (217.05028,176.77322)
  -- (223.27030,171.67321)
  -- (228.70029,169.59321)
  -- (232.05031,169.77322)
  -- (234.08029,170.73321)
  -- (235.42029,171.70321)
  -- (236.13030,172.09323)
  -- (236.62029,171.92321)
  -- (236.99031,171.41322)
  -- (236.79030,170.84321)
  -- (236.34030,170.15320)
  -- (235.31029,169.41322)
  -- (233.53029,168.55322)
  -- (232.92030,168.86321)
  -- (232.67030,169.54320)
  -- (232.43030,171.15320)
  -- (232.23030,172.00323)
  -- (231.55030,173.77322)
  -- (231.40028,174.74323)
  -- (231.42029,175.64321)
  -- (231.87030,176.24322)
  -- (232.60031,176.74323)
  -- (233.35030,177.05323)
  -- (234.00030,177.53321)
  -- (234.64029,177.90322)
  -- (235.17030,178.08323)
  -- (235.50030,177.77322)
  -- (236.02030,177.41323)
  -- (235.74031,177.78323)
  -- (235.49031,178.27323)
  -- (235.47030,178.97323)
  -- (236.10031,178.47323)
  -- (236.34030,178.58323)
  -- (236.57031,178.34323)
  -- (236.45030,178.08323)
  -- (236.27031,178.23322)
  -- (236.38031,178.07324)
  -- (236.15028,178.13322)
  -- (236.23030,178.14323)
  -- (236.15028,178.07324);
% Reference trace 54
\path[draw={rgb,1:red,0.13725;green,0.62354;blue,0.65099},line width=0.44832bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (195.11024,208.05328)
  .. controls (195.11024,207.50099) and (194.66252,207.05326) .. (194.11024,207.05326)
  .. controls (193.55795,207.05326) and (193.11024,207.50099) .. (193.11024,208.05328)
  .. controls (193.11024,208.60555) and (193.55795,209.05328) .. (194.11024,209.05328)
  .. controls (194.66252,209.05328) and (195.11024,208.60555) .. (195.11024,208.05328)
  -- cycle;
% Reference trace 55
\path[draw={rgb,1:red,0.89804;green,0.50195;blue,0.27843},line width=0.44832bp,fill={rgb,1:red,1.0;green,1.0;blue,1.0}] (235.01030,180.45323)
  .. controls (235.01030,179.90093) and (234.56258,179.45323) .. (234.01030,179.45323)
  .. controls (233.45801,179.45323) and (233.01030,179.90093) .. (233.01030,180.45323)
  .. controls (233.01030,181.00552) and (233.45801,181.45323) .. (234.01030,181.45323)
  .. controls (234.56258,181.45323) and (235.01030,181.00552) .. (235.01030,180.45323)
  -- cycle;


==> figures/pipeline/plots/imu-traces.tex <==
% Exact reference trace vertices, rendered with native TikZ paths.
% Reference trace 20
\path[draw={rgb,1:red,0.465;green,0.767;blue,0.784},line width=0.32877bp] (110.44012,73.34309)
  -- (129.00017,73.36309)
  -- (130.04015,73.32310)
  -- (130.23016,73.36309)
  -- (130.66016,73.30308)
  -- (130.91016,73.38310)
  -- (131.75015,73.32310)
  -- (134.64017,73.34309)
  -- (135.18016,73.38310)
  -- (135.32018,73.55308)
  -- (135.37016,73.50308)
  -- (135.51015,73.67309)
  -- (135.65016,73.58310)
  -- (135.74017,73.61309)
  -- (135.85017,73.40307)
  -- (135.88017,73.62307)
  -- (135.99017,73.39308)
  -- (136.10017,73.44308)
  -- (136.27017,73.31307)
  -- (136.72017,73.50308)
  -- (137.11017,73.48307)
  -- (137.25017,73.41308)
  -- (137.28017,73.48307)
  -- (137.39017,73.22308)
  -- (137.45016,73.32310)
  -- (138.15016,72.57308)
  -- (138.21017,72.60310)
  -- (138.38019,72.45309)
  -- (138.88017,72.58310)
  -- (138.97017,72.53308)
  -- (138.99017,72.59307)
  -- (139.36018,72.52308)
  -- (139.42017,72.58310)
  -- (139.44017,72.48307)
  -- (139.70016,72.30308)
  -- (139.92017,72.42307)
  -- (140.23016,72.29308)
  -- (140.26016,72.38310)
  -- (140.29018,72.30308)
  -- (140.62016,72.40307)
  -- (140.76018,72.34309)
  -- (141.04016,72.53308)
  -- (141.30017,72.52308)
  -- (141.52019,72.63310)
  -- (141.58018,72.51307)
  -- (141.75017,72.60310)
  -- (141.77017,72.56309)
  -- (142.11017,72.62307)
  -- (142.14018,72.56309)
  -- (142.36018,72.60310)
  -- (142.62016,72.53308)
  -- (142.73016,72.59307)
  -- (143.04016,72.50308)
  -- (143.77017,72.54308)
  -- (143.99019,72.49310)
  -- (144.92018,72.65309)
  -- (145.14018,72.57308)
  -- (146.46019,72.61308)
  -- (148.04018,72.53308)
  -- (148.37018,72.45309)
  -- (148.60020,72.52308)
  -- (148.79018,72.48307)
  -- (148.82019,72.53308)
  -- (148.91019,72.42307)
  -- (150.68018,72.54308)
  -- (150.70018,72.61308)
  -- (150.73018,72.45309)
  -- (150.79018,72.58310)
  -- (150.82019,72.51307)
  -- (150.93018,72.50308)
  -- (151.01018,72.59307)
  -- (151.07020,72.50308)
  -- (151.10019,72.57308)
  -- (151.12018,72.49310)
  -- (151.15018,72.56309)
  -- (151.26018,72.47310)
  -- (151.29019,72.58310)
  -- (151.38020,72.46308)
  -- (151.41019,72.51307)
  -- (151.49020,72.44308)
  -- (151.52019,72.58310)
  -- (151.55019,72.47310)
  -- (151.66019,72.60310)
  -- (151.69020,72.27310)
  -- (151.71019,72.50308)
  -- (151.74020,72.44308)
  -- (151.80020,72.52308)
  -- (151.83018,72.31307)
  -- (151.85020,72.57308)
  -- (151.91019,72.29308)
  -- (151.94020,72.73307)
  -- (151.97018,72.21308)
  -- (152.05020,72.77308)
  -- (152.08018,72.20307)
  -- (152.11018,72.71308)
  -- (152.16020,72.40307)
  -- (152.19019,72.69310)
  -- (152.22018,72.37307)
  -- (152.28018,72.61308)
  -- (152.30019,72.41308)
  -- (152.44019,72.59307)
  -- (152.47020,72.41308)
  -- (152.50018,72.58310)
  -- (152.53018,72.42307)
  -- (152.56020,72.52308)
  -- (152.75018,72.41308)
  -- (152.95018,72.46308)
  -- (152.98020,72.32308)
  -- (153.01018,72.54308)
  -- (153.03020,72.45309)
  -- (153.26018,72.47310)
  -- (153.34020,72.40307)
  -- (153.37018,72.48307)
  -- (153.40018,72.44308)
  -- (153.54019,72.51307)
  -- (153.57019,72.45309)
  -- (153.60020,72.50308)
  -- (153.65019,72.45309)
  -- (153.71019,72.47310)
  -- (153.74020,72.39308)
  -- (153.76020,72.50308)
  -- (153.79018,72.43308)
  -- (153.82019,72.51307)
  -- (153.85020,72.43308)
  -- (153.93018,72.47310)
  -- (153.96020,72.42307)
  -- (154.02019,72.50308)
  -- (154.04018,72.41308)
  -- (154.07020,72.47310)
  -- (154.24019,72.51307)
  -- (154.27020,72.44308)
  -- (154.30020,72.56309)
  -- (154.35019,72.54308)
  -- (154.38020,72.28308)
  -- (154.41020,72.78309)
  -- (154.47020,72.13308)
  -- (154.49020,73.15307)
  -- (154.52020,72.22308)
  -- (154.58020,72.78309)
  -- (154.61020,72.14309)
  -- (154.63020,72.84307)
  -- (154.66019,72.33308)
  -- (154.72020,72.71308)
  -- (154.75018,72.22308)
  -- (154.77019,72.83310)
  -- (154.80020,72.29308)
  -- (154.83020,72.60310)
  -- (154.89020,72.35308)
  -- (154.91019,72.70307)
  -- (154.94020,72.39308)
  -- (155.00020,72.63310)
  -- (155.03020,72.27310)
  -- (155.06018,72.58310)
  -- (155.11018,72.35308)
  -- (155.14020,72.53308)
  -- (155.17018,72.40307)
  -- (155.22018,72.50308)
  -- (155.25020,72.41308)
  -- (155.28020,72.47310)
  -- (155.39020,72.42307)
  -- (155.62018,72.52308)
  -- (155.64018,72.47310)
  -- (155.95018,72.50308)
  -- (156.80020,72.28308)
  -- (157.10020,72.27310)
  -- (157.13019,72.33308)
  -- (157.16020,72.21308)
  -- (158.65019,72.39308)
  -- (159.86020,72.32308)
  -- (161.65019,72.34309)
  -- (161.85020,72.22308)
  -- (161.91020,72.37307)
  -- (161.96022,72.30308)
  -- (161.99020,72.36309)
  -- (162.02020,72.30308)
  -- (162.66020,72.29308)
  -- (163.00021,72.38310)
  -- (163.09021,72.30308)
  -- (163.17020,72.36309)
  -- (163.20020,72.24308)
  -- (163.23020,72.29308)
  -- (163.28020,72.23307)
  -- (163.34021,72.34309)
  -- (163.76021,72.32308)
  -- (163.84020,72.26307)
  -- (163.87021,72.31307)
  -- (163.93019,72.24308)
  -- (163.96022,72.35308)
  -- (163.98021,72.28308)
  -- (164.12021,72.36309)
  -- (164.21020,72.32308)
  -- (164.69022,72.40307)
  -- (165.47021,72.76309)
  -- (165.81021,72.62307)
  -- (166.15019,72.65309)
  -- (166.31020,72.59307)
  -- (167.10022,73.03309)
  -- (168.62020,73.14309)
  -- (168.90020,73.10308)
  -- (169.68020,72.82308)
  -- (171.34021,72.78309)
  -- (172.21022,72.70307)
  -- (173.78023,72.83310)
  -- (173.81021,72.88308)
  -- (174.12021,72.78309)
  -- (174.82022,72.81307)
  -- (175.02022,72.75308)
  -- (176.56023,72.94310)
  -- (177.24022,72.73307)
  -- (177.49023,72.78309)
  -- (177.55022,72.72308)
  -- (177.74023,72.74310)
  -- (178.05023,72.90307)
  -- (179.34023,72.84307)
  -- (179.71022,72.92309)
  -- (180.02022,72.87309)
  -- (180.58023,72.89309)
  -- (180.61023,72.98309)
  -- (180.72023,72.86308)
  -- (181.81023,72.91308)
  -- (182.37022,72.80310)
  -- (183.05023,72.86308)
  -- (185.52023,72.87309)
  -- (189.84023,72.79307)
  -- (190.15022,72.85310)
  -- (190.83025,72.80310)
  -- (191.67024,72.83310)
  -- (192.51022,72.73307)
  -- (193.16025,72.86308)
  -- (195.68024,72.76309)
  -- (195.99025,72.79307)
  -- (196.05025,73.53308)
  -- (196.19025,72.74310)
  -- (196.33025,72.92309)
  -- (196.41025,72.79307)
  -- (196.44025,72.89309)
  -- (196.58026,72.87309)
  -- (197.00026,73.03309)
  -- (197.26024,72.97308)
  -- (197.76025,73.00309)
  -- (197.96027,73.07310)
  -- (198.27026,72.98309)
  -- (199.31024,73.00309)
  -- (199.36026,73.08308)
  -- (199.42024,73.03309)
  -- (199.59024,73.19308)
  -- (199.61026,73.10308)
  -- (199.64024,73.14309)
  -- (199.75024,73.07310)
  -- (200.51024,73.12309)
  -- (201.10027,72.91308)
  -- (201.33025,73.25309)
  -- (201.35025,73.13308)
  -- (201.38026,73.28308)
  -- (201.44025,73.14309)
  -- (201.50026,73.22308)
  -- (201.52026,73.10308)
  -- (201.58026,73.16310)
  -- (201.64024,73.04307)
  -- (201.66026,73.12309)
  -- (201.80026,72.96310)
  -- (201.83026,73.03309)
  -- (201.97026,72.95307)
  -- (202.11024,72.98309)
  -- (202.28026,72.90307)
  -- (202.31024,72.79307)
  -- (202.37025,73.10308)
  -- (202.39026,72.79307)
  -- (202.42024,73.01307)
  -- (202.48026,72.87309)
  -- (202.51024,73.01307)
  -- (202.59026,72.94310)
  -- (202.62024,73.11308)
  -- (202.67026,72.99308)
  -- (202.70026,73.12309)
  -- (202.76025,73.04307)
  -- (202.79025,73.12309)
  -- (202.84026,73.04307)
  -- (202.87025,73.07310)
  -- (203.26025,72.95307)
  -- (204.53026,73.22308)
  -- (205.12025,73.09309)
  -- (205.26025,72.95307)
  -- (205.31026,73.12309)
  -- (205.37025,72.96310)
  -- (205.43025,73.09309)
  -- (205.45026,73.02308)
  -- (205.57027,73.14309)
  -- (205.65025,73.11308)
  -- (205.73026,73.44308)
  -- (205.85027,72.92309)
  -- (205.93025,73.16310)
  -- (206.13026,72.97308)
  -- (206.24026,73.11308)
  -- (206.32027,73.01307)
  -- (206.35027,73.13308)
  -- (206.38028,72.73307)
  -- (206.41026,73.20307)
  -- (206.46027,72.99308)
  -- (206.58028,73.06307)
  -- (206.61026,72.97308)
  -- (206.72026,73.08308)
  -- (206.91026,72.90307)
  -- (206.94026,72.99308)
  -- (207.05026,73.00309)
  -- (207.31026,72.92309)
  -- (207.34026,72.98309)
  -- (207.39026,72.89309)
  -- (207.53026,73.01307)
  -- (207.56027,72.90307)
  -- (207.64026,72.95307)
  -- (207.67027,72.83310)
  -- (207.70026,73.05310)
  -- (207.73026,72.94310)
  -- (207.81026,72.90307)
  -- (207.84026,72.99308)
  -- (207.90025,72.93307)
  -- (207.95026,73.03309)
  -- (207.98027,72.94310)
  -- (208.01025,73.00309)
  -- (208.09027,72.93307)
  -- (208.21027,73.13308)
  -- (208.23026,72.85310)
  -- (208.32027,73.32310)
  -- (208.35027,73.14309)
  -- (208.40025,73.17307)
  -- (208.43025,73.09309)
  -- (208.46027,73.14309)
  -- (208.60028,73.09309)
  -- (208.85028,72.85310)
  -- (208.94028,72.91308)
  -- (208.96028,72.74310)
  -- (209.02026,72.97308)
  -- (209.05028,72.80310)
  -- (209.10027,72.96310)
  -- (209.13026,72.85310)
  -- (209.22026,72.91308)
  -- (209.24026,72.86308)
  -- (209.27028,72.93307)
  -- (209.33026,72.81307)
  -- (209.55026,72.94310)
  -- (209.58028,72.90307)
  -- (209.72028,73.03309)
  -- (209.95026,72.93307)
  -- (210.06026,73.17307)
  -- (210.11026,72.99308)
  -- (210.23027,73.26307)
  -- (210.28026,73.19308)
  -- (210.42026,73.25309)
  -- (210.68025,73.17307)
  -- (211.27028,72.81307)
  -- (211.32028,72.85310)
  -- (211.55026,72.74310)
  -- (211.77026,72.95307)
  -- (211.80028,73.08308)
  -- (211.83028,75.91308)
  -- (211.91026,72.79307)
  -- (211.94028,72.86308)
  -- (212.00027,72.68307)
  -- (212.05028,73.13308)
  -- (212.11026,72.74310)
  -- (212.22026,72.94310)
  -- (212.31026,72.78309)
  -- (212.47028,72.93307)
  -- (212.56027,72.90307)
  -- (212.98027,73.03309)
  -- (213.12027,72.93307)
  -- (213.15025,73.04307)
  -- (213.20026,72.98309)
  -- (213.43027,73.00309)
  -- (213.51025,73.09309)
  -- (213.60028,73.09309)
  -- (213.62025,73.00309)
  -- (213.65027,73.11308)
  -- (213.71027,72.89309)
  -- (213.74028,72.99308)
  -- (213.79027,72.92309)
  -- (213.85028,73.05310)
  -- (213.88028,72.83310)
  -- (213.96028,73.20307)
  -- (214.02026,73.06307)
  -- (214.05028,73.19308)
  -- (214.13026,73.01307)
  -- (214.19028,73.04307)
  -- (214.21028,72.98309)
  -- (214.27028,73.11308)
  -- (214.30028,73.02308)
  -- (214.35028,73.14309)
  -- (214.38028,73.02308)
  -- (214.55028,73.12309)
  -- (214.92027,73.07310)
  -- (215.25027,72.93307)
  -- (215.37027,73.01307)
  -- (215.59027,72.96310)
  -- (215.79027,73.04307)
  -- (216.07028,73.00309)
  -- (217.98029,73.22308)
  -- (219.77028,73.19308)
  -- (222.10030,73.05310)
  -- (224.10030,73.08308)
  -- (225.61029,73.01307)
  -- (226.40027,73.05310)
  -- (227.80031,72.87309)
  -- (227.83029,72.98309)
  -- (227.89029,72.91308)
  -- (228.06029,73.12309)
  -- (228.14029,73.03309)
  -- (228.17029,73.09309)
  -- (228.22029,73.03309)
  -- (228.25029,73.11308)
  -- (228.34029,73.13308)
  -- (228.42029,73.05310)
  -- (228.59029,73.11308)
  -- (228.73029,73.07310)
  -- (228.84029,73.13308)
  -- (229.12029,73.06307)
  -- (229.32030,73.10308)
  -- (229.35030,73.04307)
  -- (229.57030,73.13308)
  -- (229.63030,73.04307)
  -- (229.66030,73.10308)
  -- (229.77030,73.01307)
  -- (229.80031,73.07310)
  -- (229.83029,73.01307)
  -- (229.97029,73.10308)
  -- (229.99030,73.04307)
  -- (230.05030,73.12309)
  -- (230.61029,72.88308)
  -- (230.95029,73.21308)
  -- (231.00030,75.12309)
  -- (231.06029,72.95307)
  -- (231.09030,73.13308)
  -- (231.15028,72.59307)
  -- (231.20029,73.27310)
  -- (231.29030,72.81307)
  -- (231.34030,72.99308)
  -- (231.37029,72.68307)
  -- (231.40028,73.17307)
  -- (231.43028,72.96310)
  -- (231.48029,73.15307)
  -- (231.57030,73.10308)
  -- (231.62029,73.23309)
  -- (231.65030,72.74310)
  -- (231.68028,73.16310)
  -- (231.71030,73.04307)
  -- (231.76030,73.14309)
  -- (231.85031,72.99308)
  -- (231.93028,73.03309)
  -- (231.99030,72.94310)
  -- (232.02030,73.03309)
  -- (232.04028,72.95307)
  -- (232.10030,72.96310)
  -- (232.13030,73.07310)
  -- (232.16031,72.89309)
  -- (232.18030,73.17307)
  -- (232.21030,73.04307)
  -- (232.27031,73.04307)
  -- (232.30030,73.21308)
  -- (232.35030,72.74310)
  -- (232.38031,72.96310)
  -- (232.52031,73.17307)
  -- (232.61029,73.06307)
  -- (232.63031,73.11308)
  -- (232.80031,72.82308)
  -- (232.94030,73.13308)
  -- (233.00030,73.00309)
  -- (233.08029,72.98309)
  -- (233.17029,73.07310)
  -- (233.22029,73.03309)
  -- (233.25030,73.12309)
  -- (233.36030,73.02308)
  -- (233.45030,73.06307)
  -- (233.64029,72.99308)
  -- (233.76030,73.03309)
  -- (234.01030,72.92309)
  -- (235.44029,72.99308)
  -- (235.47030,72.91308)
  -- (235.53029,72.93307)
  -- (235.69030,72.84307)
  -- (235.81030,72.88308)
  -- (236.23030,72.78309)
  -- (236.48030,72.78309)
  -- (236.54030,76.77310)
  -- (236.59030,71.73307)
  -- (236.70030,73.35308)
  -- (236.76030,72.76309)
  -- (236.79030,73.15307)
  -- (236.84030,72.77308)
  -- (236.90030,73.14309)
  -- (236.93028,72.84307)
  -- (237.04030,72.98309)
  -- (237.15030,72.88308)
  -- (237.35031,73.03309)
  -- (237.43030,73.01307)
  -- (237.46031,73.08308)
  -- (237.49031,73.00309)
  -- (237.52031,73.17307)
  -- (237.55031,72.93307)
  -- (237.66031,72.97308)
  -- (237.72030,73.09309)
  -- (237.77031,73.05310)
  -- (237.80031,73.09309)
  -- (238.16031,72.89309)
  -- (238.78030,73.13308)
  -- (239.15030,73.09309)
  -- (239.20030,73.14309)
  -- (239.26030,73.06307)
  -- (239.29030,73.12309)
  -- (239.34030,73.06307)
  -- (239.85031,73.08308)
  -- (240.05031,73.03309)
  -- (240.35031,73.13308)
  -- (240.92030,73.17307)
  -- (244.29031,73.12309)
  -- (245.46031,73.16310)
  -- (247.79031,73.10308)
  -- (248.24033,72.95307)
  -- (249.25032,72.84307)
  -- (249.54031,73.09309)
  -- (249.62032,73.09309)
  -- (249.73032,72.95307)
  -- (249.76031,73.02308)
  -- (249.82033,72.95307)
  -- (250.38033,72.85310)
  -- (251.08032,73.07310)
  -- (251.25032,72.96310)
  -- (251.59032,72.95307)
  -- (251.81032,72.87309)
  -- (251.84032,72.79307)
  -- (251.89034,73.02308)
  -- (251.98033,72.91308)
  -- (252.03032,73.03309)
  -- (252.12032,72.93307)
  -- (252.32033,72.99308)
  -- (252.34032,72.88308)
  -- (252.37032,73.02308)
  -- (252.46033,72.84307)
  -- (252.48032,73.09309)
  -- (252.51031,72.78309)
  -- (252.57033,73.00309)
  -- (252.62032,72.94310)
  -- (252.76033,73.10308)
  -- (252.85033,73.06307)
  -- (252.91032,73.12309)
  -- (252.96034,72.93307)
  -- (253.02032,73.15307)
  -- (253.05032,73.06307)
  -- (253.35033,73.14309)
  -- (253.38034,73.02308)
  -- (253.41032,73.12309)
  -- (253.69034,72.97308)
  -- (253.78033,73.03309)
  -- (253.80034,72.90307)
  -- (253.86032,73.06307)
  -- (253.89034,72.98309)
  -- (254.03032,73.01307)
  -- (254.14034,73.04307)
  -- (254.17032,73.13308)
  -- (254.20032,72.92309)
  -- (254.25034,73.07310)
  -- (254.28032,72.98309)
  -- (254.37032,73.88308)
  -- (254.48032,72.56309)
  -- (254.62032,73.19308)
  -- (254.79031,72.93307)
  -- (254.87033,73.05310)
  -- (254.95032,72.98309)
  -- (255.01031,73.19308)
  -- (255.04031,72.27310)
  -- (255.07034,73.48307)
  -- (255.10033,72.95307)
  -- (255.18033,73.08308)
  -- (255.21033,72.88308)
  -- (255.35033,73.10308)
  -- (255.49034,72.92309)
  -- (255.54033,73.01307)
  -- (255.66032,72.94310)
  -- (255.68031,73.10308)
  -- (255.71033,72.48307)
  -- (255.74034,73.45309)
  -- (255.77032,72.78309)
  -- (255.80034,73.07310)
  -- (255.85034,72.93307)
  -- (256.08032,73.16310)
  -- (256.13033,73.03309)
  -- (256.22032,73.11308)
  -- (256.25034,72.58310)
  -- (256.27034,73.50308)
  -- (256.30034,73.01307)
  -- (256.33032,73.13308)
  -- (256.41034,72.87309)
  -- (256.56033,73.04307)
  -- (256.67033,72.99308)
  -- (256.78033,72.70307)
  -- (256.84032,72.87309)
  -- (256.86032,72.52308)
  -- (256.89034,73.14309)
  -- (256.92033,72.97308)
  -- (256.95032,73.06307)
  -- (256.98033,73.01307)
  -- (257.09033,72.71308)
  -- (257.20032,72.90307)
  -- (257.34033,72.74310)
  -- (257.48033,72.82308)
  -- (257.51031,72.78309)
  -- (257.54033,72.86308)
  -- (257.62032,72.76309)
  -- (257.68033,72.83310)
  -- (257.85034,72.79307)
  -- (257.99034,73.01307)
  -- (258.02032,72.91308)
  -- (258.04031,73.03309)
  -- (258.07034,72.92309)
  -- (258.10034,73.21308)
  -- (258.13033,72.88308)
  -- (258.16034,73.22308)
  -- (258.18033,72.92309)
  -- (258.24033,73.04307)
  -- (258.27034,72.86308)
  -- (258.30034,72.95307)
  -- (258.35033,72.86308)
  -- (258.46034,72.85310)
  -- (258.77034,72.97308)
  -- (259.05034,72.93307)
  -- (259.22032,73.00309)
  -- (259.42032,72.89309)
  -- (259.45033,72.94310)
  -- (259.50034,72.91308)
  -- (259.53032,72.99308)
  -- (259.56033,72.92309)
  -- (259.62032,73.04307)
  -- (259.64034,72.94310)
  -- (259.67033,73.04307)
  -- (259.76033,73.07310)
  -- (259.84033,73.01307)
  -- (259.87033,73.06307)
  -- (259.90033,72.99308)
  -- (259.95033,73.12309)
  -- (259.98033,73.03309)
  -- (260.26033,73.07310)
  -- (260.68033,72.96310)
  -- (261.10034,72.76309)
  -- (261.22034,72.79307)
  -- (261.44034,73.16310)
  -- (261.75034,72.81307)
  -- (261.78033,73.28308)
  -- (261.83034,72.70307)
  -- (261.92033,72.85310)
  -- (261.97034,72.76309)
  -- (262.03033,72.87309)
  -- (262.09033,72.80310)
  -- (262.23033,72.94310)
  -- (262.28033,72.78309)
  -- (262.34033,72.87309)
  -- (262.40033,72.82308)
  -- (262.62033,73.16310)
  -- (262.65033,72.95307)
  -- (262.68033,73.23309)
  -- (262.70033,72.91308)
  -- (262.73033,73.11308)
  -- (262.76033,72.91308)
  -- (262.79033,73.03309)
  -- (262.82034,72.96310)
  -- (262.87033,73.03309)
  -- (262.90033,72.96310)
  -- (263.04033,73.08308)
  -- (263.21034,73.03309)
  -- (263.46034,73.20307)
  -- (263.63034,73.19308)
  -- (264.28033,72.87309)
  -- (265.09035,72.80310)
  -- (266.35034,73.05310)
  -- (266.58035,72.99308)
  -- (266.61034,73.06307)
  -- (266.69035,73.02308)
  -- (266.72035,73.10308)
  -- (266.78035,73.01307)
  -- (266.92035,73.04307)
  -- (266.94035,72.99308)
  -- (266.97034,73.03309)
  -- (267.06033,72.99308)
  -- (267.08034,73.05310)
  -- (267.11034,72.99308)
  -- (267.17033,73.08308)
  -- (267.20033,73.00309)
  -- (267.28033,72.99308)
  -- (267.31033,73.07310)
  -- (267.36035,72.96310)
  -- (267.48033,73.04307)
  -- (268.01035,72.94310)
  -- (268.99036,73.09309)
  -- (269.92035,73.14309)
  -- (270.73033,73.07310)
  -- (275.68034,73.08308)
  -- (278.01035,73.03309)
  -- (281.57037,73.11308)
  -- (283.79036,73.04307)
  -- (284.10037,72.98309)
  -- (285.19037,73.02308)
  -- (285.22037,72.93307)
  -- (285.31036,72.92309)
  -- (287.02037,73.10308)
  -- (287.66037,73.10308)
  -- (288.56038,72.99308)
  -- (292.19038,73.04307)
  -- (292.92038,72.89309)
  -- (293.59038,73.09309)
  -- (293.90038,72.97308)
  -- (294.63039,72.97308)
  -- (294.88039,72.89309)
  -- (295.53038,73.00309)
  -- (296.37038,72.96310)
  -- (297.21039,73.00309)
  -- (297.30038,73.58310)
  -- (297.38040,72.98309)
  -- (297.49040,72.88308)
  -- (297.72038,73.01307)
  -- (298.03038,72.99308)
  -- (298.08038,73.04307)
  -- (298.36040,72.97308)
  -- (300.33038,72.98309)
  -- (301.98040,73.10308)
  -- (303.64038,73.06307)
  -- (305.19040,73.18308)
  -- (311.05042,73.14309)
  -- (315.24040,73.03309)
  -- (331.47043,73.02308)
  -- (331.89044,73.07310)
  -- (333.94044,73.00309)
  -- (338.09044,73.04307)
  -- (346.35045,73.00309)
  -- (348.99046,73.03309)
  -- (349.04044,73.13308)
  -- (349.07047,73.03309)
  -- (349.10046,73.10308)
  -- (349.21046,73.02308)
  -- (354.57047,73.02308)
  -- (354.94046,73.05310)
  -- (354.99046,73.18308)
  -- (355.02046,73.08308)
  -- (355.05046,73.15307)
  -- (355.22046,73.00309)
  -- (355.39046,73.05310)
  -- (358.48045,72.99308)
  -- (358.59045,73.01307)
  -- (358.70047,73.19308)
  -- (358.79045,73.02308)
  -- (358.87047,73.01307)
  -- (359.07048,73.09309)
  -- (361.51045,73.04307)
  -- (361.56047,73.11308)
  -- (361.68047,73.02308)
  -- (361.79047,73.07310)
  -- (366.70047,73.06307)
  -- (366.84047,73.12309)
  -- (366.98048,73.08308)
  -- (368.16049,73.18308)
  -- (368.67049,73.14309)
  -- (368.72047,73.22308)
  -- (368.78049,73.09309)
  -- (368.81047,73.18308)
  -- (369.15047,73.15307)
  -- (369.59047,73.23309)
  -- (369.74050,73.20307)
  -- (370.10050,73.31307)
  -- (370.30049,73.27310)
  -- (370.33047,73.34309)
  -- (370.41049,73.26307)
  -- (370.44048,73.33308)
  -- (370.55048,73.27310)
  -- (370.63050,73.36309)
  -- (370.72049,73.25309)
  -- (370.83049,73.38310)
  -- (370.86047,73.27310)
  -- (370.94049,73.35308)
  -- (371.14049,73.25309)
  -- (371.20047,73.33308)
  -- (371.39049,73.26307)
  -- (371.42047,73.33308)
  -- (371.59048,73.27310)
  -- (371.62047,73.33308)
  -- (371.70049,73.26307)
  -- (371.73047,73.32310)
  -- (371.84047,73.27310)
  -- (372.04047,73.34309)
  -- (372.07050,73.28308)
  -- (372.09048,73.34309)
  -- (372.23048,73.28308)
  -- (372.43048,73.33308)
  -- (372.52050,73.28308)
  -- (372.63050,73.35308)
  -- (372.66049,73.29308)
  -- (372.68048,73.36309)
  -- (373.02048,73.38310)
  -- (373.13048,73.31307)
  -- (373.25049,73.39308)
  -- (373.27050,73.32310)
  -- (373.39049,73.39308)
  -- (374.62048,73.30308)
  -- (375.27050,73.36309)
  -- (375.83049,73.34309)
  -- (376.02050,73.44308)
  -- (376.14049,73.34309)
  -- (376.17049,73.40307)
  -- (376.33049,73.33308)
  -- (379.34050,73.36309)
  -- (379.37048,73.32310)
  -- (379.48048,73.35308)
  -- (379.51048,73.29308)
  -- (379.53049,73.38310)
  -- (379.62048,73.30308)
  -- (379.67050,73.36309)
  -- (379.76050,73.32310)
  -- (380.15048,73.36309)
  -- (380.24050,73.31307)
  -- (380.26048,73.36309)
  -- (380.43050,73.32310)
  -- (380.46050,73.36309)
  -- (384.05050,73.32310)
  -- (384.08050,73.48307)
  -- (384.11049,73.22308)
  -- (384.14050,73.39308)
  -- (384.20049,73.23309)
  -- (384.22049,73.44308)
  -- (384.25050,73.30308)
  -- (384.28050,73.34309)
  -- (384.34050,73.29308)
  -- (384.42049,73.39308)
  -- (384.50050,73.32310)
  -- (384.56050,73.37307)
  -- (384.67050,73.32310)
  -- (386.58050,73.32310)
  -- (386.61050,73.37307)
  -- (387.00050,73.32310)
  -- (387.20050,73.36309)
  -- (387.31050,73.31307)
  -- (387.34050,73.37307)
  -- (387.40050,73.31307)
  -- (388.18050,73.37307)
  -- (388.29051,73.30308)
  -- (388.49052,73.36309)
  -- (388.55050,73.32310)
  -- (388.58052,73.38310)
  -- (388.77051,73.30308)
  -- (389.50050,73.37307)
  -- (390.88051,73.35308);
% Reference trace 21
\path[draw={rgb,1:red,0.082;green,0.374;blue,0.391},line width=0.32877bp] (110.44012,71.72308)
  -- (114.93013,71.70307)
  -- (115.10014,71.74310)
  -- (115.30014,71.68307)
  -- (115.49016,71.74310)
  -- (115.75014,71.69310)
  -- (115.97014,71.73307)
  -- (120.66014,71.68307)
  -- (120.94016,71.77308)
  -- (121.14015,71.65309)
  -- (121.33014,71.79307)
  -- (121.59015,71.64308)
  -- (121.78015,71.75308)
  -- (121.98015,71.67309)
  -- (122.18015,71.75308)
  -- (122.37015,71.70307)
  -- (122.85016,71.74310)
  -- (124.84015,71.69310)
  -- (124.98015,71.75308)
  -- (125.66016,71.68307)
  -- (125.77016,71.73307)
  -- (127.62015,71.74310)
  -- (129.28015,71.69310)
  -- (130.01015,71.76309)
  -- (130.29016,71.70307)
  -- (130.66016,71.78309)
  -- (130.77016,71.77308)
  -- (130.91016,71.65309)
  -- (131.11015,71.75308)
  -- (132.00017,71.69310)
  -- (132.20015,71.74310)
  -- (132.37015,71.68307)
  -- (132.57016,71.73307)
  -- (135.01016,71.70307)
  -- (135.37016,71.42307)
  -- (135.51015,71.43307)
  -- (135.57018,71.34307)
  -- (135.88017,71.55308)
  -- (136.10017,72.09309)
  -- (136.47017,72.30308)
  -- (136.64017,72.26307)
  -- (137.20016,71.76309)
  -- (137.23016,71.79307)
  -- (137.28017,71.69310)
  -- (137.34016,71.76309)
  -- (137.48016,71.68307)
  -- (137.84016,72.14309)
  -- (138.07018,72.59307)
  -- (138.57018,73.06307)
  -- (138.85017,73.08308)
  -- (138.99017,73.02308)
  -- (139.25017,73.09309)
  -- (139.30017,73.03309)
  -- (139.50017,73.15307)
  -- (139.64017,73.41308)
  -- (139.95016,73.41308)
  -- (140.17017,73.52310)
  -- (140.74019,73.37307)
  -- (141.10017,72.90307)
  -- (141.41017,72.85310)
  -- (141.58018,72.92309)
  -- (142.11017,72.98309)
  -- (142.34018,72.92309)
  -- (142.76018,72.97308)
  -- (143.26016,73.12309)
  -- (144.08018,73.23309)
  -- (144.67018,73.03309)
  -- (144.98018,73.01307)
  -- (145.59018,73.15307)
  -- (146.60019,73.11308)
  -- (147.39018,73.00309)
  -- (148.20018,73.11308)
  -- (148.32019,73.18308)
  -- (148.63019,73.11308)
  -- (148.79018,73.18308)
  -- (148.85019,73.52310)
  -- (149.07019,73.12309)
  -- (149.66019,73.19308)
  -- (150.09020,73.06307)
  -- (150.45018,73.13308)
  -- (150.62018,73.08308)
  -- (150.76020,73.14309)
  -- (150.79018,73.08308)
  -- (150.84018,73.21308)
  -- (150.90018,73.14309)
  -- (151.07020,73.14309)
  -- (151.12018,73.05310)
  -- (151.26018,73.11308)
  -- (151.29019,73.22308)
  -- (151.35019,73.10308)
  -- (151.38020,73.17307)
  -- (151.49020,73.06307)
  -- (151.52019,73.12309)
  -- (151.55019,73.04307)
  -- (151.60020,73.20307)
  -- (151.63019,73.04307)
  -- (151.71019,73.16310)
  -- (151.77019,73.00309)
  -- (151.83018,73.17307)
  -- (151.85020,73.03309)
  -- (151.94020,73.11308)
  -- (151.97018,73.04307)
  -- (151.99019,73.21308)
  -- (152.02019,73.03309)
  -- (152.08018,73.16310)
  -- (152.14020,73.06307)
  -- (152.16020,73.20307)
  -- (152.22018,73.04307)
  -- (152.25020,73.28308)
  -- (152.30019,73.06307)
  -- (152.39018,73.22308)
  -- (152.50018,73.14309)
  -- (152.75018,73.11308)
  -- (152.95018,73.23309)
  -- (153.01018,73.16310)
  -- (153.26018,73.19308)
  -- (153.34020,73.08308)
  -- (153.51018,73.14309)
  -- (153.79018,72.89309)
  -- (153.85020,73.01307)
  -- (154.10020,72.97308)
  -- (154.27020,73.25309)
  -- (154.35019,74.13308)
  -- (154.41020,72.63310)
  -- (154.58020,73.53308)
  -- (154.75018,73.05310)
  -- (154.91019,73.27310)
  -- (155.00020,73.29308)
  -- (155.06018,72.91308)
  -- (155.17018,73.36309)
  -- (155.31018,73.01307)
  -- (155.50020,73.12309)
  -- (156.40018,73.15307)
  -- (156.49020,73.24308)
  -- (156.74020,73.18308)
  -- (157.05020,73.32310)
  -- (157.13019,73.24308)
  -- (157.19020,73.28308)
  -- (157.39020,73.22308)
  -- (157.58020,73.29308)
  -- (157.95020,73.19308)
  -- (158.14020,73.28308)
  -- (158.37020,73.16310)
  -- (158.59020,73.24308)
  -- (159.15019,73.21308)
  -- (159.29019,73.30308)
  -- (159.44020,73.09309)
  -- (159.63020,73.29308)
  -- (159.83020,73.20307)
  -- (160.67020,73.25309)
  -- (160.87020,73.18308)
  -- (161.09021,73.23309)
  -- (161.65019,73.21308)
  -- (161.71020,73.01307)
  -- (161.82020,73.50308)
  -- (161.99020,73.07310)
  -- (162.21020,73.31307)
  -- (162.55020,73.21308)
  -- (162.75020,73.29308)
  -- (162.94022,73.21308)
  -- (163.06020,73.38310)
  -- (163.17020,73.41308)
  -- (163.31020,73.11308)
  -- (163.34021,73.23309)
  -- (163.39020,73.20307)
  -- (163.45021,73.34309)
  -- (163.51020,73.30308)
  -- (163.56021,73.38310)
  -- (163.82020,73.30308)
  -- (163.87021,73.21308)
  -- (164.01020,73.28308)
  -- (164.21020,73.18308)
  -- (164.35020,73.29308)
  -- (164.49022,73.26307)
  -- (164.60022,73.36309)
  -- (164.63022,73.32310)
  -- (164.69022,73.36309)
  -- (165.19020,73.03309)
  -- (165.81021,72.92309)
  -- (166.23021,72.56309)
  -- (166.68020,72.34309)
  -- (167.04019,72.40307)
  -- (167.35020,72.62307)
  -- (168.36021,72.80310)
  -- (168.73020,72.62307)
  -- (169.23021,72.52308)
  -- (169.66022,72.92309)
  -- (170.13022,73.08308)
  -- (170.89021,72.85310)
  -- (172.15020,73.00309)
  -- (172.91022,72.87309)
  -- (173.28021,72.88308)
  -- (173.53021,72.96310)
  -- (173.64021,73.40307)
  -- (173.87022,72.76309)
  -- (174.34023,73.07310)
  -- (174.48021,72.90307)
  -- (174.77022,72.89309)
  -- (175.02022,72.99308)
  -- (175.66022,72.95307)
  -- (175.94023,72.84307)
  -- (176.65022,72.73307)
  -- (177.29022,72.90307)
  -- (177.49023,72.88308)
  -- (177.55022,72.97308)
  -- (177.60023,72.94310)
  -- (177.83023,73.07310)
  -- (177.94023,73.27310)
  -- (178.11021,72.84307)
  -- (178.36023,72.80310)
  -- (178.72023,72.85310)
  -- (178.95021,72.80310)
  -- (179.37022,72.88308)
  -- (179.51021,73.00309)
  -- (179.79022,72.75308)
  -- (180.02022,72.92309)
  -- (180.27023,72.82308)
  -- (180.77023,72.90307)
  -- (181.14023,72.79307)
  -- (181.50023,72.97308)
  -- (181.73022,72.75308)
  -- (181.98022,72.97308)
  -- (182.12022,72.82308)
  -- (182.29022,72.95307)
  -- (182.51022,72.89309)
  -- (182.68022,72.94310)
  -- (183.47023,72.84307)
  -- (183.61023,72.95307)
  -- (183.81023,72.87309)
  -- (183.97023,72.92309)
  -- (184.68022,72.85310)
  -- (184.85023,72.91308)
  -- (187.96025,72.88308)
  -- (189.67024,72.93307)
  -- (190.94025,72.93307)
  -- (191.42023,72.87309)
  -- (191.81024,72.95307)
  -- (191.95024,72.89309)
  -- (192.12024,72.95307)
  -- (192.26024,72.92309)
  -- (192.43024,72.99308)
  -- (193.21025,72.87309)
  -- (194.42024,72.89309)
  -- (194.59024,72.94310)
  -- (194.73024,72.86308)
  -- (194.87024,72.93307)
  -- (196.02025,72.92309)
  -- (196.08025,73.32310)
  -- (196.13025,72.99308)
  -- (196.16026,73.04307)
  -- (196.22025,73.01307)
  -- (196.27026,73.17307)
  -- (196.30025,73.14309)
  -- (196.41025,72.69310)
  -- (196.47026,73.11308)
  -- (196.53024,73.06307)
  -- (196.58026,73.14309)
  -- (196.92024,72.83310)
  -- (197.34026,72.81307)
  -- (198.01024,72.08308)
  -- (198.32027,72.15307)
  -- (198.74026,72.45309)
  -- (199.28024,72.71308)
  -- (199.36026,73.54308)
  -- (199.47026,72.92309)
  -- (199.50026,73.01307)
  -- (199.70026,72.34309)
  -- (199.87025,72.75308)
  -- (199.95024,72.75308)
  -- (200.12025,72.48307)
  -- (200.37024,72.78309)
  -- (200.54025,72.59307)
  -- (200.71025,72.76309)
  -- (200.82025,72.70307)
  -- (201.05026,73.12309)
  -- (201.27026,72.19308)
  -- (201.33025,72.21308)
  -- (201.35025,72.03308)
  -- (201.41026,72.15307)
  -- (201.44025,71.99308)
  -- (201.50026,72.15307)
  -- (201.52026,72.04307)
  -- (201.55025,72.09309)
  -- (201.58026,72.26307)
  -- (201.64024,72.21308)
  -- (201.66026,72.34309)
  -- (201.72026,72.26307)
  -- (201.75024,72.36309)
  -- (201.80026,72.25309)
  -- (201.83026,72.33308)
  -- (201.89026,72.25309)
  -- (201.92026,72.34309)
  -- (201.97026,72.26307)
  -- (202.31024,72.65309)
  -- (202.37025,74.12309)
  -- (202.48026,72.67309)
  -- (202.53024,72.67309)
  -- (202.62024,72.99308)
  -- (202.76025,72.56309)
  -- (202.93024,72.60310)
  -- (203.04025,72.52308)
  -- (203.29025,72.57308)
  -- (203.52026,72.49310)
  -- (203.69026,72.59307)
  -- (203.77026,72.60310)
  -- (203.83026,72.51307)
  -- (204.08026,72.65309)
  -- (204.13026,72.56309)
  -- (204.39026,72.64308)
  -- (204.81026,72.45309)
  -- (205.15025,72.63310)
  -- (205.20026,72.51307)
  -- (205.26025,72.61308)
  -- (205.31026,72.43308)
  -- (205.45026,72.61308)
  -- (205.54025,72.44308)
  -- (205.73026,72.71308)
  -- (205.82027,72.50308)
  -- (205.85027,72.58310)
  -- (205.93025,72.44308)
  -- (206.13026,72.70307)
  -- (206.21027,72.54308)
  -- (206.38028,72.80310)
  -- (206.44026,72.63310)
  -- (206.52026,72.75308)
  -- (206.55026,72.71308)
  -- (206.58028,72.82308)
  -- (206.75026,72.56309)
  -- (206.83026,72.86308)
  -- (207.05026,72.63310)
  -- (207.14026,72.74310)
  -- (207.17026,72.63310)
  -- (207.22026,72.79307)
  -- (207.31026,72.66308)
  -- (207.39026,72.84307)
  -- (207.50026,72.60310)
  -- (207.56027,72.81307)
  -- (207.62025,72.76309)
  -- (207.67027,72.83310)
  -- (207.73026,72.66308)
  -- (207.81026,72.96310)
  -- (207.84026,72.89309)
  -- (207.90025,72.91308)
  -- (207.98027,72.66308)
  -- (208.01025,72.72308)
  -- (208.07028,72.69310)
  -- (208.21027,72.88308)
  -- (208.26025,73.15307)
  -- (208.32027,72.97308)
  -- (208.37025,73.09309)
  -- (208.43025,73.03309)
  -- (208.68025,73.38310)
  -- (208.88026,72.90307)
  -- (208.94028,72.90307)
  -- (208.99026,72.28308)
  -- (209.02026,72.58310)
  -- (209.08026,72.09309)
  -- (209.10027,72.42307)
  -- (209.16028,72.00309)
  -- (209.19026,72.30308)
  -- (209.24026,71.99308)
  -- (209.30026,72.25309)
  -- (209.33026,72.01307)
  -- (209.39026,72.19308)
  -- (209.44026,72.00309)
  -- (209.47028,72.08308)
  -- (209.53026,71.86308)
  -- (209.55026,71.94310)
  -- (209.61026,71.84307)
  -- (209.95026,72.36309)
  -- (210.00027,73.80310)
  -- (210.11026,72.23307)
  -- (210.23027,72.82308)
  -- (210.31026,72.55308)
  -- (210.37025,72.62307)
  -- (210.51025,72.28308)
  -- (210.59026,72.36309)
  -- (210.73026,72.32308)
  -- (211.04025,72.46308)
  -- (211.13026,72.43308)
  -- (211.18027,72.50308)
  -- (211.21028,72.44308)
  -- (211.27028,72.53308)
  -- (211.29027,72.47310)
  -- (211.38028,72.47310)
  -- (211.43027,72.57308)
  -- (211.60028,72.38310)
  -- (211.86026,74.08308)
  -- (211.94028,71.34307)
  -- (212.02026,72.65309)
  -- (212.08028,72.37307)
  -- (212.22026,72.91308)
  -- (212.33026,72.64308)
  -- (212.39027,72.70307)
  -- (212.45027,72.62307)
  -- (212.70027,72.55308)
  -- (212.78027,72.63310)
  -- (212.87027,72.52308)
  -- (212.98027,72.66308)
  -- (213.15025,72.65309)
  -- (213.20026,72.79307)
  -- (213.43027,72.58310)
  -- (213.54027,72.33308)
  -- (213.71027,73.03309)
  -- (213.85028,72.62307)
  -- (213.91026,72.68307)
  -- (213.93025,72.56309)
  -- (213.99028,72.91308)
  -- (214.13026,72.67309)
  -- (214.33026,72.91308)
  -- (214.44028,72.71308)
  -- (214.50027,72.79307)
  -- (214.58028,72.75308)
  -- (214.83028,72.85310)
  -- (215.14027,72.85310)
  -- (215.45027,72.65309)
  -- (215.73027,72.33308)
  -- (215.96028,72.28308)
  -- (216.35028,72.05310)
  -- (217.33028,72.45309)
  -- (217.95027,72.38310)
  -- (218.40027,72.50308)
  -- (219.02028,72.45309)
  -- (219.27030,72.36309)
  -- (219.44028,72.40307)
  -- (219.46028,72.34309)
  -- (219.61028,72.40307)
  -- (219.63028,72.35308)
  -- (219.69029,72.42307)
  -- (219.83028,72.32308)
  -- (220.25029,72.40307)
  -- (221.51027,72.37307)
  -- (222.10030,72.50308)
  -- (223.23029,72.57308)
  -- (223.93027,72.41308)
  -- (224.49030,72.48307)
  -- (225.00029,72.36309)
  -- (225.47029,72.49310)
  -- (226.18028,72.49310)
  -- (226.85030,72.62307)
  -- (227.44029,72.33308)
  -- (227.80031,72.45309)
  -- (227.89029,73.42307)
  -- (228.06029,72.01307)
  -- (228.11029,72.05310)
  -- (228.14029,71.94310)
  -- (228.31029,73.14309)
  -- (228.51028,72.37307)
  -- (228.59029,72.42307)
  -- (228.67029,72.32308)
  -- (228.87029,72.52308)
  -- (229.10030,72.44308)
  -- (229.18030,72.35308)
  -- (229.32030,72.49310)
  -- (229.40028,72.36309)
  -- (229.60031,72.57308)
  -- (229.66030,72.47310)
  -- (229.69030,72.52308)
  -- (229.74030,72.45309)
  -- (229.80031,72.48307)
  -- (229.85030,72.38310)
  -- (229.91030,72.44308)
  -- (229.94029,72.38310)
  -- (229.99030,72.42307)
  -- (230.05030,72.28308)
  -- (230.11029,72.34309)
  -- (230.25029,72.15307)
  -- (230.81029,72.87309)
  -- (230.86029,72.83310)
  -- (230.89030,72.88308)
  -- (230.95029,72.79307)
  -- (231.03029,73.47310)
  -- (231.09030,71.59307)
  -- (231.20029,72.53308)
  -- (231.34030,72.99308)
  -- (231.54030,72.21308)
  -- (231.65030,72.75308)
  -- (231.82030,72.41308)
  -- (231.99030,72.77308)
  -- (232.04028,72.65309)
  -- (232.13030,72.70307)
  -- (232.24030,72.54308)
  -- (232.32031,72.63310)
  -- (232.38031,72.87309)
  -- (232.44029,72.46308)
  -- (232.49031,72.49310)
  -- (232.58030,72.80310)
  -- (232.61029,72.70307)
  -- (232.72030,73.22308)
  -- (232.83030,72.72308)
  -- (232.91030,72.94310)
  -- (233.14030,72.60310)
  -- (233.22029,72.73307)
  -- (233.28029,72.64308)
  -- (233.45030,72.74310)
  -- (233.59029,72.66308)
  -- (234.07031,72.89309)
  -- (234.21031,72.81307)
  -- (234.57030,72.81307)
  -- (234.82030,72.73307)
  -- (235.47030,72.07310)
  -- (235.58030,72.33308)
  -- (235.64029,72.21308)
  -- (235.72030,72.39308)
  -- (235.92030,72.49310)
  -- (236.28030,72.28308)
  -- (236.42029,72.59307)
  -- (236.45030,72.53308)
  -- (236.54030,77.14309)
  -- (236.65030,70.17307)
  -- (236.84030,73.30308)
  -- (237.04030,72.52308)
  -- (237.13030,72.41308)
  -- (237.27031,73.12309)
  -- (237.49031,72.61308)
  -- (237.55031,73.16310)
  -- (237.60031,72.98309)
  -- (237.66031,73.15307)
  -- (237.72030,73.08308)
  -- (237.74031,73.14309)
  -- (237.80031,73.03309)
  -- (237.88031,73.12309)
  -- (238.05031,73.05310)
  -- (238.98030,72.22308)
  -- (239.23030,72.19308)
  -- (240.02031,72.30308)
  -- (240.38033,72.16310)
  -- (240.72030,72.19308)
  -- (241.20030,72.37307)
  -- (241.53030,72.42307)
  -- (242.74033,72.42307)
  -- (243.53030,72.52308)
  -- (245.55031,72.39308)
  -- (246.90031,72.53308)
  -- (247.26031,72.32308)
  -- (247.79031,72.23307)
  -- (248.52032,72.38310)
  -- (249.25032,72.87309)
  -- (249.31030,73.92309)
  -- (249.34032,73.49310)
  -- (249.40030,73.90307)
  -- (249.65031,72.26307)
  -- (249.76031,72.37307)
  -- (249.99033,72.86308)
  -- (250.15031,72.64308)
  -- (250.35033,72.84307)
  -- (250.46033,72.76309)
  -- (250.55032,72.78309)
  -- (250.94032,72.32308)
  -- (251.22032,72.41308)
  -- (251.47032,72.37307)
  -- (251.75032,72.51307)
  -- (251.84032,72.66308)
  -- (251.92032,73.67309)
  -- (252.23032,72.25309)
  -- (252.37032,72.31307)
  -- (252.46033,72.22308)
  -- (252.54031,72.46308)
  -- (252.60034,73.25309)
  -- (252.68031,72.98309)
  -- (252.71033,73.07310)
  -- (252.74033,73.02308)
  -- (253.02032,72.10308)
  -- (253.27034,72.71308)
  -- (253.33032,72.58310)
  -- (253.38034,72.64308)
  -- (253.44032,72.39308)
  -- (253.69034,72.55308)
  -- (253.83032,72.53308)
  -- (253.86032,72.43308)
  -- (253.92032,72.53308)
  -- (254.17032,72.45309)
  -- (254.25034,72.01307)
  -- (254.37032,72.82308)
  -- (254.42032,72.20307)
  -- (254.51031,72.60310)
  -- (254.56033,72.36309)
  -- (254.65033,72.69310)
  -- (254.70032,72.40307)
  -- (254.84032,72.64308)
  -- (254.93031,72.48307)
  -- (255.07034,72.76309)
  -- (255.12033,72.59307)
  -- (255.18033,72.70307)
  -- (255.26031,72.49310)
  -- (255.40031,72.74310)
  -- (255.46033,72.66308)
  -- (255.66032,72.70307)
  -- (255.74034,73.15307)
  -- (255.99033,72.58310)
  -- (256.11032,72.61308)
  -- (256.19032,72.49310)
  -- (256.22032,72.67309)
  -- (256.30034,72.53308)
  -- (256.50034,72.74310)
  -- (256.56033,72.55308)
  -- (256.64032,72.65309)
  -- (256.75032,73.37307)
  -- (256.84032,72.34309)
  -- (257.03033,73.23309)
  -- (257.14034,72.45309)
  -- (257.29033,73.25309)
  -- (257.40031,72.75308)
  -- (257.54033,73.28308)
  -- (257.65033,73.00309)
  -- (257.79033,73.34309)
  -- (257.93031,73.09309)
  -- (258.04031,73.25309)
  -- (258.10034,73.07310)
  -- (258.16034,73.44308)
  -- (258.21034,72.53308)
  -- (258.27034,72.86308)
  -- (258.35033,72.67309)
  -- (258.44032,72.66308)
  -- (258.52034,72.76309)
  -- (258.69034,72.57308)
  -- (258.77034,72.67309)
  -- (258.86034,72.60310)
  -- (259.00034,72.72308)
  -- (259.11032,72.62307)
  -- (259.39034,72.75308)
  -- (259.76033,72.38310)
  -- (259.78033,72.26307)
  -- (259.98033,72.42307)
  -- (260.15033,72.36309)
  -- (260.29033,72.47310)
  -- (260.37033,72.43308)
  -- (260.60034,72.54308)
  -- (260.71033,72.55308)
  -- (260.82034,72.45309)
  -- (260.99034,72.48307)
  -- (261.24034,73.08308)
  -- (261.30034,74.10310)
  -- (261.61034,71.99308)
  -- (261.78033,73.18308)
  -- (261.83034,72.55308)
  -- (261.89034,73.12309)
  -- (262.11034,72.49310)
  -- (262.25034,73.04307)
  -- (262.34033,72.88308)
  -- (262.48033,72.98309)
  -- (262.56033,73.15307)
  -- (262.65033,72.53308)
  -- (262.68033,72.91308)
  -- (262.73033,72.47310)
  -- (262.82034,73.41308)
  -- (262.96034,73.35308)
  -- (263.01033,73.70307)
  -- (263.57034,72.52308)
  -- (263.74034,72.34309)
  -- (264.19034,72.35308)
  -- (264.78035,72.23307)
  -- (265.26033,72.52308)
  -- (265.96036,72.64308)
  -- (266.30034,72.58310)
  -- (266.75034,72.77308)
  -- (266.97034,72.68307)
  -- (267.20033,72.71308)
  -- (267.22034,72.66308)
  -- (267.25035,72.72308)
  -- (267.31033,72.65309)
  -- (267.36035,72.70307)
  -- (267.67035,72.57308)
  -- (268.26033,72.68307)
  -- (268.99036,72.57308)
  -- (270.65034,72.60310)
  -- (271.10036,72.52308)
  -- (271.91034,72.62307)
  -- (273.91035,72.64308)
  -- (274.30035,72.56309)
  -- (276.01035,72.66308)
  -- (277.05037,72.57308)
  -- (278.74037,72.67309)
  -- (279.35036,72.52308)
  -- (280.14037,72.62307)
  -- (280.51035,72.54308)
  -- (281.77037,72.62307)
  -- (282.67036,72.50308)
  -- (283.00037,72.60310)
  -- (283.68036,72.54308)
  -- (284.55037,72.78309)
  -- (285.19037,72.66308)
  -- (285.31036,72.34309)
  -- (285.45036,72.73307)
  -- (285.47037,72.65309)
  -- (285.50037,72.71308)
  -- (285.64037,72.66308)
  -- (286.06036,72.79307)
  -- (286.43036,72.71308)
  -- (287.05037,72.39308)
  -- (287.41037,72.55308)
  -- (287.89038,72.49310)
  -- (288.31036,72.52308)
  -- (288.48036,72.68307)
  -- (288.79036,72.68307)
  -- (289.24037,72.86308)
  -- (289.60039,72.64308)
  -- (289.97037,72.72308)
  -- (290.22037,72.62307)
  -- (290.61038,72.72308)
  -- (291.54037,72.74310)
  -- (291.93036,72.63310)
  -- (292.35037,72.65309)
  -- (292.52039,72.54308)
  -- (292.69038,72.67309)
  -- (292.83038,72.68307)
  -- (293.22037,73.03309)
  -- (293.73036,72.66308)
  -- (294.60039,72.63310)
  -- (294.80038,72.72308)
  -- (295.47038,72.58310)
  -- (296.34038,72.79307)
  -- (297.21039,72.67309)
  -- (297.32039,73.02308)
  -- (297.41039,72.76309)
  -- (297.52039,72.70307)
  -- (297.55038,72.75308)
  -- (297.60040,72.64308)
  -- (297.69040,72.63310)
  -- (298.62038,72.78309)
  -- (298.87039,72.71308)
  -- (300.33038,72.70307)
  -- (300.89040,72.80310)
  -- (301.68037,72.63310)
  -- (302.57039,72.67309)
  -- (304.03040,72.42307)
  -- (305.04037,72.38310)
  -- (306.36040,72.52308)
  -- (306.65039,72.47310)
  -- (308.84040,72.52308)
  -- (309.26039,72.47310)
  -- (310.63040,72.46308)
  -- (311.70040,72.52308)
  -- (312.01039,72.46308)
  -- (312.20040,72.51307)
  -- (312.43040,72.47310)
  -- (313.08040,72.72308)
  -- (313.33040,72.73307)
  -- (313.61041,72.66308)
  -- (313.83041,72.72308)
  -- (314.11040,72.62307)
  -- (314.59041,72.59307)
  -- (315.55040,72.70307)
  -- (316.58041,72.72308)
  -- (317.62040,72.65309)
  -- (318.66042,72.70307)
  -- (320.63042,72.67309)
  -- (321.11041,72.73307)
  -- (322.23041,72.62307)
  -- (322.93040,72.71308)
  -- (323.58043,72.63310)
  -- (326.64041,72.62307)
  -- (327.34042,72.69310)
  -- (327.79042,72.62307)
  -- (328.97043,72.65309)
  -- (329.78043,72.60310)
  -- (330.65042,72.76309)
  -- (331.24043,72.60310)
  -- (331.66043,72.58310)
  -- (332.36043,72.71308)
  -- (333.21043,72.56309)
  -- (334.02043,72.75308)
  -- (334.78044,72.62307)
  -- (337.22043,72.71308)
  -- (338.04042,72.64308)
  -- (338.63045,72.71308)
  -- (339.41045,72.64308)
  -- (340.09044,72.68307)
  -- (346.63046,72.66308)
  -- (347.16046,72.74310)
  -- (347.89046,72.64308)
  -- (349.01045,72.68307)
  -- (349.07047,72.74310)
  -- (349.21046,72.67309)
  -- (351.29045,72.71308)
  -- (351.74046,72.65309)
  -- (352.47046,72.69310)
  -- (353.23045,72.65309)
  -- (353.59045,72.74310)
  -- (354.80048,72.62307)
  -- (354.97046,72.65309)
  -- (355.02046,72.75308)
  -- (355.11046,72.77308)
  -- (355.25046,72.66308)
  -- (355.39046,72.64308)
  -- (356.15045,72.70307)
  -- (357.21046,72.64308)
  -- (357.63048,72.70307)
  -- (358.62045,72.67309)
  -- (358.73045,72.84307)
  -- (358.87047,72.61308)
  -- (358.98047,72.60310)
  -- (359.74048,72.62307)
  -- (359.94048,72.68307)
  -- (361.54047,72.61308)
  -- (361.79047,72.70307)
  -- (362.55048,72.62307)
  -- (363.08047,72.67309)
  -- (363.22047,72.62307)
  -- (364.48047,72.64308)
  -- (364.99048,72.59307)
  -- (365.58049,72.68307)
  -- (367.26047,72.50308)
  -- (367.97047,72.52308)
  -- (368.22047,72.44308)
  -- (368.67049,72.46308)
  -- (368.72047,72.42307)
  -- (368.78049,72.50308)
  -- (368.98048,72.43308)
  -- (369.17047,72.44308)
  -- (369.37047,72.33308)
  -- (369.62047,72.32308)
  -- (370.24048,72.05310)
  -- (370.38050,72.12307)
  -- (370.55048,72.02308)
  -- (370.61049,72.05310)
  -- (370.72049,72.00309)
  -- (370.77048,72.06307)
  -- (370.89049,71.99308)
  -- (370.91048,72.05310)
  -- (371.05049,72.00309)
  -- (371.17047,72.10308)
  -- (371.31047,71.94310)
  -- (371.45049,72.09309)
  -- (371.56049,71.95307)
  -- (371.70049,72.06307)
  -- (372.07050,71.94310)
  -- (372.46050,71.97308)
  -- (373.13048,71.74310)
  -- (373.22047,71.84307)
  -- (373.33047,71.74310)
  -- (373.44049,71.80310)
  -- (374.59048,71.85310)
  -- (375.01048,71.77308)
  -- (375.24050,71.79307)
  -- (375.63050,71.69310)
  -- (375.74050,71.74310)
  -- (375.97049,71.71308)
  -- (376.11049,71.54307)
  -- (376.33049,71.72308)
  -- (377.46050,71.68307)
  -- (377.68048,71.75308)
  -- (377.96050,71.68307)
  -- (378.19049,71.76309)
  -- (378.36050,71.67309)
  -- (378.66049,71.75308)
  -- (379.23048,71.68307)
  -- (379.39049,71.74310)
  -- (379.56050,71.69310)
  -- (383.86050,71.72308)
  -- (384.03050,71.71308)
  -- (384.08050,71.56309)
  -- (384.14050,71.81307)
  -- (384.20049,71.73307)
  -- (384.31049,71.85310)
  -- (384.45050,71.61308)
  -- (384.50050,71.70307)
  -- (384.53049,71.67309)
  -- (384.67050,71.75308)
  -- (384.78050,71.70307)
  -- (385.63051,71.73307)
  -- (385.77051,71.68307)
  -- (385.99051,71.76309)
  -- (386.16050,71.66308)
  -- (386.47050,71.75308)
  -- (386.64050,71.65309)
  -- (386.95050,71.74310)
  -- (387.20050,71.67309)
  -- (387.42050,71.79307)
  -- (387.56050,71.67309)
  -- (387.76050,71.78309)
  -- (388.04050,71.63308)
  -- (388.15050,71.63308)
  -- (388.38052,71.84307)
  -- (388.60052,71.54307)
  -- (388.83050,71.79307)
  -- (389.02051,71.65309)
  -- (389.25050,71.81307)
  -- (389.50050,71.59307)
  -- (389.70050,71.78309)
  -- (389.89052,71.67309)
  -- (390.15050,71.78309)
  -- (390.37050,71.62307)
  -- (390.57051,71.78309)
  -- (390.79050,71.67309)
  -- (390.88051,71.70307);
% Reference trace 22
\path[draw={rgb,1:red,0.137;green,0.624;blue,0.651},line width=0.32877bp] (110.44012,71.74310)
  -- (120.63016,71.74310)
  -- (120.86014,71.81307)
  -- (121.14015,71.66308)
  -- (121.39015,71.79307)
  -- (121.81015,71.78309)
  -- (122.01015,71.68307)
  -- (122.32016,71.79307)
  -- (123.89015,71.72308)
  -- (124.28015,71.77308)
  -- (124.56015,71.71308)
  -- (124.96016,71.76309)
  -- (128.92015,71.72308)
  -- (129.28015,71.77308)
  -- (129.84015,71.71308)
  -- (130.77016,71.80310)
  -- (131.11015,71.71308)
  -- (131.89017,71.77308)
  -- (132.42015,71.72308)
  -- (134.78017,71.75308)
  -- (135.20015,71.70307)
  -- (135.29016,71.64308)
  -- (135.46017,71.71308)
  -- (135.54016,71.65309)
  -- (135.68016,71.70307)
  -- (135.79016,71.66308)
  -- (136.10017,72.03308)
  -- (136.13017,72.16310)
  -- (136.19017,72.06307)
  -- (136.24017,72.18308)
  -- (136.30017,72.07310)
  -- (136.36017,72.14309)
  -- (136.58017,72.08308)
  -- (137.11017,71.86308)
  -- (137.14017,71.80310)
  -- (137.20016,71.83308)
  -- (137.34016,71.70307)
  -- (137.37016,71.76309)
  -- (137.42017,71.61308)
  -- (137.45016,71.67309)
  -- (137.93016,71.34307)
  -- (138.04016,71.41308)
  -- (138.63017,71.43307)
  -- (139.05017,71.78309)
  -- (139.42017,71.86308)
  -- (139.47018,71.94310)
  -- (139.64017,71.93307)
  -- (139.72017,72.05310)
  -- (139.84016,72.07310)
  -- (140.71017,71.90307)
  -- (140.93016,71.94310)
  -- (141.18018,71.87309)
  -- (141.44017,71.89309)
  -- (141.52019,71.81307)
  -- (141.66017,71.88308)
  -- (141.72018,71.81307)
  -- (142.28017,71.99308)
  -- (142.48016,71.92307)
  -- (143.12018,71.87309)
  -- (144.25018,72.03308)
  -- (144.47018,71.97308)
  -- (145.06018,71.99308)
  -- (145.26018,71.94310)
  -- (146.04018,71.99308)
  -- (146.10019,71.95307)
  -- (146.24019,72.02308)
  -- (147.47018,71.90307)
  -- (148.04018,72.06307)
  -- (148.06018,72.02308)
  -- (148.12018,72.11308)
  -- (148.15018,72.05310)
  -- (148.20018,72.10308)
  -- (148.37018,72.08308)
  -- (148.63019,72.19308)
  -- (148.79018,72.14309)
  -- (148.82019,72.04307)
  -- (148.93018,72.20307)
  -- (149.75018,71.85310)
  -- (150.70018,71.95307)
  -- (150.73018,71.87309)
  -- (150.90018,71.97308)
  -- (150.93018,71.90307)
  -- (150.98020,71.97308)
  -- (151.04018,71.88308)
  -- (151.07020,71.94310)
  -- (151.29019,71.85310)
  -- (151.32019,71.96310)
  -- (151.35019,71.84307)
  -- (151.41019,71.95307)
  -- (151.46019,71.85310)
  -- (151.49020,71.92307)
  -- (151.52019,71.79307)
  -- (151.55019,72.04307)
  -- (151.57019,71.79307)
  -- (151.63019,72.00309)
  -- (151.71019,71.81307)
  -- (151.85020,72.01307)
  -- (151.88019,71.81307)
  -- (151.91019,72.02308)
  -- (151.94020,71.90307)
  -- (151.97018,72.00309)
  -- (151.99019,71.75308)
  -- (152.02019,72.11308)
  -- (152.05020,71.87309)
  -- (152.11018,72.00309)
  -- (152.16020,71.88308)
  -- (152.19019,72.13308)
  -- (152.25020,71.81307)
  -- (152.28018,72.08308)
  -- (152.30019,71.96310)
  -- (152.36020,72.03308)
  -- (152.42018,72.00309)
  -- (152.44019,71.85310)
  -- (152.47020,71.99308)
  -- (152.56020,71.95307)
  -- (152.58020,72.02308)
  -- (152.98020,71.97308)
  -- (153.01018,71.89309)
  -- (153.03020,72.03308)
  -- (153.09020,71.92307)
  -- (153.26018,72.05310)
  -- (153.31018,71.98309)
  -- (153.34020,72.09309)
  -- (153.37018,72.02308)
  -- (153.45020,72.06307)
  -- (153.48018,72.00309)
  -- (153.51018,72.06307)
  -- (153.54019,71.94310)
  -- (153.60020,72.05310)
  -- (153.62018,72.00309)
  -- (153.71019,72.03308)
  -- (153.76020,71.92307)
  -- (153.79018,72.05310)
  -- (154.02019,71.94310)
  -- (154.04018,72.02308)
  -- (154.13019,71.91308)
  -- (154.21020,71.96310)
  -- (154.27020,71.76309)
  -- (154.30020,72.15307)
  -- (154.38020,71.56309)
  -- (154.41020,72.01307)
  -- (154.44019,71.63308)
  -- (154.49020,72.14309)
  -- (154.52020,72.09309)
  -- (154.55019,72.22308)
  -- (154.58020,72.09309)
  -- (154.61020,72.22308)
  -- (154.66019,72.17307)
  -- (154.69020,72.41308)
  -- (154.72020,72.21308)
  -- (154.75018,72.40307)
  -- (154.80020,72.24308)
  -- (154.83020,72.38310)
  -- (154.86018,72.16310)
  -- (154.89020,72.29308)
  -- (155.00020,72.08308)
  -- (155.06018,72.15307)
  -- (155.25020,71.93307)
  -- (155.39020,71.99308)
  -- (155.50020,71.90307)
  -- (156.09020,71.94310)
  -- (156.37020,71.89309)
  -- (156.77020,72.01307)
  -- (156.99020,71.94310)
  -- (157.33018,72.00309)
  -- (157.58020,71.88308)
  -- (158.14020,71.82308)
  -- (158.42020,71.90307)
  -- (159.15019,71.85310)
  -- (159.35020,71.92307)
  -- (159.63020,71.87309)
  -- (160.84020,71.93307)
  -- (161.68019,71.89309)
  -- (161.71020,71.70307)
  -- (161.77020,71.87309)
  -- (161.82020,71.80310)
  -- (161.85020,71.96310)
  -- (161.88020,71.66308)
  -- (162.02020,71.92307)
  -- (162.13020,71.83308)
  -- (162.47021,71.93307)
  -- (162.97020,71.81307)
  -- (163.11020,72.17307)
  -- (163.17020,72.15307)
  -- (163.20020,72.23307)
  -- (163.31020,71.88308)
  -- (163.45021,72.10308)
  -- (163.56021,72.10308)
  -- (163.62020,72.02308)
  -- (163.79019,72.07310)
  -- (163.82020,71.97308)
  -- (163.87021,72.01307)
  -- (163.90019,71.82308)
  -- (163.93019,72.01307)
  -- (163.98021,71.88308)
  -- (164.04019,71.93307)
  -- (164.07022,71.87309)
  -- (164.10020,71.94310)
  -- (164.40019,72.02308)
  -- (164.43020,71.97308)
  -- (164.66020,72.16310)
  -- (165.16022,72.30308)
  -- (165.61021,71.97308)
  -- (165.95020,71.81307)
  -- (166.59021,71.74310)
  -- (168.22020,71.88308)
  -- (168.67021,72.07310)
  -- (169.32022,72.22308)
  -- (170.02022,72.03308)
  -- (170.81021,72.12307)
  -- (172.58023,71.88308)
  -- (172.94022,72.00309)
  -- (173.19022,72.01307)
  -- (173.56023,71.91308)
  -- (173.73021,71.99308)
  -- (173.84021,71.93307)
  -- (174.46022,71.93307)
  -- (175.44022,71.74310)
  -- (176.14023,71.78309)
  -- (176.48021,71.92307)
  -- (177.40020,71.82308)
  -- (177.52023,71.88308)
  -- (177.57022,71.84307)
  -- (179.09023,71.81307)
  -- (179.85023,71.87309)
  -- (180.58023,71.74310)
  -- (181.98022,71.86308)
  -- (182.40022,71.71308)
  -- (182.63023,71.69310)
  -- (182.88023,71.75308)
  -- (183.89024,71.72308)
  -- (184.42023,71.79307)
  -- (186.02023,71.76309)
  -- (186.36024,71.81307)
  -- (187.77023,71.74310)
  -- (188.24023,71.85310)
  -- (189.14024,71.79307)
  -- (189.84023,71.84307)
  -- (190.63025,71.74310)
  -- (191.36024,71.89309)
  -- (192.20023,71.72308)
  -- (192.74025,71.92307)
  -- (193.72025,71.73307)
  -- (194.78026,71.93307)
  -- (195.77025,71.80310)
  -- (195.99025,71.82308)
  -- (196.10025,72.25309)
  -- (196.24025,71.81307)
  -- (196.30025,71.78309)
  -- (196.39024,71.92307)
  -- (196.50024,71.86308)
  -- (197.17024,72.35308)
  -- (197.56026,72.17307)
  -- (198.10025,71.74310)
  -- (198.49026,71.64308)
  -- (198.86024,71.71308)
  -- (199.31024,71.68307)
  -- (199.33025,71.56309)
  -- (199.67026,72.07310)
  -- (199.89026,72.21308)
  -- (200.04024,72.21308)
  -- (200.29025,72.12307)
  -- (200.46025,72.13308)
  -- (200.91025,71.88308)
  -- (201.13025,71.87309)
  -- (201.41026,71.63308)
  -- (201.50026,71.76309)
  -- (201.52026,71.73307)
  -- (201.72026,71.84307)
  -- (201.92026,71.73307)
  -- (202.17026,71.70307)
  -- (202.31024,71.83308)
  -- (202.39026,71.65309)
  -- (202.51024,72.07310)
  -- (202.53024,71.97308)
  -- (202.76025,72.23307)
  -- (202.93024,72.33308)
  -- (203.26025,72.24308)
  -- (203.43025,72.14309)
  -- (203.46027,72.04307)
  -- (203.52026,72.08308)
  -- (203.66026,71.96310)
  -- (203.83026,71.99308)
  -- (204.11024,71.84307)
  -- (204.16026,71.92307)
  -- (204.19026,71.86308)
  -- (204.70026,72.00309)
  -- (204.89026,71.95307)
  -- (205.17026,71.97308)
  -- (205.29025,71.87309)
  -- (205.34026,71.96310)
  -- (205.37025,71.87309)
  -- (205.45026,71.93307)
  -- (205.62025,71.87309)
  -- (205.79025,72.18308)
  -- (205.93025,71.98309)
  -- (206.02026,72.05310)
  -- (206.24026,71.87309)
  -- (206.38028,71.94310)
  -- (206.46027,71.75308)
  -- (206.52026,71.85310)
  -- (206.69028,71.71308)
  -- (206.77026,71.72308)
  -- (206.80028,71.79307)
  -- (206.83026,71.75308)
  -- (207.14026,72.12307)
  -- (207.22026,72.04307)
  -- (207.25026,72.12307)
  -- (207.31026,72.06307)
  -- (207.42026,72.14309)
  -- (207.48026,72.06307)
  -- (207.59026,72.11308)
  -- (207.76027,71.90307)
  -- (207.84026,71.89309)
  -- (207.95026,71.98309)
  -- (208.07028,71.94310)
  -- (208.18027,72.01307)
  -- (208.21027,71.93307)
  -- (208.26025,72.02308)
  -- (208.32027,71.93307)
  -- (208.43025,72.14309)
  -- (208.80028,71.67309)
  -- (208.85028,71.71308)
  -- (208.94028,71.66308)
  -- (208.96028,71.79307)
  -- (208.99026,71.61308)
  -- (209.02026,71.90307)
  -- (209.05028,71.72308)
  -- (209.13026,71.93307)
  -- (209.16028,71.75308)
  -- (209.19026,71.92307)
  -- (209.27028,71.87309)
  -- (209.30026,71.98309)
  -- (209.33026,71.90307)
  -- (209.50026,72.07310)
  -- (209.86026,71.90307)
  -- (209.95026,71.96310)
  -- (210.03027,71.77308)
  -- (210.14027,72.15307)
  -- (210.20026,72.05310)
  -- (210.34027,72.38310)
  -- (210.40025,72.31307)
  -- (210.51025,72.40307)
  -- (210.62025,72.37307)
  -- (211.15025,72.09309)
  -- (211.21028,72.12307)
  -- (211.24026,72.05310)
  -- (211.29027,72.08308)
  -- (211.32028,71.99308)
  -- (211.35027,72.05310)
  -- (211.41028,71.97308)
  -- (211.63028,72.08308)
  -- (211.80028,72.26307)
  -- (211.86026,74.18308)
  -- (211.91026,72.64308)
  -- (211.94028,72.83310)
  -- (212.00027,72.24308)
  -- (212.05028,72.48307)
  -- (212.08028,72.27310)
  -- (212.22026,72.56309)
  -- (212.28027,72.45309)
  -- (212.45027,72.51307)
  -- (212.64026,72.31307)
  -- (212.70027,72.36309)
  -- (212.87027,72.07310)
  -- (212.98027,72.09309)
  -- (213.01027,72.16310)
  -- (213.06027,71.98309)
  -- (213.09027,72.05310)
  -- (213.20026,71.97308)
  -- (213.46028,72.26307)
  -- (213.65027,71.96310)
  -- (213.82027,72.23307)
  -- (213.85028,72.09309)
  -- (213.88028,72.19308)
  -- (213.96028,72.02308)
  -- (214.02026,72.09309)
  -- (214.05028,71.99308)
  -- (214.07028,72.07310)
  -- (214.13026,71.97308)
  -- (214.19028,72.03308)
  -- (214.21028,71.85310)
  -- (214.27028,71.96310)
  -- (214.33026,71.85310)
  -- (214.41028,71.94310)
  -- (215.06027,72.12307)
  -- (215.31026,72.00309)
  -- (215.59027,72.09309)
  -- (216.63028,71.90307)
  -- (217.50027,72.22308)
  -- (221.04027,72.06307)
  -- (223.51027,72.30308)
  -- (225.47029,72.22308)
  -- (227.02030,72.31307)
  -- (227.47029,72.29308)
  -- (227.83029,72.38310)
  -- (227.89029,72.49310)
  -- (227.92029,72.36309)
  -- (227.97029,72.50308)
  -- (228.00030,72.34309)
  -- (228.03029,72.45309)
  -- (228.08029,72.40307)
  -- (228.17029,72.47310)
  -- (228.31029,72.32308)
  -- (228.51028,72.60310)
  -- (228.56029,72.56309)
  -- (228.67029,72.63310)
  -- (229.24030,72.22308)
  -- (229.63030,71.80310)
  -- (229.88030,71.67309)
  -- (230.13030,71.74310)
  -- (230.30030,71.87309)
  -- (230.50029,71.83308)
  -- (230.95029,72.31307)
  -- (231.00030,73.22308)
  -- (231.17029,72.12307)
  -- (231.23029,72.26307)
  -- (231.26028,72.08308)
  -- (231.29030,72.13308)
  -- (231.34030,72.08308)
  -- (231.40028,71.95307)
  -- (231.43028,72.13308)
  -- (231.45030,72.02308)
  -- (231.57030,72.12307)
  -- (231.68028,71.92307)
  -- (231.71030,72.11308)
  -- (231.82030,71.96310)
  -- (231.85031,72.01307)
  -- (231.90028,71.92307)
  -- (231.93028,72.01307)
  -- (232.16031,71.85310)
  -- (232.21030,71.98309)
  -- (232.32031,71.64308)
  -- (232.49031,71.93307)
  -- (232.75029,71.35308)
  -- (232.89030,71.82308)
  -- (233.11029,71.64308)
  -- (233.19029,71.72308)
  -- (233.31029,71.69310)
  -- (233.98030,72.26307)
  -- (234.77030,72.15307)
  -- (235.08030,72.21308)
  -- (235.67030,72.02308)
  -- (236.28030,72.29308)
  -- (236.34030,72.25309)
  -- (236.40028,72.31307)
  -- (236.48030,72.23307)
  -- (236.59030,73.21308)
  -- (236.68030,72.13308)
  -- (236.76030,72.45309)
  -- (236.79030,72.22308)
  -- (236.82030,72.54308)
  -- (236.90030,71.94310)
  -- (236.93028,72.10308)
  -- (237.07031,71.80310)
  -- (237.10031,71.85310)
  -- (237.18030,71.80310)
  -- (237.38031,71.83308)
  -- (237.46031,71.76309)
  -- (237.49031,71.60310)
  -- (237.55031,71.77308)
  -- (237.74031,71.68307)
  -- (238.05031,72.00309)
  -- (238.89030,72.52308)
  -- (239.03030,72.44308)
  -- (239.06030,72.48307)
  -- (239.29030,72.27310)
  -- (239.34030,72.30308)
  -- (239.79030,71.78309)
  -- (239.85031,71.83308)
  -- (239.88031,71.73307)
  -- (239.93030,71.81307)
  -- (240.07031,71.70307)
  -- (240.27031,71.68307)
  -- (241.81030,72.04307)
  -- (242.32031,72.10308)
  -- (246.25032,72.03308)
  -- (246.95030,72.12307)
  -- (248.41032,72.14309)
  -- (249.25032,72.29308)
  -- (249.37032,72.54308)
  -- (249.40030,72.42307)
  -- (249.42032,72.56309)
  -- (249.48032,72.39308)
  -- (249.51030,72.57308)
  -- (249.56032,72.38310)
  -- (249.59032,72.44308)
  -- (249.68031,72.37307)
  -- (249.73032,72.44308)
  -- (249.76031,72.37307)
  -- (249.87032,72.44308)
  -- (250.29031,72.19308)
  -- (250.57033,72.14309)
  -- (250.60034,72.18308)
  -- (250.74033,72.12307)
  -- (250.80034,72.18308)
  -- (250.83032,72.14309)
  -- (251.25032,72.28308)
  -- (251.78033,72.19308)
  -- (251.84032,72.27310)
  -- (251.87032,72.19308)
  -- (251.92032,72.50308)
  -- (252.09033,72.14309)
  -- (252.12032,72.27310)
  -- (252.18033,72.10308)
  -- (252.20032,72.19308)
  -- (252.26031,72.08308)
  -- (252.34032,72.19308)
  -- (252.37032,72.10308)
  -- (252.43031,72.29308)
  -- (252.48032,72.17307)
  -- (252.54031,72.32308)
  -- (252.57033,72.24308)
  -- (252.68031,72.43308)
  -- (253.02032,72.56309)
  -- (253.07034,72.45309)
  -- (253.10033,72.54308)
  -- (253.16034,72.46308)
  -- (253.19032,72.51307)
  -- (253.38034,72.48307)
  -- (253.92032,72.00309)
  -- (254.17032,71.92307)
  -- (254.22032,71.84307)
  -- (254.28032,71.97308)
  -- (254.31032,71.90307)
  -- (254.37032,72.45309)
  -- (254.42032,72.42307)
  -- (254.51031,71.84307)
  -- (254.56033,72.14309)
  -- (254.59032,72.05310)
  -- (254.67033,72.22308)
  -- (254.81032,72.13308)
  -- (254.95032,72.16310)
  -- (255.04031,72.12307)
  -- (255.07034,71.89309)
  -- (255.10033,72.25309)
  -- (255.15031,71.94310)
  -- (255.18033,72.03308)
  -- (255.26031,71.94310)
  -- (255.54033,71.85310)
  -- (255.71033,71.61308)
  -- (255.74034,71.45309)
  -- (255.77032,71.85310)
  -- (255.80034,71.45309)
  -- (255.85034,71.58310)
  -- (255.88033,71.47310)
  -- (255.91032,71.51307)
  -- (256.02032,71.91308)
  -- (256.16034,71.64308)
  -- (256.25034,71.59307)
  -- (256.30034,71.90307)
  -- (256.33032,71.49310)
  -- (256.36034,71.83308)
  -- (256.41034,71.63308)
  -- (256.56033,72.09309)
  -- (256.58034,72.01307)
  -- (256.67033,72.16310)
  -- (256.75032,71.94310)
  -- (256.78033,72.02308)
  -- (256.89034,71.88308)
  -- (256.92033,72.22308)
  -- (256.95032,72.06307)
  -- (257.00034,72.14309)
  -- (257.06032,71.91308)
  -- (257.23033,71.92307)
  -- (257.43033,71.65309)
  -- (257.76033,71.52308)
  -- (257.96034,71.34307)
  -- (258.02032,71.45309)
  -- (258.04031,71.35308)
  -- (258.10034,71.40307)
  -- (258.27034,71.93307)
  -- (258.41034,72.15307)
  -- (258.58034,72.17307)
  -- (258.83034,72.00309)
  -- (259.00034,71.96310)
  -- (259.05034,72.01307)
  -- (259.22032,71.94310)
  -- (259.42032,72.04307)
  -- (259.81033,72.08308)
  -- (260.01033,71.95307)
  -- (260.91032,71.95307)
  -- (261.30034,72.30308)
  -- (261.33034,72.23307)
  -- (261.47034,72.54308)
  -- (261.61034,72.57308)
  -- (261.75034,72.46308)
  -- (261.81033,71.90307)
  -- (261.83034,72.22308)
  -- (261.95033,72.15307)
  -- (262.00035,72.40307)
  -- (262.09033,72.22308)
  -- (262.14034,72.27310)
  -- (262.17033,72.08308)
  -- (262.23033,72.15307)
  -- (262.40033,71.65309)
  -- (262.56033,71.95307)
  -- (262.62033,71.83308)
  -- (262.65033,72.05310)
  -- (262.70033,71.87309)
  -- (262.73033,71.97308)
  -- (262.76033,71.94310)
  -- (262.87033,71.64308)
  -- (263.04033,71.54307)
  -- (263.10034,71.42307)
  -- (263.24034,71.58310)
  -- (263.29034,71.57308)
  -- (263.66034,71.83308)
  -- (263.86034,71.88308)
  -- (264.00035,71.87309)
  -- (264.39034,71.69310)
  -- (264.92033,71.68307)
  -- (265.29034,71.82308)
  -- (266.07036,72.27310)
  -- (266.49036,72.39308)
  -- (266.52036,72.45309)
  -- (266.55034,72.40307)
  -- (266.63036,72.47310)
  -- (266.66034,72.40307)
  -- (266.83035,72.49310)
  -- (266.89035,72.41308)
  -- (266.92035,72.48307)
  -- (266.94035,72.41308)
  -- (267.03035,72.45309)
  -- (267.06033,72.37307)
  -- (267.11034,72.44308)
  -- (267.17033,72.37307)
  -- (267.20033,72.47310)
  -- (267.25035,72.32308)
  -- (267.28033,72.45309)
  -- (267.31033,72.36309)
  -- (267.36035,72.43308)
  -- (267.39034,72.32308)
  -- (267.42033,72.45309)
  -- (267.45035,72.35308)
  -- (267.51033,72.42307)
  -- (267.56035,72.32308)
  -- (267.59033,72.41308)
  -- (267.62033,72.32308)
  -- (267.67035,72.37307)
  -- (267.73033,72.29308)
  -- (267.76035,72.33308)
  -- (267.90034,72.29308)
  -- (268.43034,72.05310)
  -- (269.58035,71.83308)
  -- (271.32036,71.92307)
  -- (274.55035,71.87309)
  -- (275.25035,71.92307)
  -- (277.42035,71.89309)
  -- (280.42035,71.98309)
  -- (282.27037,71.89309)
  -- (284.80038,72.13308)
  -- (285.19037,72.09309)
  -- (285.28036,72.03308)
  -- (285.39037,72.10308)
  -- (286.40036,72.10308)
  -- (287.72037,71.82308)
  -- (289.13037,71.97308)
  -- (289.86037,71.92307)
  -- (289.88037,71.87309)
  -- (291.03038,71.98309)
  -- (292.30038,71.83308)
  -- (292.63039,71.88308)
  -- (293.03038,72.05310)
  -- (293.51036,71.70307)
  -- (294.71037,71.80310)
  -- (295.58038,72.12307)
  -- (295.92038,72.16310)
  -- (297.10039,71.94310)
  -- (297.24039,71.93307)
  -- (297.32039,72.11308)
  -- (297.49040,71.90307)
  -- (297.63039,71.96310)
  -- (298.56040,71.88308)
  -- (299.26038,71.95307)
  -- (300.33038,71.83308)
  -- (301.00040,71.85310)
  -- (301.39038,71.80310)
  -- (302.63040,71.87309)
  -- (303.56040,71.72308)
  -- (304.46040,71.79307)
  -- (306.20038,71.75308)
  -- (308.36040,71.83308)
  -- (311.56041,71.78309)
  -- (312.46040,71.81307)
  -- (313.89041,71.69310)
  -- (317.01040,71.64308)
  -- (322.12040,71.68307)
  -- (322.73041,71.60310)
  -- (323.52043,71.72308)
  -- (325.20041,71.60310)
  -- (331.38045,71.67309)
  -- (335.59042,71.62307)
  -- (337.98044,71.69310)
  -- (339.69044,71.68307)
  -- (340.70044,71.60310)
  -- (342.16045,71.69310)
  -- (342.89046,71.62307)
  -- (344.44044,71.68307)
  -- (346.21045,71.63308)
  -- (347.22044,71.67309)
  -- (347.98045,71.62307)
  -- (349.41046,71.71308)
  -- (350.84045,71.59307)
  -- (351.71045,71.66308)
  -- (352.47046,71.61308)
  -- (354.52046,71.68307)
  -- (354.97046,71.66308)
  -- (354.99046,71.58310)
  -- (355.22046,71.66308)
  -- (355.92046,71.61308)
  -- (356.60048,71.67309)
  -- (358.59045,71.65309)
  -- (358.73045,71.44308)
  -- (358.81047,71.68307)
  -- (358.90047,71.73307)
  -- (359.07048,71.65309)
  -- (361.12047,71.66308)
  -- (361.62045,71.72308)
  -- (362.24048,71.89309)
  -- (363.08047,71.64308)
  -- (363.61047,71.63308)
  -- (365.02048,71.78309)
  -- (366.93047,71.62307)
  -- (368.16049,71.72308)
  -- (368.33047,71.79307)
  -- (368.67049,71.77308)
  -- (368.72047,71.71308)
  -- (368.78049,71.80310)
  -- (369.31047,71.62307)
  -- (369.54048,71.71308)
  -- (369.85050,71.70307)
  -- (370.04047,71.80310)
  -- (370.13048,71.68307)
  -- (370.16049,71.75308)
  -- (370.21050,71.68307)
  -- (370.38050,71.82308)
  -- (370.72049,71.78309)
  -- (370.77048,71.71308)
  -- (371.14049,71.82308)
  -- (371.20047,71.74310)
  -- (371.31047,71.72308)
  -- (371.39049,71.78309)
  -- (371.53047,71.69310)
  -- (371.70049,71.76309)
  -- (371.76048,71.68307)
  -- (371.98048,71.74310)
  -- (372.04047,71.66308)
  -- (372.15047,71.67309)
  -- (372.40047,71.75308)
  -- (372.60050,71.66308)
  -- (372.85050,71.73307)
  -- (372.96050,71.90307)
  -- (373.19049,71.84307)
  -- (373.41049,71.67309)
  -- (373.78049,71.79307)
  -- (374.09048,71.69310)
  -- (374.42047,71.78309)
  -- (374.68048,71.72308)
  -- (375.04048,71.76309)
  -- (375.55049,71.71308)
  -- (376.08049,71.86308)
  -- (376.45049,71.70307)
  -- (376.81049,71.76309)
  -- (378.07051,71.74310)
  -- (378.21050,71.80310)
  -- (378.86049,71.70307)
  -- (379.11049,71.79307)
  -- (379.39049,71.74310)
  -- (384.03050,71.76309)
  -- (384.11049,71.67309)
  -- (384.17050,71.80310)
  -- (384.22049,71.70307)
  -- (384.53049,71.83308)
  -- (384.84050,71.69310)
  -- (385.54050,71.78309)
  -- (385.91049,71.70307)
  -- (386.30050,71.84307)
  -- (386.55050,71.67309)
  -- (386.61050,71.72308)
  -- (386.72050,71.57308)
  -- (387.06050,71.85310)
  -- (387.26050,71.71308)
  -- (387.37050,71.78309)
  -- (387.48050,71.72308)
  -- (387.79050,71.79307)
  -- (387.87050,71.72308)
  -- (388.10051,71.75308)
  -- (388.29051,71.52308)
  -- (388.63051,71.98309)
  -- (388.97050,71.65309)
  -- (389.14050,71.65309)
  -- (389.53050,71.82308)
  -- (389.95050,71.66308)
  -- (390.43050,71.80310)
  -- (390.79050,71.68307)
  -- (390.88051,71.71308);
% Reference trace 23
\path[draw={rgb,1:red,0.937;green,0.691;blue,0.553},line width=0.32877bp] (113.26013,83.16311)
  -- (115.05014,83.15309)
  -- (115.08014,83.19310)
  -- (115.53014,83.14310)
  -- (115.56013,83.20309)
  -- (116.37013,83.18310)
  -- (116.43013,83.11309)
  -- (116.46014,83.18310)
  -- (116.71014,83.20309)
  -- (116.77014,83.15309)
  -- (116.96016,83.20309)
  -- (116.99014,83.12309)
  -- (117.02014,83.20309)
  -- (117.05016,83.14310)
  -- (117.07016,83.19310)
  -- (118.84013,83.15309)
  -- (119.69016,83.18310)
  -- (119.74016,83.23309)
  -- (119.83015,83.11309)
  -- (119.88014,83.22310)
  -- (119.94016,83.09310)
  -- (120.11014,83.23309)
  -- (120.39015,83.12309)
  -- (120.56015,83.23309)
  -- (120.75014,83.12309)
  -- (120.98015,83.21310)
  -- (121.31013,83.15309)
  -- (122.24014,83.16311)
  -- (122.86015,83.26309)
  -- (123.31013,83.14310)
  -- (123.48015,83.17309)
  -- (123.64015,83.09310)
  -- (124.15015,83.36310)
  -- (124.99016,83.12309)
  -- (125.02016,83.05311)
  -- (125.05016,83.10310)
  -- (125.22015,82.96311)
  -- (125.47015,82.88310)
  -- (125.67015,82.94310)
  -- (125.89017,82.80311)
  -- (126.03015,82.91310)
  -- (126.34015,82.65310)
  -- (126.48015,82.79308)
  -- (126.65015,82.66310)
  -- (126.68015,82.55310)
  -- (126.82016,82.54308)
  -- (127.01015,82.75309)
  -- (127.21016,82.54308)
  -- (127.46016,82.63310)
  -- (127.83015,82.42309)
  -- (127.94016,82.46310)
  -- (129.43016,82.34309)
  -- (129.85017,82.45309)
  -- (129.96017,82.39309)
  -- (130.83017,82.30310)
  -- (130.89017,82.22310)
  -- (130.92017,82.30310)
  -- (131.08015,82.30310)
  -- (131.14017,82.36310)
  -- (131.39015,82.29310)
  -- (131.73015,82.37309)
  -- (131.81017,82.24310)
  -- (131.84015,82.44310)
  -- (131.93015,82.18310)
  -- (131.96017,82.28309)
  -- (131.98016,82.24310)
  -- (132.07018,82.30310)
  -- (132.18016,82.26309)
  -- (132.77017,82.35310)
  -- (133.42015,82.31309)
  -- (134.57018,82.41310)
  -- (135.63017,82.28309)
  -- (136.36017,82.34309)
  -- (137.15016,82.27311)
  -- (137.51016,82.31309)
  -- (138.95016,82.23309)
  -- (140.13017,82.06309)
  -- (140.97017,82.06309)
  -- (142.57018,81.92309)
  -- (143.30019,81.94310)
  -- (143.47018,81.87310)
  -- (143.94019,81.90309)
  -- (145.18018,81.68308)
  -- (146.72018,81.63310)
  -- (147.73018,81.51309)
  -- (148.72018,81.52310)
  -- (149.08018,81.44310)
  -- (149.59018,81.54308)
  -- (150.74019,81.43308)
  -- (151.50018,81.49311)
  -- (151.75018,81.48309)
  -- (151.78020,81.43308)
  -- (151.83018,81.48309)
  -- (152.09020,81.46310)
  -- (152.11018,81.42309)
  -- (152.14020,81.49311)
  -- (152.23020,81.44310)
  -- (152.40018,81.51309)
  -- (153.41020,81.46310)
  -- (154.14020,81.55310)
  -- (154.78020,81.50309)
  -- (155.99020,81.76309)
  -- (156.21020,81.74310)
  -- (156.92020,81.98310)
  -- (157.08020,81.92309)
  -- (157.65019,82.09310)
  -- (158.46020,82.19310)
  -- (159.41020,81.99310)
  -- (159.72020,81.83310)
  -- (159.92020,81.90309)
  -- (159.98020,81.85310)
  -- (160.06020,81.93308)
  -- (160.12020,81.89310)
  -- (160.43019,82.02310)
  -- (160.45020,81.97310)
  -- (161.58022,82.03309)
  -- (161.60022,82.13310)
  -- (161.63020,81.96310)
  -- (161.80022,82.18310)
  -- (161.86020,81.81309)
  -- (161.89021,82.26309)
  -- (161.91020,82.02310)
  -- (161.97020,82.09310)
  -- (162.00021,81.99310)
  -- (162.03020,82.14309)
  -- (162.05020,82.01309)
  -- (162.08020,82.13310)
  -- (162.11020,81.99310)
  -- (162.14020,82.11309)
  -- (162.17020,82.03309)
  -- (162.19020,82.11309)
  -- (162.25021,82.06309)
  -- (162.28020,82.12309)
  -- (162.31020,81.98310)
  -- (162.33020,82.19310)
  -- (162.36021,82.03309)
  -- (162.45021,82.20309)
  -- (162.48020,82.11309)
  -- (162.53020,82.23309)
  -- (162.56021,81.99310)
  -- (162.59020,82.29310)
  -- (162.62020,82.18310)
  -- (162.70020,82.19310)
  -- (162.73020,82.27311)
  -- (162.76021,82.16311)
  -- (162.81020,82.26309)
  -- (162.87021,82.09310)
  -- (162.90019,82.23309)
  -- (162.92020,82.13310)
  -- (162.98021,82.18310)
  -- (163.12020,81.89310)
  -- (163.15019,82.07311)
  -- (163.18020,81.91310)
  -- (163.21020,81.97310)
  -- (163.23020,81.90309)
  -- (163.29020,81.93308)
  -- (163.32020,82.03309)
  -- (163.40019,81.88310)
  -- (163.43020,82.04308)
  -- (163.46020,81.97310)
  -- (163.65020,82.04308)
  -- (163.68019,82.00310)
  -- (163.71020,82.14309)
  -- (163.74022,82.08310)
  -- (163.85022,82.11309)
  -- (164.08020,81.90309)
  -- (164.33020,82.10310)
  -- (164.38022,82.03309)
  -- (164.52022,82.15309)
  -- (164.55020,82.01309)
  -- (164.58022,82.14309)
  -- (164.69022,82.06309)
  -- (164.83022,82.13310)
  -- (164.86020,82.02310)
  -- (164.89021,82.12309)
  -- (164.97020,82.06309)
  -- (165.37020,82.29310)
  -- (165.62020,82.36310)
  -- (165.84020,82.15309)
  -- (166.46020,82.19310)
  -- (166.66020,82.07311)
  -- (167.02020,82.07311)
  -- (167.42020,82.20309)
  -- (168.09021,82.16311)
  -- (168.29020,82.26309)
  -- (168.46022,82.20309)
  -- (168.68020,82.24310)
  -- (169.30022,82.15309)
  -- (169.52022,82.21310)
  -- (169.89021,82.15309)
  -- (170.31021,82.32310)
  -- (170.76021,82.31309)
  -- (171.85022,82.17309)
  -- (172.05022,82.20309)
  -- (172.64021,82.15309)
  -- (172.67023,82.11309)
  -- (172.75021,82.16311)
  -- (172.78023,82.06309)
  -- (172.81021,82.24310)
  -- (172.84021,82.08310)
  -- (172.86021,82.18310)
  -- (173.37021,82.10310)
  -- (175.92023,82.12309)
  -- (176.26021,82.01309)
  -- (177.33022,82.10310)
  -- (177.47023,82.03309)
  -- (179.60023,82.02310)
  -- (180.11021,81.93308)
  -- (180.64023,81.93308)
  -- (181.20021,82.01309)
  -- (182.16023,82.00310)
  -- (184.24023,81.93308)
  -- (184.85023,81.86309)
  -- (185.70023,81.91310)
  -- (186.12022,81.85310)
  -- (186.26022,81.91310)
  -- (187.30023,81.87310)
  -- (187.38025,81.82310)
  -- (187.41025,81.89310)
  -- (187.58025,81.84309)
  -- (187.91023,81.90309)
  -- (188.05025,81.82310)
  -- (188.31023,81.92309)
  -- (188.39023,81.84309)
  -- (188.50024,81.89310)
  -- (188.62022,81.83310)
  -- (188.84023,81.91310)
  -- (188.87024,81.77310)
  -- (188.90024,81.93308)
  -- (189.04022,81.82310)
  -- (189.23024,81.90309)
  -- (189.32025,81.85310)
  -- (189.68024,81.84309)
  -- (190.19025,81.96310)
  -- (190.30025,81.90309)
  -- (190.61024,81.89310)
  -- (190.83025,82.04308)
  -- (191.11023,81.89310)
  -- (191.28024,81.94310)
  -- (191.70024,81.88310)
  -- (192.12024,81.93308)
  -- (192.41025,81.83310)
  -- (192.55025,81.88310)
  -- (192.71024,81.83310)
  -- (192.94025,81.94310)
  -- (193.67024,81.79308)
  -- (194.01024,81.84309)
  -- (194.37024,81.78310)
  -- (194.43024,82.04308)
  -- (194.46025,81.79308)
  -- (194.48024,82.13310)
  -- (194.57025,81.75309)
  -- (194.60027,81.87310)
  -- (194.65024,81.71310)
  -- (194.79024,81.98310)
  -- (194.93024,81.81309)
  -- (194.99025,81.85310)
  -- (195.21025,81.80311)
  -- (195.30025,81.65309)
  -- (195.41025,81.75309)
  -- (195.61024,81.74310)
  -- (195.63025,81.85310)
  -- (195.66025,81.77310)
  -- (195.80026,81.72310)
  -- (196.00026,81.91310)
  -- (196.08025,81.87310)
  -- (196.39024,82.02310)
  -- (196.79024,81.87310)
  -- (197.80026,81.97310)
  -- (197.96027,81.92309)
  -- (198.78026,81.90309)
  -- (199.26024,81.92309)
  -- (199.42024,82.00310)
  -- (199.51024,81.92309)
  -- (199.59024,82.01309)
  -- (199.65025,81.95309)
  -- (200.46025,82.00310)
  -- (202.12025,81.93308)
  -- (202.35027,81.95309)
  -- (202.43025,82.07311)
  -- (202.51024,81.92309)
  -- (202.54025,82.05310)
  -- (202.57027,81.82310)
  -- (202.60027,82.09310)
  -- (202.63026,81.94310)
  -- (202.65025,82.07311)
  -- (202.77026,81.98310)
  -- (202.91025,82.06309)
  -- (203.13025,82.03309)
  -- (203.16026,81.97310)
  -- (203.19026,82.06309)
  -- (203.22025,81.99310)
  -- (203.30026,82.06309)
  -- (204.03026,82.01309)
  -- (204.09026,82.06309)
  -- (204.65025,81.99310)
  -- (204.68025,82.08310)
  -- (204.70026,82.03309)
  -- (205.24026,82.05310)
  -- (205.71027,81.99310)
  -- (206.84026,82.09310)
  -- (207.06026,82.01309)
  -- (207.51025,81.99310)
  -- (207.90025,82.11309)
  -- (207.93025,82.02310)
  -- (207.96028,82.08310)
  -- (208.33026,81.93308)
  -- (208.63026,81.91310)
  -- (208.94028,81.97310)
  -- (209.06026,82.18310)
  -- (209.14027,82.03309)
  -- (209.17026,82.19310)
  -- (209.20026,82.10310)
  -- (209.42026,82.22310)
  -- (209.84026,81.99310)
  -- (210.01025,81.95309)
  -- (210.09027,82.00310)
  -- (210.12027,81.87310)
  -- (210.21028,82.07311)
  -- (210.23027,81.89310)
  -- (210.26025,82.01309)
  -- (210.29027,81.94310)
  -- (210.52028,82.04308)
  -- (211.02026,82.07311)
  -- (211.61028,82.02310)
  -- (211.84026,82.08310)
  -- (211.95026,81.95309)
  -- (212.06026,82.00310)
  -- (212.12027,81.91310)
  -- (212.26025,82.03309)
  -- (212.51025,81.98310)
  -- (212.82027,82.02310)
  -- (213.04025,82.14309)
  -- (213.27028,82.15309)
  -- (213.44026,82.09310)
  -- (213.58028,82.15309)
  -- (213.80028,82.05310)
  -- (213.88028,82.15309)
  -- (214.87027,81.96310)
  -- (215.32028,82.06309)
  -- (215.51025,82.01309)
  -- (215.60028,82.06309)
  -- (215.63028,82.26309)
  -- (215.65027,81.95309)
  -- (215.68027,82.16311)
  -- (215.77028,81.93308)
  -- (215.79027,82.09310)
  -- (215.93027,82.00310)
  -- (216.02028,82.13310)
  -- (216.13028,82.04308)
  -- (216.41028,82.18310)
  -- (216.83028,82.12309)
  -- (217.06027,82.35310)
  -- (217.37027,82.19310)
  -- (217.51027,82.30310)
  -- (217.93027,82.06309)
  -- (218.12027,82.21310)
  -- (218.43027,82.06309)
  -- (218.63028,82.23309)
  -- (218.88028,82.11309)
  -- (219.22028,82.19310)
  -- (219.56029,82.06309)
  -- (219.89029,82.15309)
  -- (220.12027,82.07311)
  -- (220.45029,82.18310)
  -- (220.68027,82.11309)
  -- (220.82028,82.18310)
  -- (221.18028,82.10310)
  -- (221.30028,82.18310)
  -- (221.69029,82.11309)
  -- (221.91028,82.19310)
  -- (222.08028,82.12309)
  -- (222.31027,82.17309)
  -- (222.34029,82.08310)
  -- (222.36029,82.19310)
  -- (222.42027,82.12309)
  -- (222.45029,82.18310)
  -- (222.64027,82.12309)
  -- (223.77030,82.19310)
  -- (223.99030,82.13310)
  -- (224.30030,82.16311)
  -- (224.33028,82.23309)
  -- (224.36029,82.09310)
  -- (224.39029,82.23309)
  -- (224.41030,82.10310)
  -- (224.50029,82.25309)
  -- (225.71028,82.11309)
  -- (226.15028,82.25309)
  -- (226.88030,82.16311)
  -- (227.81029,82.22310)
  -- (227.95029,82.14309)
  -- (228.04028,82.23309)
  -- (228.06029,82.17309)
  -- (228.12029,82.35310)
  -- (228.20029,82.17309)
  -- (228.32030,82.23309)
  -- (228.49031,82.16311)
  -- (228.54028,82.23309)
  -- (228.65028,82.17309)
  -- (228.68028,82.26309)
  -- (228.71030,82.19310)
  -- (228.85030,82.25309)
  -- (230.76030,82.18310)
  -- (230.98030,82.25309)
  -- (231.07031,82.11309)
  -- (231.15028,82.26309)
  -- (231.24030,82.12309)
  -- (231.26028,82.18310)
  -- (231.35030,82.13310)
  -- (231.43028,82.19310)
  -- (231.60031,82.11309)
  -- (231.71030,82.18310)
  -- (231.85031,82.15309)
  -- (231.88030,82.21310)
  -- (231.91030,82.14309)
  -- (231.97029,82.20309)
  -- (231.99030,82.14309)
  -- (232.16031,82.17309)
  -- (232.39029,82.13310)
  -- (232.42029,82.07311)
  -- (232.44029,82.12309)
  -- (232.53029,82.03309)
  -- (232.56030,82.08310)
  -- (232.58030,82.03309)
  -- (232.64029,82.15309)
  -- (232.67030,81.98310)
  -- (232.81029,82.31309)
  -- (232.84029,82.01309)
  -- (232.86029,82.28309)
  -- (232.89030,82.08310)
  -- (232.98030,82.15309)
  -- (233.01030,82.07311)
  -- (233.03030,82.14309)
  -- (233.15028,82.14309)
  -- (233.29030,82.25309)
  -- (233.43030,82.20309)
  -- (233.99031,82.20309)
  -- (234.44029,82.08310)
  -- (235.25030,82.20309)
  -- (235.67030,82.14309)
  -- (236.07031,82.23309)
  -- (236.46031,82.23309)
  -- (236.49031,82.46310)
  -- (236.52031,81.74310)
  -- (236.54030,82.54308)
  -- (236.57031,81.89310)
  -- (236.60031,82.25309)
  -- (236.66031,81.78310)
  -- (236.82030,82.21310)
  -- (236.88031,82.02310)
  -- (236.91030,82.24310)
  -- (236.99031,81.96310)
  -- (237.02030,82.02310)
  -- (237.05031,81.96310)
  -- (237.08030,82.10310)
  -- (237.10031,81.93308)
  -- (237.22029,82.13310)
  -- (237.25030,82.05310)
  -- (237.27031,82.20309)
  -- (237.30031,82.04308)
  -- (237.33029,82.18310)
  -- (237.47030,82.06309)
  -- (237.58030,82.20309)
  -- (237.64030,82.13310)
  -- (237.72030,82.18310)
  -- (237.86030,82.07311)
  -- (238.03030,82.15309)
  -- (238.09030,82.12309)
  -- (238.12030,82.20309)
  -- (238.14030,82.14309)
  -- (238.62030,82.12309)
  -- (238.87030,82.24310)
  -- (239.10031,82.18310)
  -- (239.29030,82.36310)
  -- (239.58030,82.29310)
  -- (239.63031,82.35310)
  -- (239.80032,82.31309)
  -- (240.17030,82.43308)
  -- (240.39030,82.33310)
  -- (240.59030,82.55310)
  -- (240.90030,82.36310)
  -- (241.12030,82.43308)
  -- (241.26030,82.34309)
  -- (241.68030,82.26309)
  -- (242.52031,82.35310)
  -- (243.65031,82.28309)
  -- (244.57031,82.39309)
  -- (244.94032,82.37309)
  -- (245.08030,82.29310)
  -- (245.61032,82.28309)
  -- (245.92032,82.32310)
  -- (245.95030,82.44310)
  -- (245.98032,82.22310)
  -- (246.01031,82.38311)
  -- (246.03032,82.31309)
  -- (246.26030,82.35310)
  -- (246.57033,82.28309)
  -- (247.89032,82.37309)
  -- (248.00032,82.33310)
  -- (248.20030,82.39309)
  -- (249.21033,82.33310)
  -- (249.29031,82.27311)
  -- (249.40030,82.45309)
  -- (249.74033,82.26309)
  -- (249.91032,82.35310)
  -- (250.97032,82.37309)
  -- (251.87032,82.30310)
  -- (251.99033,82.33310)
  -- (252.04031,82.27311)
  -- (252.24033,82.32310)
  -- (252.27034,82.26309)
  -- (252.29033,82.34309)
  -- (252.32033,82.25309)
  -- (252.35033,82.37309)
  -- (252.38034,82.31309)
  -- (252.58034,82.31309)
  -- (252.80034,82.41310)
  -- (252.94032,82.34309)
  -- (253.92032,82.30310)
  -- (254.40031,82.39309)
  -- (254.46033,82.35310)
  -- (254.57033,82.41310)
  -- (254.82033,82.40309)
  -- (255.05034,82.38311)
  -- (255.27034,82.26309)
  -- (255.58034,82.34309)
  -- (255.69034,82.29310)
  -- (256.34033,82.39309)
  -- (256.62032,82.29310)
  -- (256.65033,82.32310)
  -- (256.79033,82.08310)
  -- (256.90033,82.13310)
  -- (256.93031,82.01309)
  -- (256.96034,82.21310)
  -- (256.98033,82.08310)
  -- (257.01033,82.13310)
  -- (257.21034,81.96310)
  -- (257.60034,82.13310)
  -- (257.63034,82.09310)
  -- (258.11032,82.16311)
  -- (258.19034,82.67310)
  -- (258.22032,82.24310)
  -- (258.25034,82.47311)
  -- (258.36034,82.09310)
  -- (258.39034,82.22310)
  -- (258.44032,82.09310)
  -- (258.47034,82.35310)
  -- (258.50034,82.17309)
  -- (258.53032,82.31309)
  -- (258.56033,82.25309)
  -- (258.67033,82.34309)
  -- (258.70033,82.22310)
  -- (258.72034,82.43308)
  -- (258.75032,82.27311)
  -- (258.78033,82.32310)
  -- (258.86034,82.23309)
  -- (259.15033,82.13310)
  -- (259.65033,82.22310)
  -- (259.79033,82.32310)
  -- (259.85034,82.25309)
  -- (259.96034,82.26309)
  -- (259.99034,82.32310)
  -- (260.10034,82.24310)
  -- (260.94034,82.28309)
  -- (261.31033,82.17309)
  -- (261.36034,82.21310)
  -- (261.67033,81.98310)
  -- (261.84033,82.06309)
  -- (261.87033,82.14309)
  -- (261.90033,81.87310)
  -- (261.93033,82.11309)
  -- (262.04033,82.08310)
  -- (262.07034,82.18310)
  -- (262.09033,82.04308)
  -- (262.12033,82.20309)
  -- (262.15033,82.08310)
  -- (262.18033,82.19310)
  -- (262.21034,82.09310)
  -- (262.23033,82.19310)
  -- (262.46034,82.12309)
  -- (262.57034,82.22310)
  -- (262.82034,82.12309)
  -- (263.16034,82.16311)
  -- (263.19034,82.21310)
  -- (263.39034,82.11309)
  -- (263.61034,82.11309)
  -- (263.64034,82.17309)
  -- (263.67035,82.11309)
  -- (263.69035,82.69311)
  -- (263.72034,81.80311)
  -- (263.75034,82.60311)
  -- (263.78035,82.06309)
  -- (263.89035,82.26309)
  -- (264.00035,82.14309)
  -- (264.03033,82.25309)
  -- (264.06033,82.16311)
  -- (264.14034,82.20309)
  -- (264.48033,82.13310)
  -- (264.70033,82.17309)
  -- (265.07036,82.13310)
  -- (265.32034,82.23309)
  -- (265.97034,82.36310)
  -- (266.11034,82.31309)
  -- (266.42033,82.39309)
  -- (266.61034,82.30310)
  -- (266.84033,82.40309)
  -- (267.40033,82.16311)
  -- (267.54034,82.23309)
  -- (267.82034,82.22310)
  -- (267.99034,82.14309)
  -- (268.21036,82.17309)
  -- (268.30035,82.11309)
  -- (268.61035,82.14309)
  -- (268.75034,82.08310)
  -- (269.62033,82.05310)
  -- (269.73033,82.17309)
  -- (269.81035,82.01309)
  -- (269.84033,82.12309)
  -- (269.93033,82.00310)
  -- (270.07036,82.06309)
  -- (270.18034,81.97310)
  -- (270.26035,82.05310)
  -- (270.60036,81.88310)
  -- (270.77036,81.87310)
  -- (270.99036,81.86309)
  -- (271.08035,81.94310)
  -- (271.22034,81.82310)
  -- (271.58035,81.94310)
  -- (271.75035,81.86309)
  -- (272.48035,81.89310)
  -- (273.24036,81.83310)
  -- (273.46036,81.86309)
  -- (273.52036,81.93308)
  -- (273.55035,81.82310)
  -- (273.61035,81.89310)
  -- (273.63036,81.81309)
  -- (273.91035,81.92309)
  -- (274.03035,81.84309)
  -- (274.39035,81.84309)
  -- (274.50035,81.76309)
  -- (274.62035,81.88310)
  -- (274.64035,81.71310)
  -- (274.70035,81.88310)
  -- (274.73035,81.77310)
  -- (274.76035,81.86309)
  -- (274.78036,81.79308)
  -- (274.84035,81.87310)
  -- (274.87035,81.80311)
  -- (275.04034,81.79308)
  -- (275.57036,81.88310)
  -- (276.02036,81.85310)
  -- (276.41035,81.93308)
  -- (276.64035,82.14309)
  -- (276.92035,82.28309)
  -- (277.06035,82.26309)
  -- (277.23036,82.35310)
  -- (277.48035,82.31309)
  -- (278.58037,82.52310)
  -- (279.50037,82.33310)
  -- (280.43036,82.45309)
  -- (281.52037,82.31309)
  -- (281.83037,82.36310)
  -- (282.23036,82.23309)
  -- (282.73035,82.35310)
  -- (282.90036,82.30310)
  -- (283.29036,82.45309)
  -- (284.75037,82.42309)
  -- (285.79036,82.50309)
  -- (286.18037,82.44310)
  -- (287.64037,82.50309)
  -- (288.77037,82.46310)
  -- (289.72038,82.55310)
  -- (290.87038,82.48309)
  -- (292.45038,82.56310)
  -- (292.70038,82.47311)
  -- (293.43037,82.52310)
  -- (293.99039,82.66310)
  -- (295.03038,82.70309)
  -- (296.85039,82.44310)
  -- (297.11038,82.47311)
  -- (297.36038,82.36310)
  -- (298.31038,82.45309)
  -- (298.68037,82.37309)
  -- (299.38040,82.35310)
  -- (299.46039,82.41310)
  -- (299.89040,82.46310)
  -- (300.11038,82.38311)
  -- (301.37038,82.60311)
  -- (302.64038,82.51309)
  -- (302.97038,82.44310)
  -- (303.31038,82.46310)
  -- (303.76039,82.34309)
  -- (305.05040,82.52310)
  -- (306.12039,82.42309)
  -- (306.91040,82.42309)
  -- (307.10040,82.35310)
  -- (308.56040,82.38311)
  -- (309.07040,82.28309)
  -- (309.24040,82.41310)
  -- (309.26039,82.31309)
  -- (309.29040,82.44310)
  -- (309.38042,82.28309)
  -- (309.43039,82.36310)
  -- (309.46040,82.29310)
  -- (309.57040,82.32310)
  -- (309.60042,82.24310)
  -- (309.74040,82.38311)
  -- (310.11040,82.28309)
  -- (310.98041,82.53309)
  -- (311.45041,82.50309)
  -- (312.83041,82.57310)
  -- (313.05042,82.50309)
  -- (314.82040,82.46310)
  -- (315.30042,82.35310)
  -- (316.09041,82.38311)
  -- (316.79040,82.30310)
  -- (321.51040,82.55310)
  -- (322.24042,82.44310)
  -- (322.85043,82.45309)
  -- (323.36043,82.38311)
  -- (323.70041,82.38311)
  -- (323.89043,82.47311)
  -- (324.45042,82.52310)
  -- (325.21043,82.41310)
  -- (326.39043,82.46310)
  -- (327.01042,82.35310)
  -- (327.04040,82.50309)
  -- (327.06042,82.37309)
  -- (327.12042,82.48309)
  -- (327.15040,82.40309)
  -- (327.21043,82.50309)
  -- (327.32043,82.35310)
  -- (327.37042,82.43308)
  -- (327.63043,82.34309)
  -- (327.65042,82.42309)
  -- (327.91042,82.50309)
  -- (327.99043,82.36310)
  -- (328.22041,82.50309)
  -- (328.55043,82.42309)
  -- (328.89043,82.50309)
  -- (329.06042,82.47311)
  -- (329.17043,82.55310)
  -- (329.23042,82.46310)
  -- (329.31041,82.54308)
  -- (329.59042,82.45309)
  -- (329.87042,82.49311)
  -- (330.43042,82.32310)
  -- (330.46043,82.24310)
  -- (330.52043,82.29310)
  -- (330.55043,82.24310)
  -- (330.97043,82.34309)
  -- (331.02043,82.56310)
  -- (331.05043,82.47311)
  -- (331.11043,82.58311)
  -- (331.14043,82.49311)
  -- (331.19043,82.62309)
  -- (331.22043,82.56310)
  -- (331.33043,82.60311)
  -- (331.59042,82.52310)
  -- (331.70042,82.54308)
  -- (331.75043,82.47311)
  -- (331.78044,82.52310)
  -- (331.89044,82.42309)
  -- (332.06042,82.49311)
  -- (332.09044,82.41310)
  -- (332.17043,82.45309)
  -- (332.26042,82.34309)
  -- (332.43042,82.31309)
  -- (333.24043,82.39309)
  -- (333.35043,82.42309)
  -- (333.38045,82.50309)
  -- (333.58044,82.47311)
  -- (334.08043,82.61309)
  -- (334.76044,82.49311)
  -- (335.01042,82.52310)
  -- (335.12044,82.59309)
  -- (335.15042,82.53309)
  -- (335.35043,82.65310)
  -- (335.57043,82.55310)
  -- (335.68042,82.57310)
  -- (335.80045,82.44310)
  -- (335.85045,82.50309)
  -- (335.97043,82.40309)
  -- (336.13043,82.38311)
  -- (336.25044,82.46310)
  -- (336.58044,82.41310)
  -- (336.70044,82.55310)
  -- (336.78044,82.47311)
  -- (336.81044,82.67310)
  -- (336.89044,82.51309)
  -- (336.92044,82.62309)
  -- (336.95042,82.50309)
  -- (336.98044,82.63310)
  -- (337.00044,82.48309)
  -- (337.03044,82.57310)
  -- (337.09044,82.49311)
  -- (337.14044,82.55310)
  -- (337.28044,82.49311)
  -- (337.37042,82.58311)
  -- (337.57043,82.61309)
  -- (337.76044,82.44310)
  -- (338.04042,82.49311)
  -- (338.18044,82.41310)
  -- (338.44043,82.49311)
  -- (338.77045,82.42309)
  -- (339.14044,82.51309)
  -- (340.09044,82.57310)
  -- (340.15044,82.68308)
  -- (340.29044,82.53309)
  -- (340.40042,82.58311)
  -- (341.27045,82.57310)
  -- (341.92044,82.48309)
  -- (342.65044,82.57310)
  -- (343.77045,82.48309)
  -- (347.28044,82.61309)
  -- (348.35045,82.52310)
  -- (348.63046,82.65310)
  -- (348.94046,82.52310)
  -- (349.13045,82.54308)
  -- (349.39046,82.41310)
  -- (349.72046,82.51309)
  -- (350.14046,82.55310)
  -- (350.79045,82.45309)
  -- (351.69046,82.61309)
  -- (351.72046,82.55310)
  -- (351.77046,82.59309)
  -- (352.19046,82.41310)
  -- (352.87045,82.53309)
  -- (353.09045,82.38311)
  -- (353.37045,82.51309)
  -- (353.65045,82.38311)
  -- (353.82047,82.46310)
  -- (354.24046,82.43308)
  -- (354.97046,82.63310)
  -- (355.56047,82.54308)
  -- (356.46046,82.67310)
  -- (356.74048,82.63310)
  -- (358.06046,82.67310)
  -- (358.26045,82.59309)
  -- (358.48045,82.64309)
  -- (359.04045,82.60311)
  -- (359.27048,82.67310)
  -- (359.52048,82.59309)
  -- (360.22046,82.59309)
  -- (361.04045,82.48309)
  -- (362.13046,82.53309)
  -- (362.50047,82.47311)
  -- (363.68047,82.54308)
  -- (363.79047,82.50309)
  -- (363.82048,82.55310)
  -- (363.85048,82.50309)
  -- (364.07048,82.57310)
  -- (364.10048,82.51309)
  -- (364.21048,82.57310)
  -- (364.46048,82.54308)
  -- (365.05048,82.70309)
  -- (365.70047,82.68308)
  -- (367.61047,82.86309)
  -- (368.39047,82.85311)
  -- (369.43048,83.05311)
  -- (370.50049,83.02310)
  -- (370.72049,83.08310)
  -- (370.92049,83.02310)
  -- (371.01048,83.09310)
  -- (371.12048,83.04308)
  -- (371.20047,83.12309)
  -- (372.16049,83.08310)
  -- (373.25049,83.18310)
  -- (373.79048,83.12309)
  -- (374.35050,83.18310)
  -- (374.43048,83.47311)
  -- (374.60050,83.04308)
  -- (374.74050,83.16311)
  -- (374.77050,83.11309)
  -- (374.99050,83.12309)
  -- (375.08049,83.02310)
  -- (375.19049,83.06309)
  -- (375.27050,83.27311)
  -- (375.30049,83.16311)
  -- (375.39049,83.26309)
  -- (375.50049,83.12309)
  -- (375.53049,83.17309)
  -- (375.64049,83.09310)
  -- (375.81049,83.14310)
  -- (375.89049,83.24310)
  -- (376.06049,83.07311)
  -- (376.17049,83.19310)
  -- (376.28049,83.08310)
  -- (376.42049,83.19310)
  -- (376.51048,83.04308)
  -- (376.59048,83.19310)
  -- (376.71050,83.11309)
  -- (376.87048,83.13310)
  -- (376.96050,83.08310)
  -- (376.99050,83.14310)
  -- (377.21050,83.07311)
  -- (377.24050,83.14310)
  -- (377.35050,83.13310)
  -- (377.38051,83.06309)
  -- (377.41049,83.16311)
  -- (377.44049,83.10310)
  -- (377.55049,83.20309)
  -- (377.60051,83.10310)
  -- (377.83049,83.12309)
  -- (377.86049,83.17309)
  -- (377.91049,83.06309)
  -- (377.94049,83.18310)
  -- (378.03049,83.12309)
  -- (378.05049,83.21310)
  -- (378.08049,83.05311)
  -- (378.22049,83.44310)
  -- (378.31049,83.40309)
  -- (378.36050,82.93308)
  -- (378.47050,83.33310)
  -- (378.53049,83.07311)
  -- (378.56050,83.17309)
  -- (378.59048,83.05311)
  -- (378.61049,83.29310)
  -- (378.70049,83.01309)
  -- (378.76050,83.18310)
  -- (378.81049,83.19310)
  -- (378.90048,83.08310)
  -- (378.95049,83.13310)
  -- (378.98050,83.04308)
  -- (379.01048,83.16311)
  -- (379.12048,83.03309)
  -- (379.20049,83.18310)
  -- (379.23048,83.05311)
  -- (379.32050,83.85311)
  -- (379.40048,83.05311)
  -- (379.43048,83.31309)
  -- (379.46050,82.99310)
  -- (379.49051,83.38311)
  -- (379.51048,82.96311)
  -- (379.54050,83.24310)
  -- (379.63050,83.05311)
  -- (379.68048,83.31309)
  -- (379.74051,82.97310)
  -- (379.79048,83.32310)
  -- (379.88050,83.04308)
  -- (379.93048,83.24310)
  -- (380.02050,82.91310)
  -- (380.05050,83.42309)
  -- (380.07051,83.02310)
  -- (380.19049,83.27311)
  -- (380.22049,83.07311)
  -- (380.24050,83.31309)
  -- (380.27051,83.18310)
  -- (380.30049,83.25310)
  -- (380.33049,83.15309)
  -- (380.36050,83.24310)
  -- (380.41049,83.04308)
  -- (380.44049,83.16311)
  -- (380.52051,83.09310)
  -- (380.69050,83.21310)
  -- (380.86049,83.12309)
  -- (381.00050,83.19310)
  -- (381.28049,83.13310)
  -- (381.37048,83.19310)
  -- (381.62048,83.19310)
  -- (381.73048,83.12309)
  -- (382.04048,83.19310)
  -- (382.71050,83.14310)
  -- (382.77050,83.21310)
  -- (382.83050,83.16311)
  -- (383.14050,83.14310)
  -- (388.95050,83.16311);
% Reference trace 24
\path[draw={rgb,1:red,0.584;green,0.326;blue,0.181},line width=0.32877bp] (113.26013,81.51309)
  -- (114.72014,81.48309)
  -- (114.86014,81.55310)
  -- (115.05014,81.48309)
  -- (115.17014,81.52310)
  -- (116.29015,81.50309)
  -- (116.43013,81.57310)
  -- (116.60016,81.43308)
  -- (116.82014,81.54308)
  -- (116.93013,81.47311)
  -- (117.13014,81.56309)
  -- (117.36015,81.43308)
  -- (117.58015,81.55310)
  -- (117.78015,81.48309)
  -- (118.14015,81.48309)
  -- (118.31013,81.54308)
  -- (118.56015,81.47311)
  -- (118.79013,81.54308)
  -- (119.01015,81.47311)
  -- (119.15013,81.53309)
  -- (119.69016,81.48309)
  -- (119.77014,81.28309)
  -- (119.94016,81.83310)
  -- (120.16016,81.21310)
  -- (120.36015,81.76309)
  -- (120.58015,81.24310)
  -- (120.75014,81.74310)
  -- (121.06013,81.36309)
  -- (121.23015,81.61309)
  -- (121.48015,81.46310)
  -- (121.74016,81.54308)
  -- (122.07016,81.48309)
  -- (122.30016,81.54308)
  -- (122.63016,81.34309)
  -- (122.94016,81.38311)
  -- (123.50015,81.77310)
  -- (123.56015,81.73309)
  -- (123.78015,81.85310)
  -- (123.95015,81.84309)
  -- (124.01015,81.77310)
  -- (124.99016,81.45309)
  -- (125.44016,81.74310)
  -- (125.53015,81.71310)
  -- (125.86015,82.11309)
  -- (126.00017,82.08310)
  -- (126.31015,82.60311)
  -- (126.40015,82.48309)
  -- (126.42015,82.53309)
  -- (126.48015,82.49311)
  -- (126.79015,82.97310)
  -- (126.99016,82.58311)
  -- (127.21016,82.84309)
  -- (127.46016,82.62309)
  -- (127.77016,82.96311)
  -- (128.19016,82.84309)
  -- (128.36017,82.86309)
  -- (128.42015,82.95309)
  -- (128.50015,82.84309)
  -- (128.53015,82.94310)
  -- (128.59015,82.83310)
  -- (128.64015,82.92309)
  -- (129.04015,83.03309)
  -- (129.29016,82.95309)
  -- (129.51015,82.98310)
  -- (129.65016,83.15309)
  -- (129.82016,82.81309)
  -- (130.24016,82.91310)
  -- (130.38017,82.88310)
  -- (130.66016,83.03309)
  -- (130.80017,82.88310)
  -- (130.86015,82.93308)
  -- (130.94017,82.79308)
  -- (131.14017,83.16311)
  -- (131.34016,82.77310)
  -- (131.59016,83.10310)
  -- (131.73015,82.85311)
  -- (131.90016,83.26309)
  -- (132.04015,82.79308)
  -- (132.29016,83.04308)
  -- (132.43016,82.95309)
  -- (133.08017,83.03309)
  -- (133.78017,82.85311)
  -- (133.95016,82.88310)
  -- (134.43016,82.82310)
  -- (135.04016,82.65310)
  -- (135.35017,82.77310)
  -- (135.89017,82.81309)
  -- (136.14017,82.71310)
  -- (136.56017,82.64309)
  -- (137.12016,82.73309)
  -- (137.49019,82.61309)
  -- (137.68016,82.66310)
  -- (137.77017,82.61309)
  -- (138.67018,82.61309)
  -- (139.42017,82.47311)
  -- (139.59016,82.49311)
  -- (139.93016,82.36310)
  -- (140.29018,82.31309)
  -- (140.77017,82.42309)
  -- (141.45018,82.44310)
  -- (142.04016,82.34309)
  -- (142.82018,82.41310)
  -- (143.19019,82.33310)
  -- (143.58018,82.44310)
  -- (143.92018,82.33310)
  -- (144.59018,82.26309)
  -- (144.79018,82.30310)
  -- (145.29018,82.19310)
  -- (146.33018,82.21310)
  -- (146.53018,82.27311)
  -- (147.03018,82.23309)
  -- (147.20016,82.14309)
  -- (148.72018,82.11309)
  -- (148.80020,81.89310)
  -- (148.89020,82.15309)
  -- (149.00020,82.01309)
  -- (149.19019,82.24310)
  -- (149.34018,82.30310)
  -- (150.40018,82.10310)
  -- (150.96020,82.19310)
  -- (151.24019,82.18310)
  -- (151.30019,82.13310)
  -- (151.44019,82.19310)
  -- (151.53018,82.02310)
  -- (151.67020,82.18310)
  -- (151.81018,82.00310)
  -- (151.89020,82.12309)
  -- (151.95018,82.07311)
  -- (152.06018,82.17309)
  -- (152.17018,82.18310)
  -- (152.28018,82.08310)
  -- (152.34020,82.17309)
  -- (152.51018,82.12309)
  -- (153.77019,82.28309)
  -- (153.86018,82.20309)
  -- (153.91019,82.22310)
  -- (154.02019,82.00310)
  -- (154.36020,82.08310)
  -- (154.61020,81.96310)
  -- (155.15018,82.14309)
  -- (155.93018,82.19310)
  -- (156.16020,82.34309)
  -- (156.49020,82.28309)
  -- (157.08020,82.61309)
  -- (157.25020,82.57310)
  -- (157.87020,82.72310)
  -- (158.21020,82.66310)
  -- (158.46020,82.53309)
  -- (158.85020,82.75309)
  -- (159.16020,82.62309)
  -- (159.27020,82.69311)
  -- (159.39020,82.56310)
  -- (159.75020,82.66310)
  -- (160.34020,82.52310)
  -- (160.71020,82.52310)
  -- (161.16020,82.69311)
  -- (161.63020,82.72310)
  -- (161.69022,82.93308)
  -- (161.77020,82.83310)
  -- (161.83020,83.36310)
  -- (161.91020,82.51309)
  -- (161.94020,82.68308)
  -- (161.97020,82.61309)
  -- (162.03020,82.77310)
  -- (162.05020,82.68308)
  -- (162.31020,82.75309)
  -- (162.48020,82.59309)
  -- (162.50020,82.65310)
  -- (162.59020,82.63310)
  -- (162.62020,82.54308)
  -- (162.64020,82.63310)
  -- (162.70020,82.55310)
  -- (162.73020,82.63310)
  -- (162.87021,82.65310)
  -- (162.92020,82.53309)
  -- (163.15019,82.75309)
  -- (163.18020,82.66310)
  -- (163.26020,82.94310)
  -- (163.40019,82.74310)
  -- (163.43020,82.83310)
  -- (163.49022,82.82310)
  -- (163.74022,82.66310)
  -- (164.16022,82.98310)
  -- (164.33020,82.77310)
  -- (164.44020,82.77310)
  -- (164.61021,82.54308)
  -- (164.67021,82.55310)
  -- (164.78021,82.88310)
  -- (164.92021,82.81309)
  -- (165.09021,82.93308)
  -- (165.20020,82.85311)
  -- (165.48020,82.79308)
  -- (165.68019,82.81309)
  -- (165.84020,82.94310)
  -- (166.24020,82.91310)
  -- (166.38022,82.83310)
  -- (166.63022,82.98310)
  -- (167.39021,82.89310)
  -- (167.53020,82.99310)
  -- (167.87021,82.96311)
  -- (168.12021,83.06309)
  -- (168.23021,82.99310)
  -- (168.57022,83.06309)
  -- (168.68020,83.00310)
  -- (168.93019,83.03309)
  -- (169.30022,82.98310)
  -- (169.52022,82.87310)
  -- (169.94022,83.06309)
  -- (170.20020,82.98310)
  -- (170.53021,83.05311)
  -- (171.49023,82.94310)
  -- (171.83022,83.00310)
  -- (172.11021,82.93308)
  -- (172.47021,82.92309)
  -- (172.72021,82.82310)
  -- (172.81021,82.85311)
  -- (172.84021,82.78310)
  -- (173.03021,82.77310)
  -- (173.40020,82.91310)
  -- (173.82022,82.95309)
  -- (174.04020,83.06309)
  -- (174.38023,82.98310)
  -- (174.69023,83.06309)
  -- (175.14023,83.04308)
  -- (175.92023,82.81309)
  -- (176.29022,83.03309)
  -- (176.71022,82.95309)
  -- (177.24022,82.99310)
  -- (177.52023,83.10310)
  -- (177.83023,83.11309)
  -- (178.28023,82.92309)
  -- (178.48022,82.95309)
  -- (178.68022,83.09310)
  -- (179.01022,83.14310)
  -- (179.24022,83.14310)
  -- (179.52023,83.01309)
  -- (179.97023,83.04308)
  -- (180.16023,83.13310)
  -- (180.98022,83.14310)
  -- (181.51021,82.99310)
  -- (182.63023,83.12309)
  -- (183.70023,83.07311)
  -- (184.88023,83.13310)
  -- (185.19023,83.04308)
  -- (185.50023,83.10310)
  -- (185.75023,83.04308)
  -- (186.48022,83.14310)
  -- (186.73022,83.08310)
  -- (187.30023,83.13310)
  -- (187.35023,83.19310)
  -- (187.41025,83.14310)
  -- (187.55023,83.19310)
  -- (187.77023,83.14310)
  -- (188.05025,83.23309)
  -- (188.31023,83.09310)
  -- (188.47025,83.07311)
  -- (188.59024,83.14310)
  -- (188.81024,83.04308)
  -- (188.90024,83.10310)
  -- (188.92024,83.03309)
  -- (189.06023,83.19310)
  -- (189.63025,83.17309)
  -- (189.91023,83.03309)
  -- (190.58025,83.04308)
  -- (190.81024,82.89310)
  -- (191.06024,83.12309)
  -- (191.31023,83.01309)
  -- (191.73022,83.13310)
  -- (192.12024,83.13310)
  -- (192.38025,83.22310)
  -- (192.60025,83.15309)
  -- (192.71024,83.17309)
  -- (192.94025,82.94310)
  -- (193.28024,82.97310)
  -- (193.73024,83.16311)
  -- (193.98024,83.03309)
  -- (194.17024,83.14310)
  -- (194.37024,83.14310)
  -- (194.46025,84.61309)
  -- (194.57025,82.63310)
  -- (194.65024,83.52310)
  -- (194.76024,82.75309)
  -- (194.88025,83.31309)
  -- (194.96025,82.97310)
  -- (195.07025,83.20309)
  -- (195.19025,82.96311)
  -- (195.30025,83.17309)
  -- (195.49026,83.00310)
  -- (195.61024,83.09310)
  -- (195.66025,83.75309)
  -- (195.77025,82.85311)
  -- (195.89026,83.30310)
  -- (196.00026,82.94310)
  -- (196.11024,83.18310)
  -- (196.22025,83.02310)
  -- (196.31024,83.15309)
  -- (196.45026,82.97310)
  -- (196.73024,83.14310)
  -- (196.84024,83.05311)
  -- (196.95024,83.13310)
  -- (197.71025,83.05311)
  -- (197.88025,83.12309)
  -- (198.30025,83.07311)
  -- (199.20024,83.12309)
  -- (199.34026,83.04308)
  -- (199.42024,83.22310)
  -- (199.54025,82.88310)
  -- (199.62024,83.28309)
  -- (199.76025,82.99310)
  -- (199.90025,83.13310)
  -- (200.04024,83.06309)
  -- (201.98026,83.14310)
  -- (202.32027,83.08310)
  -- (202.43025,83.73309)
  -- (202.51024,82.23309)
  -- (202.65025,83.57310)
  -- (202.79025,82.76310)
  -- (202.88026,83.19310)
  -- (203.02025,83.05311)
  -- (203.19026,83.12309)
  -- (203.27026,83.04308)
  -- (203.47026,83.12309)
  -- (204.39026,83.02310)
  -- (204.59026,83.11309)
  -- (204.65025,83.01309)
  -- (204.82027,83.12309)
  -- (205.04025,83.06309)
  -- (205.18025,83.11309)
  -- (205.27026,83.03309)
  -- (205.43025,83.13310)
  -- (205.57027,82.97310)
  -- (205.71027,83.13310)
  -- (205.80028,83.15309)
  -- (205.94026,83.00310)
  -- (206.05026,83.17309)
  -- (206.22026,82.97310)
  -- (206.36026,83.13310)
  -- (206.53026,83.03309)
  -- (206.61026,83.10310)
  -- (206.75026,82.99310)
  -- (206.87027,83.15309)
  -- (207.01025,83.01309)
  -- (207.15025,83.14310)
  -- (207.20026,83.04308)
  -- (207.26025,83.12309)
  -- (207.34026,83.03309)
  -- (207.40025,83.15309)
  -- (207.51025,82.99310)
  -- (207.60028,83.20309)
  -- (207.74026,82.94310)
  -- (207.85028,83.06309)
  -- (207.93025,82.97310)
  -- (208.04025,83.10310)
  -- (208.27028,83.05311)
  -- (208.38028,82.94310)
  -- (208.47028,83.11309)
  -- (208.69028,82.94310)
  -- (208.77026,83.23309)
  -- (208.92026,82.92309)
  -- (209.00027,84.42309)
  -- (209.14027,82.31309)
  -- (209.28026,83.37309)
  -- (209.39026,82.83310)
  -- (209.50026,83.08310)
  -- (209.65027,83.01309)
  -- (209.98027,83.08310)
  -- (210.07028,83.82310)
  -- (210.18027,82.26309)
  -- (210.29027,83.54310)
  -- (210.40025,82.85311)
  -- (210.49028,83.10310)
  -- (210.57027,82.99310)
  -- (210.68025,83.16311)
  -- (210.80028,83.04308)
  -- (210.88026,83.10310)
  -- (210.99026,83.07311)
  -- (211.08026,83.14310)
  -- (211.16028,83.02310)
  -- (211.30028,83.16311)
  -- (211.41028,83.04308)
  -- (211.50027,83.19310)
  -- (211.61028,82.99310)
  -- (211.72028,83.18310)
  -- (211.92027,82.55310)
  -- (212.06026,83.67310)
  -- (212.20026,82.89310)
  -- (212.37027,83.16311)
  -- (212.48027,83.03309)
  -- (212.57028,83.11309)
  -- (212.71027,83.04308)
  -- (212.82027,83.09310)
  -- (212.93025,83.00310)
  -- (213.04025,83.06309)
  -- (213.41028,83.05311)
  -- (213.60028,82.88310)
  -- (213.72028,83.28309)
  -- (213.86028,82.85311)
  -- (213.94028,83.09310)
  -- (214.00027,83.01309)
  -- (214.05028,83.16311)
  -- (214.19028,82.87310)
  -- (214.28027,83.10310)
  -- (214.47028,82.99310)
  -- (214.64027,83.13310)
  -- (214.76027,83.02310)
  -- (214.87027,83.12309)
  -- (215.06027,83.14310)
  -- (215.20026,83.02310)
  -- (215.57028,83.05311)
  -- (215.63028,83.73309)
  -- (215.79027,82.83310)
  -- (215.88028,83.20309)
  -- (215.99028,82.94310)
  -- (216.10028,83.16311)
  -- (216.22028,83.05311)
  -- (216.33028,83.13310)
  -- (216.44028,83.05311)
  -- (216.78027,83.23309)
  -- (217.09029,82.87310)
  -- (217.28027,83.01309)
  -- (217.53027,82.76310)
  -- (217.93027,83.08310)
  -- (218.15027,82.86309)
  -- (218.41028,83.10310)
  -- (218.66028,82.88310)
  -- (218.91028,83.05311)
  -- (219.25029,82.91310)
  -- (219.58029,83.11309)
  -- (219.87029,82.98310)
  -- (220.09029,83.11309)
  -- (220.45029,82.96311)
  -- (220.65028,83.10310)
  -- (220.85030,83.00310)
  -- (221.18028,83.08310)
  -- (221.47029,82.96311)
  -- (221.69029,83.06309)
  -- (222.31027,83.02310)
  -- (222.34029,83.28309)
  -- (222.36029,83.01309)
  -- (222.42027,83.25310)
  -- (222.45029,83.12309)
  -- (222.50029,83.16311)
  -- (222.64027,83.01309)
  -- (222.81029,83.08310)
  -- (223.07030,83.00310)
  -- (223.40027,83.08310)
  -- (223.74030,82.85311)
  -- (224.10030,82.95309)
  -- (224.30030,83.13310)
  -- (224.33028,83.48309)
  -- (224.55028,82.95309)
  -- (224.67029,82.91310)
  -- (224.89029,83.03309)
  -- (225.06029,82.99310)
  -- (225.45029,83.07311)
  -- (225.59029,83.01309)
  -- (225.96030,83.02310)
  -- (226.10030,82.93308)
  -- (226.24030,83.06309)
  -- (226.46030,82.97310)
  -- (226.69029,83.02310)
  -- (227.81029,83.01309)
  -- (227.90028,82.69311)
  -- (228.01028,82.83310)
  -- (228.15028,83.76310)
  -- (228.26028,82.46310)
  -- (228.34029,83.51309)
  -- (228.46030,82.63310)
  -- (228.60031,83.20309)
  -- (228.71030,82.91310)
  -- (228.82030,83.06309)
  -- (228.93028,82.94310)
  -- (229.16030,83.03309)
  -- (229.27030,82.96311)
  -- (229.36029,83.06309)
  -- (229.47030,82.95309)
  -- (230.25029,83.07311)
  -- (230.62029,83.02310)
  -- (230.70029,82.91310)
  -- (230.90028,83.11309)
  -- (231.07031,82.63310)
  -- (231.15028,83.38311)
  -- (231.26028,82.88310)
  -- (231.38031,83.08310)
  -- (231.55030,82.94310)
  -- (231.71030,83.21310)
  -- (231.85031,82.95309)
  -- (231.91030,83.08310)
  -- (231.97029,83.03309)
  -- (232.02030,83.10310)
  -- (232.28029,82.88310)
  -- (232.39029,83.11309)
  -- (232.47030,82.80311)
  -- (232.53029,82.95309)
  -- (232.61029,82.83310)
  -- (232.64029,82.93308)
  -- (232.70029,82.80311)
  -- (232.78030,83.97310)
  -- (232.89030,82.52310)
  -- (233.01030,83.37309)
  -- (233.12030,82.83310)
  -- (233.20029,83.12309)
  -- (233.31029,82.97310)
  -- (233.40028,83.01309)
  -- (233.85031,82.96311)
  -- (234.13030,82.98310)
  -- (234.58030,83.12309)
  -- (234.69030,82.96311)
  -- (234.80031,83.06309)
  -- (234.89030,82.99310)
  -- (235.14030,82.99310)
  -- (235.25030,83.15309)
  -- (235.34030,83.01309)
  -- (235.45030,83.18310)
  -- (235.53029,82.99310)
  -- (235.62029,83.20309)
  -- (235.73029,83.01309)
  -- (235.81030,83.10310)
  -- (236.01030,82.98310)
  -- (236.26030,83.00310)
  -- (236.37030,83.30310)
  -- (236.46031,83.17309)
  -- (236.49031,83.94311)
  -- (236.54030,81.39309)
  -- (236.63031,82.59309)
  -- (236.68030,81.86309)
  -- (236.80031,85.60311)
  -- (236.91030,81.97310)
  -- (236.96031,82.78310)
  -- (237.02030,82.19310)
  -- (237.13030,84.44310)
  -- (237.25030,82.19310)
  -- (237.36030,83.52310)
  -- (237.47030,82.77310)
  -- (237.58030,83.23309)
  -- (237.69030,82.76310)
  -- (237.81030,83.08310)
  -- (237.92030,82.98310)
  -- (238.09030,83.14310)
  -- (238.23030,82.98310)
  -- (238.37030,83.11309)
  -- (238.48030,83.02310)
  -- (238.59030,83.10310)
  -- (238.79030,83.00310)
  -- (239.10031,83.03309)
  -- (239.29030,82.91310)
  -- (239.80032,83.02310)
  -- (240.14030,82.86309)
  -- (240.39030,83.09310)
  -- (240.61030,82.81309)
  -- (240.95030,82.97310)
  -- (241.15030,82.82310)
  -- (241.71031,82.93308)
  -- (242.16032,82.89310)
  -- (242.38033,82.98310)
  -- (242.61030,82.85311)
  -- (242.83030,82.84309)
  -- (243.17030,82.94310)
  -- (243.42030,82.87310)
  -- (243.67032,82.99310)
  -- (244.24031,83.00310)
  -- (244.88031,82.78310)
  -- (245.13031,83.03309)
  -- (245.30032,82.94310)
  -- (245.58032,83.01309)
  -- (245.86030,82.95309)
  -- (245.95030,83.22310)
  -- (246.06030,82.84309)
  -- (246.17030,83.04308)
  -- (246.31030,82.90309)
  -- (246.45032,82.99310)
  -- (246.62030,82.88310)
  -- (246.79031,82.97310)
  -- (247.13031,82.99310)
  -- (247.30032,82.91310)
  -- (247.44030,82.97310)
  -- (248.00032,82.89310)
  -- (249.15031,82.95309)
  -- (249.26031,82.90309)
  -- (249.32033,82.51309)
  -- (249.40030,83.54310)
  -- (249.54031,82.49311)
  -- (249.68031,83.38311)
  -- (249.82033,82.67310)
  -- (249.94032,83.13310)
  -- (250.05032,82.80311)
  -- (250.16032,83.01309)
  -- (250.27032,82.88310)
  -- (250.44032,82.97310)
  -- (250.53032,82.90309)
  -- (250.64032,82.96311)
  -- (250.83032,82.86309)
  -- (250.92032,83.00310)
  -- (251.06032,82.89310)
  -- (251.17032,82.95309)
  -- (251.31032,82.90309)
  -- (251.42032,82.96311)
  -- (251.87032,82.94310)
  -- (251.96033,83.25310)
  -- (252.07033,82.50309)
  -- (252.21033,83.42309)
  -- (252.32033,82.65310)
  -- (252.46033,83.15309)
  -- (252.58034,82.80311)
  -- (252.66032,83.21310)
  -- (252.74033,82.67310)
  -- (252.94032,83.02310)
  -- (253.05032,82.92309)
  -- (253.14032,82.99310)
  -- (253.33032,82.87310)
  -- (253.59032,83.01309)
  -- (253.70032,82.93308)
  -- (254.29033,83.02310)
  -- (254.46033,82.72310)
  -- (254.60034,83.12309)
  -- (254.71033,82.75309)
  -- (254.85034,83.04308)
  -- (254.96034,82.83310)
  -- (255.10033,83.02310)
  -- (255.19032,82.91310)
  -- (255.33032,82.99310)
  -- (255.44032,82.93308)
  -- (255.58034,83.00310)
  -- (255.69034,82.94310)
  -- (255.83034,82.99310)
  -- (255.89034,82.89310)
  -- (255.94034,83.00310)
  -- (256.03033,82.97310)
  -- (256.14034,83.08310)
  -- (256.34033,82.87310)
  -- (256.56033,83.02310)
  -- (256.67033,82.81309)
  -- (256.73032,82.01309)
  -- (256.90033,83.52310)
  -- (257.10034,82.88310)
  -- (257.29033,83.21310)
  -- (257.40031,83.02310)
  -- (257.57033,83.09310)
  -- (257.69034,82.77310)
  -- (257.77032,82.84309)
  -- (257.94034,82.68308)
  -- (258.02032,82.81309)
  -- (258.11032,82.70309)
  -- (258.19034,85.09310)
  -- (258.30034,81.84309)
  -- (258.42032,83.73309)
  -- (258.56033,82.43308)
  -- (258.67033,83.33310)
  -- (258.81033,82.70309)
  -- (258.92033,83.20309)
  -- (259.03033,82.91310)
  -- (259.15033,83.14310)
  -- (259.20032,82.94310)
  -- (259.31032,83.08310)
  -- (259.45033,82.95309)
  -- (259.54033,83.02310)
  -- (259.71033,82.96311)
  -- (259.79033,83.22310)
  -- (259.90033,82.75309)
  -- (260.04033,83.09310)
  -- (260.16034,82.93308)
  -- (260.30034,83.04308)
  -- (260.44034,82.96311)
  -- (260.80034,83.03309)
  -- (261.05034,82.96311)
  -- (261.11032,82.97310)
  -- (261.20032,83.19310)
  -- (261.34033,82.58311)
  -- (261.39034,83.05311)
  -- (261.50034,82.86309)
  -- (261.67033,83.23309)
  -- (261.76033,83.03309)
  -- (261.87033,83.42309)
  -- (261.93033,82.54308)
  -- (261.98033,83.14310)
  -- (262.04033,82.92309)
  -- (262.09033,83.24310)
  -- (262.21034,82.97310)
  -- (262.40033,83.03309)
  -- (262.46034,82.93308)
  -- (262.57034,83.16311)
  -- (262.68033,82.94310)
  -- (262.74034,83.03309)
  -- (262.82034,82.79308)
  -- (262.94034,83.05311)
  -- (263.05034,82.83310)
  -- (263.19034,83.26309)
  -- (263.30034,82.77310)
  -- (263.41034,83.09310)
  -- (263.53033,82.92309)
  -- (263.64034,83.26309)
  -- (263.67035,83.20309)
  -- (263.69035,84.13310)
  -- (263.83034,82.38311)
  -- (263.95033,83.31309)
  -- (264.06033,82.83310)
  -- (264.20033,83.09310)
  -- (264.31033,82.93308)
  -- (264.45033,83.08310)
  -- (264.56035,82.99310)
  -- (264.70033,83.04308)
  -- (265.69035,83.04308)
  -- (265.97034,82.94310)
  -- (266.11034,83.02310)
  -- (266.42033,82.84309)
  -- (266.64034,82.91310)
  -- (266.87035,82.73309)
  -- (267.43034,82.96311)
  -- (267.79033,82.90309)
  -- (267.99034,83.00310)
  -- (268.16035,82.94310)
  -- (268.30035,82.99310)
  -- (268.58035,82.95309)
  -- (268.78035,83.04308)
  -- (269.62033,82.95309)
  -- (269.67035,83.96311)
  -- (269.76035,82.69311)
  -- (269.81035,82.81309)
  -- (269.84033,82.72310)
  -- (269.93033,83.11309)
  -- (270.01035,82.80311)
  -- (270.10036,83.00310)
  -- (270.21036,82.80311)
  -- (270.32036,82.95309)
  -- (270.40033,82.85311)
  -- (270.46036,82.96311)
  -- (270.63036,82.85311)
  -- (270.71034,82.91310)
  -- (270.80035,82.83310)
  -- (270.99036,82.89310)
  -- (271.05035,83.37309)
  -- (271.13034,82.90309)
  -- (271.25035,83.36310)
  -- (271.33034,82.96311)
  -- (271.42033,83.07311)
  -- (271.53035,82.87310)
  -- (271.61035,82.92309)
  -- (271.84035,82.90309)
  -- (271.92035,82.81309)
  -- (272.06035,82.93308)
  -- (272.12035,82.89310)
  -- (272.29034,82.95309)
  -- (272.85036,82.89310)
  -- (273.32036,83.04308)
  -- (273.41035,83.01309)
  -- (273.49036,83.13310)
  -- (273.63036,82.95309)
  -- (273.69035,83.07311)
  -- (273.75035,82.95309)
  -- (273.80037,83.02310)
  -- (273.94035,82.98310)
  -- (274.00037,83.06309)
  -- (274.36035,83.04308)
  -- (274.50035,83.12309)
  -- (274.62035,82.88310)
  -- (274.67035,83.09310)
  -- (274.73035,82.96311)
  -- (274.76035,83.06309)
  -- (274.81035,82.97310)
  -- (274.95035,83.06309)
  -- (275.46036,82.88310)
  -- (276.08035,83.11309)
  -- (276.41035,83.01309)
  -- (276.55035,82.79308)
  -- (276.92035,82.57310)
  -- (277.28035,82.66310)
  -- (277.59035,82.87310)
  -- (278.04034,82.83310)
  -- (278.29036,82.74310)
  -- (278.86035,82.72310)
  -- (279.50037,83.04308)
  -- (280.09036,82.96311)
  -- (280.43036,82.84309)
  -- (280.65036,82.94310)
  -- (280.96037,82.85311)
  -- (281.50037,83.00310)
  -- (281.92036,82.84309)
  -- (282.23036,82.95309)
  -- (282.37036,82.94310)
  -- (282.45036,83.05311)
  -- (282.67036,83.09310)
  -- (282.90036,83.27311)
  -- (282.96037,83.20309)
  -- (283.01036,83.22310)
  -- (283.32037,82.82310)
  -- (283.69037,82.85311)
  -- (283.91035,82.77310)
  -- (284.30037,82.85311)
  -- (284.53036,82.79308)
  -- (284.84036,82.83310)
  -- (285.00038,82.79308)
  -- (285.20036,82.88310)
  -- (285.29037,83.07311)
  -- (285.45036,82.76310)
  -- (285.82037,82.72310)
  -- (286.32037,82.86309)
  -- (287.11037,82.80311)
  -- (287.28036,82.67310)
  -- (287.59036,82.71310)
  -- (287.73036,82.66310)
  -- (287.95036,82.75309)
  -- (288.49039,82.70309)
  -- (288.77037,82.79308)
  -- (289.33037,82.76310)
  -- (289.58038,82.82310)
  -- (290.03038,82.67310)
  -- (290.14038,82.72310)
  -- (290.28036,82.68308)
  -- (290.51036,82.76310)
  -- (291.52039,82.83310)
  -- (292.11037,82.74310)
  -- (292.30038,82.80311)
  -- (292.53036,82.73309)
  -- (292.59038,82.81309)
  -- (292.78038,82.79308)
  -- (293.12038,82.61309)
  -- (293.54037,82.75309)
  -- (293.88039,82.73309)
  -- (294.44038,82.85311)
  -- (294.80038,82.77310)
  -- (295.11037,82.61309)
  -- (295.34038,82.63310)
  -- (295.70038,82.53309)
  -- (296.60040,82.63310)
  -- (296.85039,82.73309)
  -- (297.02039,82.67310)
  -- (297.13039,82.70309)
  -- (297.39038,82.94310)
  -- (297.84038,82.98310)
  -- (298.34038,82.83310)
  -- (298.65038,82.99310)
  -- (299.30038,83.07311)
  -- (299.44038,82.97310)
  -- (299.49040,83.01309)
  -- (299.80040,82.89310)
  -- (300.36040,83.09310)
  -- (300.98040,82.91310)
  -- (301.35039,82.69311)
  -- (301.60040,82.75309)
  -- (302.86038,82.53309)
  -- (303.26038,82.53309)
  -- (303.76039,82.89310)
  -- (304.32040,83.03309)
  -- (305.78040,82.85311)
  -- (306.91040,82.90309)
  -- (307.13040,82.97310)
  -- (307.38040,82.91310)
  -- (308.93039,82.91310)
  -- (309.07040,82.98310)
  -- (309.12039,83.89310)
  -- (309.26039,82.58311)
  -- (309.32040,82.73309)
  -- (309.46040,82.69311)
  -- (309.63040,83.40309)
  -- (309.85040,82.83310)
  -- (310.05040,83.11309)
  -- (310.36041,83.25310)
  -- (310.61040,83.16311)
  -- (310.84040,82.98310)
  -- (311.57040,82.92309)
  -- (312.77040,82.41310)
  -- (313.45041,82.65310)
  -- (314.32042,82.85311)
  -- (314.79040,82.73309)
  -- (315.67041,83.01309)
  -- (316.11040,82.94310)
  -- (316.42040,82.98310)
  -- (316.79040,83.12309)
  -- (318.02042,83.01309)
  -- (318.39041,83.09310)
  -- (318.70041,83.05311)
  -- (320.49043,82.55310)
  -- (320.72041,82.55310)
  -- (321.11041,82.73309)
  -- (321.45041,82.62309)
  -- (321.84041,82.78310)
  -- (322.15040,82.83310)
  -- (322.43040,82.78310)
  -- (322.85043,82.83310)
  -- (323.22041,82.95309)
  -- (324.23042,83.02310)
  -- (324.54042,82.86309)
  -- (325.72043,82.95309)
  -- (326.48042,82.78310)
  -- (326.98042,82.89310)
  -- (327.09042,83.97310)
  -- (327.21043,82.59309)
  -- (327.29042,82.75309)
  -- (327.40040,82.66310)
  -- (327.51040,82.66310)
  -- (327.63043,82.77310)
  -- (327.74043,83.44310)
  -- (327.91042,82.51309)
  -- (328.10043,83.12309)
  -- (328.30043,82.76310)
  -- (328.64043,82.99310)
  -- (328.78043,82.89310)
  -- (329.06042,83.01309)
  -- (329.11041,82.96311)
  -- (329.17043,83.10310)
  -- (329.28043,82.86309)
  -- (329.40040,82.95309)
  -- (329.56042,82.90309)
  -- (329.73042,82.70309)
  -- (330.07043,82.51309)
  -- (330.32043,82.59309)
  -- (330.38043,82.70309)
  -- (330.41043,82.66310)
  -- (330.55043,82.91310)
  -- (330.60045,82.89310)
  -- (330.80045,83.00310)
  -- (330.94043,82.98310)
  -- (331.05043,84.14310)
  -- (331.16043,82.57310)
  -- (331.22043,82.69311)
  -- (331.36043,82.56310)
  -- (331.42043,82.65310)
  -- (331.44043,82.59309)
  -- (331.50043,82.66310)
  -- (331.53043,82.60311)
  -- (331.59042,82.65310)
  -- (331.64043,82.61309)
  -- (331.87042,82.80311)
  -- (332.01042,83.78310)
  -- (332.15042,82.63310)
  -- (332.20042,82.82310)
  -- (332.43042,82.90309)
  -- (332.48042,82.84309)
  -- (332.54042,82.89310)
  -- (332.79042,82.81309)
  -- (333.19043,82.94310)
  -- (333.38045,83.14310)
  -- (333.47044,83.04308)
  -- (333.61043,83.09310)
  -- (333.80045,82.99310)
  -- (334.17043,82.69311)
  -- (334.76044,82.82310)
  -- (334.93042,82.79308)
  -- (335.35043,82.27311)
  -- (335.49045,82.34309)
  -- (335.74045,82.65310)
  -- (335.80045,82.83310)
  -- (335.91043,82.81309)
  -- (335.97043,82.99310)
  -- (336.02043,82.97310)
  -- (336.13043,83.09310)
  -- (336.36044,82.96311)
  -- (336.41045,83.00310)
  -- (336.47044,82.94310)
  -- (336.55043,82.96311)
  -- (336.67044,84.00310)
  -- (336.81044,82.55310)
  -- (336.84042,82.69311)
  -- (336.89044,82.54308)
  -- (336.92044,82.61309)
  -- (337.00044,82.49311)
  -- (337.06042,82.59309)
  -- (337.09044,82.52310)
  -- (337.14044,82.59309)
  -- (337.20042,82.50309)
  -- (337.31042,82.90309)
  -- (337.40042,83.69311)
  -- (337.57043,82.39309)
  -- (337.62042,82.56310)
  -- (337.65044,82.52310)
  -- (337.82043,82.79308)
  -- (337.93042,83.26309)
  -- (338.10045,82.65310)
  -- (338.21045,82.71310)
  -- (338.27045,82.68308)
  -- (338.46045,83.17309)
  -- (338.66045,82.67310)
  -- (338.86044,83.00310)
  -- (339.08044,82.75309)
  -- (339.28044,82.87310)
  -- (339.45044,82.75309)
  -- (339.62042,82.81309)
  -- (339.81044,82.75309)
  -- (340.01044,82.81309)
  -- (340.15044,82.73309)
  -- (340.54044,82.80311)
  -- (341.61044,82.79308)
  -- (341.75044,82.85311)
  -- (342.45044,82.79308)
  -- (345.23044,82.87310)
  -- (345.82045,82.77310)
  -- (346.02045,82.81309)
  -- (346.35045,82.62309)
  -- (346.72046,82.62309)
  -- (347.22044,82.64309)
  -- (347.50046,82.80311)
  -- (347.95044,82.79308)
  -- (348.21046,82.93308)
  -- (348.49046,82.72310)
  -- (348.71045,82.97310)
  -- (348.85046,82.71310)
  -- (348.94046,82.71310)
  -- (349.22044,82.95309)
  -- (349.36046,82.93308)
  -- (349.72046,82.68308)
  -- (350.17046,82.98310)
  -- (350.45045,82.67310)
  -- (350.79045,83.00310)
  -- (351.01045,82.70309)
  -- (351.21046,82.92309)
  -- (351.38046,82.71310)
  -- (351.69046,82.84309)
  -- (351.77046,82.72310)
  -- (351.91045,82.87310)
  -- (352.00046,82.88310)
  -- (352.05046,82.76310)
  -- (352.22046,82.91310)
  -- (352.28046,82.85311)
  -- (352.33046,82.91310)
  -- (352.39046,82.85311)
  -- (352.50046,82.86309)
  -- (352.59045,82.79308)
  -- (353.06046,82.89310)
  -- (353.23045,82.78310)
  -- (353.43045,82.95309)
  -- (353.57047,82.79308)
  -- (353.74046,82.94310)
  -- (353.91046,82.84309)
  -- (354.02046,82.91310)
  -- (354.16046,82.83310)
  -- (354.30046,82.91310)
  -- (354.47046,82.77310)
  -- (354.64046,82.87310)
  -- (354.78047,82.75309)
  -- (355.03046,82.81309)
  -- (355.17046,82.74310)
  -- (355.39046,82.85311)
  -- (355.93045,82.96311)
  -- (356.21046,82.89310)
  -- (356.71046,83.06309)
  -- (357.42046,82.68308)
  -- (358.23047,82.59309)
  -- (358.54047,82.42309)
  -- (358.99046,82.38311)
  -- (359.21048,82.30310)
  -- (359.97046,82.73309)
  -- (360.22046,82.67310)
  -- (360.45047,82.76310)
  -- (360.62045,82.74310)
  -- (361.07048,82.96311)
  -- (361.54047,82.99310)
  -- (362.13046,82.86309)
  -- (363.20045,82.95309)
  -- (363.62047,82.83310)
  -- (364.38048,82.89310)
  -- (364.83047,82.66310)
  -- (365.22047,82.56310)
  -- (365.61047,82.62309)
  -- (366.37047,82.49311)
  -- (367.02048,82.54308)
  -- (367.52048,82.44310)
  -- (368.31047,82.43308)
  -- (369.80049,82.11309)
  -- (370.11047,82.17309)
  -- (370.87048,82.08310)
  -- (370.95047,82.15309)
  -- (371.09048,82.05310)
  -- (371.15047,82.10310)
  -- (371.23048,81.99310)
  -- (371.79048,81.93308)
  -- (372.55048,82.01309)
  -- (373.20047,81.79308)
  -- (373.34048,81.85310)
  -- (373.56049,81.77310)
  -- (373.84048,81.82310)
  -- (374.12048,81.72310)
  -- (374.35050,81.80311)
  -- (374.40047,81.92309)
  -- (374.43048,81.87310)
  -- (374.49050,82.01309)
  -- (374.66049,81.65309)
  -- (374.71048,81.78310)
  -- (374.77050,81.63310)
  -- (374.82050,81.69311)
  -- (374.94049,81.60311)
  -- (375.13050,81.79308)
  -- (375.19049,81.77310)
  -- (375.25049,81.94310)
  -- (375.30049,81.86309)
  -- (375.36049,81.94310)
  -- (375.47049,81.70309)
  -- (375.61049,81.62309)
  -- (375.78049,81.63310)
  -- (375.92049,81.77310)
  -- (376.03049,81.64309)
  -- (376.17049,81.73309)
  -- (376.31049,81.65309)
  -- (376.62048,81.71310)
  -- (376.93048,81.68308)
  -- (376.99050,81.74310)
  -- (377.18050,81.68308)
  -- (377.30049,81.75309)
  -- (377.44049,81.63310)
  -- (377.74050,81.71310)
  -- (377.86049,81.59309)
  -- (377.91049,81.63310)
  -- (377.97049,81.58311)
  -- (378.00050,81.63310)
  -- (378.14049,81.53309)
  -- (378.28049,81.81309)
  -- (378.39049,81.23309)
  -- (378.50049,81.84309)
  -- (378.64049,81.55310)
  -- (378.76050,81.48309)
  -- (379.06049,81.64309)
  -- (379.12048,81.59309)
  -- (379.26048,81.79308)
  -- (379.40048,80.43308)
  -- (379.60051,82.05310)
  -- (379.82050,81.24310)
  -- (379.96051,81.49311)
  -- (379.99050,81.68308)
  -- (380.10050,81.72310)
  -- (380.24050,81.26309)
  -- (380.44049,81.74310)
  -- (380.66049,81.35310)
  -- (380.86049,81.65309)
  -- (381.03050,81.41310)
  -- (381.37048,81.57310)
  -- (381.51048,81.42309)
  -- (381.76050,81.62309)
  -- (381.98050,81.40309)
  -- (382.15048,81.62309)
  -- (382.38051,81.41310)
  -- (382.60051,81.60311)
  -- (382.85051,81.45309)
  -- (383.02050,81.54308)
  -- (383.44049,81.54308)
  -- (383.67050,81.46310)
  -- (383.95049,81.54308)
  -- (384.12050,81.48309)
  -- (384.37050,81.54308)
  -- (384.62048,81.47311)
  -- (384.85051,81.54308)
  -- (385.07051,81.47311)
  -- (386.14050,81.52310)
  -- (386.42050,81.48309)
  -- (386.64050,81.54308)
  -- (386.87050,81.48309)
  -- (387.09050,81.54308)
  -- (387.26050,81.48309)
  -- (388.95050,81.51309);
% Reference trace 25
\path[draw={rgb,1:red,0.898;green,0.502;blue,0.278},line width=0.32877bp] (113.26013,81.50309)
  -- (113.54013,81.59309)
  -- (113.87013,81.51309)
  -- (114.13014,81.59309)
  -- (114.35014,81.50309)
  -- (114.66014,81.58311)
  -- (114.91014,81.50309)
  -- (115.19014,81.61309)
  -- (115.47014,81.51309)
  -- (115.75014,81.59309)
  -- (116.06013,81.51309)
  -- (116.40013,81.60311)
  -- (116.51013,81.48309)
  -- (116.85016,81.62309)
  -- (117.19014,81.47311)
  -- (117.41014,81.62309)
  -- (117.75014,81.47311)
  -- (118.03015,81.63310)
  -- (118.28014,81.47311)
  -- (118.59013,81.63310)
  -- (118.87015,81.47311)
  -- (119.18015,81.62309)
  -- (119.43015,81.48309)
  -- (119.71014,81.62309)
  -- (119.80016,81.50309)
  -- (119.91014,81.57310)
  -- (119.99014,81.49311)
  -- (120.16016,81.59309)
  -- (120.36015,81.58311)
  -- (120.58015,81.48309)
  -- (120.75014,81.65309)
  -- (121.06013,81.48309)
  -- (121.31013,81.59309)
  -- (121.59015,81.52310)
  -- (121.88016,81.59309)
  -- (122.75015,81.49311)
  -- (123.25015,81.59309)
  -- (123.28015,81.52310)
  -- (123.53015,81.62309)
  -- (123.73015,81.55310)
  -- (124.23015,81.66310)
  -- (124.71016,81.67310)
  -- (125.27016,81.65309)
  -- (125.58015,81.49311)
  -- (125.86015,81.55310)
  -- (125.97015,81.51309)
  -- (126.14015,81.60311)
  -- (126.20015,81.55310)
  -- (126.26015,81.63310)
  -- (126.48015,81.67310)
  -- (126.54015,81.75309)
  -- (126.59015,81.72310)
  -- (126.79015,81.85310)
  -- (126.96016,81.76309)
  -- (127.18016,81.81309)
  -- (127.46016,81.67310)
  -- (127.69017,81.79308)
  -- (128.42015,81.48309)
  -- (128.47017,81.57310)
  -- (128.50015,81.42309)
  -- (128.61015,81.53309)
  -- (128.64015,81.47311)
  -- (128.70015,81.53309)
  -- (129.57016,81.67310)
  -- (130.07018,81.66310)
  -- (130.38017,81.74310)
  -- (130.80017,81.71310)
  -- (130.83017,81.65309)
  -- (130.89017,81.84309)
  -- (130.94017,81.64309)
  -- (131.00017,81.75309)
  -- (131.03017,81.68308)
  -- (131.08015,81.74310)
  -- (131.11015,81.68308)
  -- (131.20015,81.72310)
  -- (131.34016,81.62309)
  -- (131.53015,81.64309)
  -- (131.56017,81.57310)
  -- (131.67017,81.64309)
  -- (131.70016,81.57310)
  -- (131.79016,81.59309)
  -- (131.81017,81.78310)
  -- (131.84015,81.31309)
  -- (131.90016,81.92309)
  -- (131.96017,81.53309)
  -- (131.98016,81.76309)
  -- (132.07018,81.59309)
  -- (132.10017,81.70309)
  -- (132.29016,81.63310)
  -- (132.71016,81.66310)
  -- (133.05017,81.60311)
  -- (133.50017,81.36309)
  -- (133.86017,81.26309)
  -- (134.09016,81.09310)
  -- (134.51015,80.92309)
  -- (135.72017,80.71310)
  -- (136.11017,80.72310)
  -- (136.53017,80.86309)
  -- (137.96017,80.56309)
  -- (138.64017,80.56309)
  -- (139.84016,80.31309)
  -- (140.49019,80.02310)
  -- (141.22017,80.31309)
  -- (141.61017,80.34309)
  -- (142.40016,80.12309)
  -- (143.50018,80.29310)
  -- (143.92018,80.26309)
  -- (144.31017,80.06309)
  -- (144.62016,80.02310)
  -- (145.57019,80.11309)
  -- (146.39018,79.93308)
  -- (147.09018,80.15309)
  -- (147.34018,80.16310)
  -- (148.16019,79.88310)
  -- (148.52019,79.89309)
  -- (148.91019,80.12309)
  -- (150.94019,79.95309)
  -- (151.47020,79.99310)
  -- (151.55019,80.06309)
  -- (151.58020,79.96310)
  -- (151.61018,80.07310)
  -- (151.67020,80.02310)
  -- (151.75018,80.09309)
  -- (151.81018,80.03309)
  -- (151.86018,80.08310)
  -- (151.89020,80.01309)
  -- (151.92018,80.11309)
  -- (151.95018,79.96310)
  -- (152.03020,80.14309)
  -- (152.06018,79.97310)
  -- (152.09020,80.04308)
  -- (152.14020,79.97310)
  -- (152.23020,80.07310)
  -- (152.26018,80.00310)
  -- (152.37018,80.07310)
  -- (152.56020,80.00310)
  -- (153.43019,80.05310)
  -- (153.91019,79.90309)
  -- (153.97018,79.94310)
  -- (154.22018,79.79308)
  -- (154.33018,79.79308)
  -- (154.81020,79.94310)
  -- (155.03020,79.87309)
  -- (155.20018,79.96310)
  -- (155.48020,79.96310)
  -- (156.33018,80.20309)
  -- (156.35019,80.16310)
  -- (156.89020,80.37309)
  -- (157.45020,80.47310)
  -- (157.90019,80.76309)
  -- (158.35020,80.85310)
  -- (158.54019,80.83310)
  -- (159.27020,80.30310)
  -- (159.30020,80.36309)
  -- (159.39020,80.26309)
  -- (159.64020,80.15309)
  -- (159.92020,80.13310)
  -- (159.95020,80.17309)
  -- (159.98020,80.10310)
  -- (160.09021,80.24310)
  -- (160.12020,80.16310)
  -- (160.29020,80.26309)
  -- (160.31020,80.34309)
  -- (160.34020,80.28309)
  -- (160.43019,80.39309)
  -- (160.45020,80.31309)
  -- (160.54019,80.36309)
  -- (160.57020,80.44310)
  -- (160.59020,80.37309)
  -- (161.27022,80.53309)
  -- (161.58022,80.53309)
  -- (161.63020,80.57310)
  -- (161.66020,80.81309)
  -- (161.69022,80.15309)
  -- (161.75020,80.83310)
  -- (161.80022,79.66310)
  -- (161.83020,81.65309)
  -- (161.86020,80.14309)
  -- (161.89021,80.77310)
  -- (161.94020,80.39309)
  -- (161.97020,80.52310)
  -- (162.00021,80.46310)
  -- (162.05020,80.51309)
  -- (162.08020,80.41310)
  -- (162.14020,80.46310)
  -- (162.17020,80.37309)
  -- (162.22020,80.46310)
  -- (162.31020,80.36309)
  -- (162.33020,80.50309)
  -- (162.36021,80.34309)
  -- (162.45021,80.46310)
  -- (162.48020,80.32310)
  -- (162.56021,80.41310)
  -- (162.64020,80.25309)
  -- (162.67021,80.36309)
  -- (162.73020,80.20309)
  -- (162.78021,80.33310)
  -- (162.87021,80.26309)
  -- (162.92020,80.40309)
  -- (162.98021,80.29310)
  -- (163.06020,80.88310)
  -- (163.12020,80.83310)
  -- (163.18020,81.06309)
  -- (163.35020,80.44310)
  -- (163.46020,80.67309)
  -- (163.68019,80.47310)
  -- (163.79019,80.25309)
  -- (163.82020,80.31309)
  -- (163.88020,80.24310)
  -- (164.72021,81.04308)
  -- (164.78021,81.02310)
  -- (164.86020,81.17309)
  -- (164.97020,81.13310)
  -- (165.00021,81.19310)
  -- (165.48020,80.80311)
  -- (165.59020,80.77310)
  -- (165.87021,80.89310)
  -- (166.07022,80.81309)
  -- (166.43020,80.80311)
  -- (166.63022,80.90309)
  -- (167.36021,81.05310)
  -- (167.73020,81.26309)
  -- (168.20020,81.42309)
  -- (168.23021,81.38311)
  -- (168.40019,81.51309)
  -- (168.43020,81.42309)
  -- (168.54020,81.55310)
  -- (168.57022,81.51309)
  -- (168.65020,81.55310)
  -- (168.68020,81.50309)
  -- (168.71020,81.56309)
  -- (168.76021,81.49311)
  -- (168.82020,81.53309)
  -- (169.58022,81.43308)
  -- (169.89021,81.52310)
  -- (170.08022,81.47311)
  -- (170.34021,81.55310)
  -- (170.65020,81.51309)
  -- (171.66022,81.66310)
  -- (172.44022,81.95309)
  -- (172.81021,82.22310)
  -- (172.84021,82.12309)
  -- (172.92021,82.24310)
  -- (173.14021,82.32310)
  -- (173.57022,82.24310)
  -- (174.07024,81.94310)
  -- (174.44022,81.86309)
  -- (174.63022,81.87310)
  -- (174.94023,82.04308)
  -- (175.45023,82.13310)
  -- (176.32024,81.92309)
  -- (176.94023,81.92309)
  -- (177.86021,81.80311)
  -- (178.65022,81.89310)
  -- (179.41023,81.72310)
  -- (179.97023,81.83310)
  -- (180.42021,81.80311)
  -- (180.78023,81.68308)
  -- (181.29022,81.66310)
  -- (182.02023,81.79308)
  -- (182.75023,81.66310)
  -- (183.79022,81.74310)
  -- (184.77023,81.68308)
  -- (185.47025,81.75309)
  -- (186.00024,81.62309)
  -- (186.59023,81.71310)
  -- (186.82024,81.66310)
  -- (186.99023,81.74310)
  -- (187.74025,81.48309)
  -- (188.47025,81.70309)
  -- (188.73022,81.70309)
  -- (188.92024,81.57310)
  -- (188.95023,81.62309)
  -- (189.04022,81.53309)
  -- (189.18024,81.54308)
  -- (189.40022,81.59309)
  -- (189.93022,81.86309)
  -- (190.38025,81.67310)
  -- (190.55023,81.66310)
  -- (190.86024,81.68308)
  -- (191.14024,81.85310)
  -- (191.62022,81.83310)
  -- (192.18024,81.58311)
  -- (192.52025,81.59309)
  -- (193.47025,81.87310)
  -- (193.78024,81.67310)
  -- (194.40024,81.53309)
  -- (194.48024,81.21310)
  -- (194.51024,81.73309)
  -- (194.54024,81.35310)
  -- (194.57025,81.64309)
  -- (194.62024,81.50309)
  -- (194.71025,81.59309)
  -- (194.74025,81.48309)
  -- (194.76024,81.57310)
  -- (194.79024,81.50309)
  -- (195.07025,81.71310)
  -- (195.21025,81.70309)
  -- (195.61024,81.84309)
  -- (195.66025,81.78310)
  -- (195.72025,81.83310)
  -- (195.83025,81.76309)
  -- (195.94025,81.65309)
  -- (196.20024,81.67310)
  -- (196.48024,81.57310)
  -- (196.76025,81.78310)
  -- (197.09026,81.80311)
  -- (197.77025,81.72310)
  -- (198.25026,81.51309)
  -- (199.31024,81.64309)
  -- (199.37024,81.39309)
  -- (199.40024,81.70309)
  -- (199.51024,81.45309)
  -- (199.54025,81.59309)
  -- (199.68024,81.50309)
  -- (199.73024,81.58311)
  -- (199.82025,81.54308)
  -- (200.74026,81.73309)
  -- (200.94026,81.70309)
  -- (201.19026,81.75309)
  -- (201.28026,81.64309)
  -- (201.33025,81.71310)
  -- (201.42024,81.59309)
  -- (201.62024,81.63310)
  -- (201.92026,81.49311)
  -- (202.32027,81.53309)
  -- (202.35027,81.60311)
  -- (202.40024,81.42309)
  -- (202.46027,81.68308)
  -- (202.54025,81.54308)
  -- (202.57027,81.73309)
  -- (202.68025,81.54308)
  -- (202.71025,81.66310)
  -- (202.79025,81.58311)
  -- (202.82025,81.62309)
  -- (203.08026,81.56309)
  -- (204.03026,81.66310)
  -- (204.25026,81.59309)
  -- (204.54025,81.61309)
  -- (205.18025,81.40309)
  -- (205.24026,81.45309)
  -- (205.29025,81.38311)
  -- (205.38026,81.46310)
  -- (205.43025,81.38311)
  -- (205.52026,81.53309)
  -- (205.57027,81.49311)
  -- (205.66026,81.59309)
  -- (205.83026,81.53309)
  -- (205.85027,81.60311)
  -- (205.88026,81.54308)
  -- (206.11026,81.59309)
  -- (206.16026,81.53309)
  -- (206.19026,81.60311)
  -- (206.30026,81.55310)
  -- (206.33026,81.60311)
  -- (206.56026,81.51309)
  -- (206.75026,81.51309)
  -- (206.84026,81.44310)
  -- (206.92026,81.46310)
  -- (206.98027,81.38311)
  -- (207.09027,81.44310)
  -- (207.26025,81.33310)
  -- (207.34026,81.39309)
  -- (207.40025,81.31309)
  -- (207.46027,81.44310)
  -- (207.57027,81.37309)
  -- (208.27028,81.87310)
  -- (208.41026,81.90309)
  -- (208.61026,81.79308)
  -- (208.69028,81.83310)
  -- (208.75026,81.68308)
  -- (208.83026,81.80311)
  -- (208.89027,81.69311)
  -- (208.94028,81.77310)
  -- (209.03027,81.56309)
  -- (209.08026,81.72310)
  -- (209.11026,81.46310)
  -- (209.14027,81.74310)
  -- (209.17026,81.45309)
  -- (209.20026,81.60311)
  -- (209.31026,81.50309)
  -- (209.42026,81.61309)
  -- (209.53026,81.57310)
  -- (209.98027,81.76309)
  -- (210.01025,81.94310)
  -- (210.04025,81.80311)
  -- (210.09027,81.89310)
  -- (210.15025,81.84309)
  -- (210.23027,82.03309)
  -- (210.35027,81.81309)
  -- (210.38028,81.85310)
  -- (210.49028,81.75309)
  -- (210.74028,81.70309)
  -- (211.08026,81.52310)
  -- (211.16028,81.57310)
  -- (211.22026,81.47311)
  -- (211.25027,81.60311)
  -- (211.30028,81.49311)
  -- (211.33026,81.61309)
  -- (211.36028,81.53309)
  -- (211.41028,81.61309)
  -- (211.44026,81.54308)
  -- (211.53026,81.62309)
  -- (211.81027,81.69311)
  -- (211.84026,81.65309)
  -- (211.89027,81.85310)
  -- (211.95026,81.63310)
  -- (212.03027,81.80311)
  -- (212.09027,81.69311)
  -- (212.20026,81.73309)
  -- (212.26025,81.67310)
  -- (212.34027,81.76309)
  -- (212.87027,81.80311)
  -- (213.60028,81.59309)
  -- (213.74028,81.64309)
  -- (213.83028,81.54308)
  -- (214.00027,81.64309)
  -- (214.03027,81.58311)
  -- (214.22026,81.65309)
  -- (214.39027,81.60311)
  -- (214.73027,81.78310)
  -- (214.87027,81.79308)
  -- (215.01027,81.78310)
  -- (215.34027,81.56309)
  -- (215.60028,81.60311)
  -- (215.63028,81.53309)
  -- (215.68027,81.77310)
  -- (215.71027,81.58311)
  -- (215.93027,81.84309)
  -- (216.83028,81.78310)
  -- (217.17027,81.59309)
  -- (217.98029,81.74310)
  -- (218.24028,81.67310)
  -- (218.74028,81.70309)
  -- (220.48027,81.53309)
  -- (221.16030,81.70309)
  -- (221.72029,81.61309)
  -- (222.11028,81.44310)
  -- (222.28027,81.44310)
  -- (222.34029,81.54308)
  -- (222.39027,81.47311)
  -- (222.48027,81.55310)
  -- (222.53027,81.49311)
  -- (223.01028,81.64309)
  -- (223.49030,81.70309)
  -- (223.77030,81.63310)
  -- (224.13028,81.64309)
  -- (224.33028,81.55310)
  -- (224.41030,81.61309)
  -- (224.44028,81.49311)
  -- (224.47029,81.56309)
  -- (224.61029,81.47311)
  -- (224.95029,81.51309)
  -- (225.34029,81.67310)
  -- (227.11029,81.49311)
  -- (227.81029,81.57310)
  -- (228.01028,81.69311)
  -- (228.04028,81.57310)
  -- (228.09029,81.65309)
  -- (228.18028,81.56309)
  -- (228.20029,81.71310)
  -- (228.29030,81.57310)
  -- (228.32030,81.62309)
  -- (228.37029,81.56309)
  -- (228.40028,81.63310)
  -- (228.43028,81.56309)
  -- (228.49031,81.61309)
  -- (228.57030,81.54308)
  -- (228.65028,81.58311)
  -- (228.88030,81.53309)
  -- (229.72029,81.72310)
  -- (230.65030,81.56309)
  -- (231.01028,81.56309)
  -- (231.10030,81.45309)
  -- (231.12029,81.53309)
  -- (231.18030,81.43308)
  -- (231.43028,81.53309)
  -- (231.46030,81.47311)
  -- (231.55030,81.67310)
  -- (231.60031,81.53309)
  -- (231.69030,81.69311)
  -- (231.74031,81.55310)
  -- (231.85031,81.73309)
  -- (231.88030,81.46310)
  -- (231.94030,81.71310)
  -- (231.99030,81.55310)
  -- (232.08029,81.65309)
  -- (232.11029,81.55310)
  -- (232.16031,81.62309)
  -- (232.33029,81.54308)
  -- (232.44029,81.72310)
  -- (232.47030,81.61309)
  -- (232.58030,81.78310)
  -- (232.61029,81.71310)
  -- (232.67030,81.80311)
  -- (232.81029,81.69311)
  -- (232.84029,81.88310)
  -- (232.86029,81.57310)
  -- (232.89030,81.75309)
  -- (233.29030,81.53309)
  -- (233.54030,81.47311)
  -- (234.35030,81.46310)
  -- (235.20029,81.59309)
  -- (235.64029,81.78310)
  -- (235.90030,81.77310)
  -- (236.37030,81.63310)
  -- (236.46031,81.66310)
  -- (236.54030,81.31309)
  -- (236.60031,82.05310)
  -- (236.63031,81.38311)
  -- (236.66031,81.80311)
  -- (236.71030,81.43308)
  -- (236.74031,81.57310)
  -- (236.77031,81.43308)
  -- (236.82030,81.79308)
  -- (236.85031,80.94310)
  -- (236.88031,81.59309)
  -- (236.96031,81.43308)
  -- (237.02030,81.53309)
  -- (237.13030,81.35310)
  -- (237.16031,81.68308)
  -- (237.19030,81.39309)
  -- (237.22029,81.49311)
  -- (237.27031,81.42309)
  -- (237.30031,81.52310)
  -- (237.36030,81.43308)
  -- (237.55031,81.51309)
  -- (237.58030,81.46310)
  -- (237.67030,81.57310)
  -- (237.86030,81.59309)
  -- (238.56030,81.54308)
  -- (239.18030,81.70309)
  -- (239.94030,81.72310)
  -- (240.17030,81.62309)
  -- (240.36030,81.64309)
  -- (240.61030,81.54308)
  -- (241.06030,81.73309)
  -- (241.23030,81.73309)
  -- (242.02031,81.57310)
  -- (242.89032,81.72310)
  -- (243.34032,81.73309)
  -- (244.07033,81.56309)
  -- (244.57031,81.61309)
  -- (245.02031,81.74310)
  -- (245.50032,81.71310)
  -- (245.95030,81.50309)
  -- (245.98032,81.66310)
  -- (246.01031,81.47311)
  -- (246.03032,81.63310)
  -- (246.06030,81.53309)
  -- (247.52032,81.71310)
  -- (248.64032,81.52310)
  -- (249.26031,81.63310)
  -- (249.29031,81.70309)
  -- (249.32033,81.55310)
  -- (249.35033,81.61309)
  -- (249.40030,81.58311)
  -- (249.43031,81.71310)
  -- (249.46033,81.51309)
  -- (249.49033,81.65309)
  -- (249.57033,81.62309)
  -- (249.60033,81.54308)
  -- (249.71031,81.62309)
  -- (249.88033,81.56309)
  -- (250.67032,81.72310)
  -- (250.92032,81.57310)
  -- (250.95032,81.63310)
  -- (251.31032,81.51309)
  -- (251.85033,81.55310)
  -- (251.87032,81.61309)
  -- (251.93031,81.50309)
  -- (252.01031,81.60311)
  -- (252.18033,81.59309)
  -- (252.21033,81.65309)
  -- (252.24033,81.55310)
  -- (252.27034,81.71310)
  -- (252.35033,81.55310)
  -- (252.38034,81.63310)
  -- (252.49034,81.56309)
  -- (252.63033,81.60311)
  -- (252.69034,81.53309)
  -- (252.77032,81.63310)
  -- (252.83032,81.54308)
  -- (253.33032,81.64309)
  -- (253.92032,81.64309)
  -- (254.34033,81.53309)
  -- (254.37032,81.59309)
  -- (254.46033,81.52310)
  -- (254.51031,81.59309)
  -- (254.60034,81.50309)
  -- (254.68031,81.55310)
  -- (254.77032,81.49311)
  -- (255.19032,81.61309)
  -- (255.21033,81.66310)
  -- (255.24033,81.60311)
  -- (255.30032,81.64309)
  -- (255.72034,81.64309)
  -- (255.92033,81.54308)
  -- (256.14034,81.57310)
  -- (256.28032,81.53309)
  -- (256.31032,81.61309)
  -- (256.37032,81.54308)
  -- (256.39032,81.61309)
  -- (256.42032,81.54308)
  -- (256.48032,81.61309)
  -- (256.53032,81.57310)
  -- (256.59032,81.71310)
  -- (256.62032,81.63310)
  -- (256.67033,81.64309)
  -- (256.73032,81.83310)
  -- (256.76033,81.64309)
  -- (256.82033,81.83310)
  -- (256.90033,81.68308)
  -- (256.96034,81.84309)
  -- (257.01033,81.72310)
  -- (257.10034,81.81309)
  -- (257.12033,81.76309)
  -- (257.24033,81.79308)
  -- (257.35033,81.73309)
  -- (257.46033,81.53309)
  -- (257.49034,81.60311)
  -- (257.57033,81.49311)
  -- (257.99034,81.41310)
  -- (258.11032,81.46310)
  -- (258.13033,81.33310)
  -- (258.16034,81.49311)
  -- (258.19034,80.96310)
  -- (258.22032,81.66310)
  -- (258.25034,81.16310)
  -- (258.30034,81.44310)
  -- (258.33032,81.39309)
  -- (258.39034,81.45309)
  -- (258.42032,81.34309)
  -- (258.56033,81.46310)
  -- (258.64032,81.42309)
  -- (259.03033,81.77310)
  -- (259.45033,81.87310)
  -- (259.48033,81.79308)
  -- (259.59033,81.79308)
  -- (259.62032,81.72310)
  -- (259.65033,81.76309)
  -- (259.76033,81.67310)
  -- (259.79033,81.73309)
  -- (259.82033,81.58311)
  -- (259.90033,81.70309)
  -- (259.99034,81.56309)
  -- (260.07034,81.63310)
  -- (260.30034,81.58311)
  -- (261.14034,81.59309)
  -- (261.25034,81.66310)
  -- (261.31033,81.55310)
  -- (261.36034,81.67310)
  -- (261.42033,81.51309)
  -- (261.50034,81.61309)
  -- (261.56033,81.49311)
  -- (261.64034,81.69311)
  -- (261.67033,81.51309)
  -- (261.73033,81.67310)
  -- (261.81033,81.49311)
  -- (261.90033,81.76309)
  -- (261.95033,81.38311)
  -- (262.04033,81.67310)
  -- (262.12033,81.49311)
  -- (262.15033,81.69311)
  -- (262.18033,81.51309)
  -- (262.21034,81.61309)
  -- (262.23033,81.50309)
  -- (262.26033,81.63310)
  -- (262.32034,81.53309)
  -- (262.35034,81.64309)
  -- (262.40033,81.56309)
  -- (262.46034,81.64309)
  -- (262.57034,81.58311)
  -- (262.60036,81.63310)
  -- (262.71034,81.51309)
  -- (262.77034,81.57310)
  -- (263.02034,81.45309)
  -- (263.10034,81.49311)
  -- (263.19034,81.40309)
  -- (263.24034,81.45309)
  -- (263.50034,81.47311)
  -- (263.67035,81.59309)
  -- (263.69035,81.16310)
  -- (263.72034,81.72310)
  -- (263.75034,81.38311)
  -- (263.78035,81.69311)
  -- (263.83034,81.55310)
  -- (264.09035,81.80311)
  -- (264.34033,81.89310)
  -- (264.79033,81.87310)
  -- (265.35034,81.67310)
  -- (265.63034,81.64309)
  -- (266.31033,81.76309)
  -- (267.12035,81.77310)
  -- (267.48033,81.87310)
  -- (268.05035,81.89310)
  -- (268.35034,81.81309)
  -- (268.64034,81.82310)
  -- (269.67035,81.98310)
  -- (269.70035,81.84309)
  -- (269.73033,82.14309)
  -- (269.79034,81.92309)
  -- (269.87035,82.11309)
  -- (269.93033,81.99310)
  -- (270.01035,82.09310)
  -- (270.63036,82.29310)
  -- (270.99036,82.29310)
  -- (271.02034,82.23309)
  -- (271.11034,82.39309)
  -- (271.16035,82.36310)
  -- (271.33034,82.52310)
  -- (271.58035,82.39309)
  -- (271.81035,82.42309)
  -- (272.34035,82.33310)
  -- (272.82036,82.16311)
  -- (273.10036,82.26309)
  -- (273.44035,82.20309)
  -- (273.46036,82.15309)
  -- (273.49036,82.37309)
  -- (273.52036,82.16311)
  -- (273.61035,82.24310)
  -- (273.69035,82.20309)
  -- (273.72035,82.24310)
  -- (273.75035,82.19310)
  -- (273.83035,82.24310)
  -- (274.03035,82.21310)
  -- (274.11035,82.29310)
  -- (274.39035,82.19310)
  -- (274.50035,82.25309)
  -- (274.56035,82.08310)
  -- (274.59035,82.24310)
  -- (274.62035,82.10310)
  -- (274.73035,82.18310)
  -- (274.76035,82.10310)
  -- (274.81035,82.14309)
  -- (274.84035,82.09310)
  -- (275.35036,82.25309)
  -- (275.63036,82.26309)
  -- (276.13036,82.47311)
  -- (276.41035,82.48309)
  -- (276.86035,82.05310)
  -- (277.14037,81.89310)
  -- (277.45036,81.86309)
  -- (277.90034,81.62309)
  -- (278.38037,81.52310)
  -- (279.28035,81.84309)
  -- (280.18036,81.66310)
  -- (281.44035,81.72310)
  -- (281.97037,81.59309)
  -- (282.56036,81.67310)
  -- (282.73035,81.60311)
  -- (282.79036,81.66310)
  -- (282.81036,81.57310)
  -- (282.90036,81.64309)
  -- (282.98036,81.58311)
  -- (283.24037,81.58311)
  -- (283.74037,81.74310)
  -- (284.67036,81.87310)
  -- (285.20036,81.84309)
  -- (285.29037,81.70309)
  -- (285.37036,81.76309)
  -- (285.68036,81.67310)
  -- (286.80038,82.00310)
  -- (287.53036,82.07311)
  -- (288.51036,81.98310)
  -- (289.22037,81.99310)
  -- (289.67038,81.87310)
  -- (290.54037,81.97310)
  -- (292.08038,81.89310)
  -- (292.45038,81.80311)
  -- (293.32039,82.15309)
  -- (294.13037,81.85310)
  -- (294.52039,81.91310)
  -- (295.39038,81.81309)
  -- (295.93037,81.82310)
  -- (298.68037,81.40309)
  -- (299.35039,81.36309)
  -- (299.46039,81.25309)
  -- (299.52039,81.37309)
  -- (299.58040,81.27310)
  -- (299.60040,81.31309)
  -- (299.69040,81.23309)
  -- (299.75038,81.28309)
  -- (299.80040,81.22310)
  -- (299.94040,81.33310)
  -- (300.03040,81.22310)
  -- (300.05040,81.29310)
  -- (300.36040,81.28309)
  -- (301.65039,81.67310)
  -- (302.30040,81.76309)
  -- (303.73038,81.71310)
  -- (304.97040,81.50309)
  -- (308.98041,81.50309)
  -- (309.21040,81.34309)
  -- (309.32040,81.49311)
  -- (309.40039,81.41310)
  -- (309.43039,81.50309)
  -- (309.49042,81.43308)
  -- (309.60042,81.55310)
  -- (309.71040,81.41310)
  -- (310.25041,81.67310)
  -- (310.92040,81.45309)
  -- (311.87040,81.45309)
  -- (312.75040,81.37309)
  -- (313.19040,81.42309)
  -- (314.06040,81.79308)
  -- (314.77040,81.65309)
  -- (315.69041,81.64309)
  -- (316.51039,81.43308)
  -- (317.94041,81.47311)
  -- (318.00041,81.38311)
  -- (318.11040,81.45309)
  -- (318.16042,81.37309)
  -- (318.19041,81.45309)
  -- (318.22041,81.37309)
  -- (318.33041,81.45309)
  -- (318.36041,81.40309)
  -- (318.87040,81.44310)
  -- (320.13042,81.82310)
  -- (320.38043,81.79308)
  -- (320.75041,81.63310)
  -- (321.14041,81.61309)
  -- (321.84041,81.69311)
  -- (322.46042,81.51309)
  -- (324.12042,81.48309)
  -- (324.40040,81.39309)
  -- (325.30043,81.46310)
  -- (326.14043,81.40309)
  -- (327.01042,81.51309)
  -- (327.09042,81.40309)
  -- (327.15040,81.46310)
  -- (327.21043,81.42309)
  -- (327.26042,81.48309)
  -- (327.37042,81.45309)
  -- (327.40040,81.52310)
  -- (327.57043,81.51309)
  -- (327.68042,81.58311)
  -- (327.71042,81.53309)
  -- (327.79042,81.57310)
  -- (327.88043,81.50309)
  -- (327.94043,81.53309)
  -- (327.96043,81.44310)
  -- (327.99043,81.64309)
  -- (328.02042,81.51309)
  -- (328.58043,81.50309)
  -- (328.64043,81.45309)
  -- (328.67043,81.50309)
  -- (329.03043,81.42309)
  -- (329.06042,81.47311)
  -- (329.20041,81.38311)
  -- (329.25043,81.48309)
  -- (329.37042,81.38311)
  -- (329.45042,81.49311)
  -- (329.48042,81.44310)
  -- (329.59042,81.50309)
  -- (330.04042,81.51309)
  -- (330.41043,81.75309)
  -- (330.43042,81.69311)
  -- (330.52043,81.83310)
  -- (330.83043,81.92309)
  -- (331.00044,81.80311)
  -- (331.05043,81.85310)
  -- (331.39043,81.47311)
  -- (331.44043,81.50309)
  -- (331.70042,81.37309)
  -- (331.84042,81.50309)
  -- (331.87042,81.37309)
  -- (331.92043,81.49311)
  -- (332.01042,81.32310)
  -- (332.17043,81.48309)
  -- (332.20042,81.40309)
  -- (332.26042,81.47311)
  -- (332.29044,81.43308)
  -- (332.57043,81.68308)
  -- (332.85043,81.81309)
  -- (333.27045,81.66310)
  -- (333.41043,81.58311)
  -- (333.47044,81.45309)
  -- (333.49045,81.51309)
  -- (333.72043,81.34309)
  -- (334.00044,81.27310)
  -- (334.03043,81.37309)
  -- (334.08043,81.33310)
  -- (334.79042,81.56309)
  -- (335.49045,81.54308)
  -- (335.54044,81.60311)
  -- (335.60045,81.54308)
  -- (335.82043,81.65309)
  -- (336.16045,81.69311)
  -- (336.41045,81.63310)
  -- (336.44043,81.68308)
  -- (336.50044,81.56309)
  -- (336.55043,81.59309)
  -- (336.67044,81.28309)
  -- (336.75043,81.29310)
  -- (336.78044,81.37309)
  -- (336.81044,81.28309)
  -- (336.86043,81.41310)
  -- (336.89044,81.29310)
  -- (336.95042,81.44310)
  -- (336.98044,81.27310)
  -- (337.00044,81.36309)
  -- (337.06042,81.29310)
  -- (337.09044,81.40309)
  -- (337.14044,81.30310)
  -- (337.28044,81.36309)
  -- (337.37042,81.23309)
  -- (337.59044,81.43308)
  -- (337.65044,81.40309)
  -- (337.76044,81.48309)
  -- (337.90044,81.41310)
  -- (338.27045,81.62309)
  -- (338.41045,81.53309)
  -- (338.69044,81.58311)
  -- (338.97044,81.47311)
  -- (340.54044,81.60311)
  -- (341.24045,81.46310)
  -- (342.06044,81.56309)
  -- (343.49046,81.54308)
  -- (343.85045,81.60311)
  -- (345.20044,81.47311)
  -- (346.72046,81.67310)
  -- (347.25046,81.68308)
  -- (348.18045,81.46310)
  -- (348.66045,81.23309)
  -- (348.68045,81.33310)
  -- (348.74046,81.28309)
  -- (349.36046,81.54308)
  -- (349.69046,81.47311)
  -- (350.42044,81.55310)
  -- (350.45045,81.62309)
  -- (350.48045,81.57310)
  -- (350.76045,81.62309)
  -- (351.13045,81.56309)
  -- (351.69046,81.43308)
  -- (351.72046,81.48309)
  -- (351.91045,81.45309)
  -- (352.17046,81.58311)
  -- (352.53046,81.61309)
  -- (352.64046,81.69311)
  -- (352.67046,81.57310)
  -- (353.18045,81.57310)
  -- (353.20045,81.46310)
  -- (353.26045,81.57310)
  -- (353.43045,81.46310)
  -- (353.46046,81.51309)
  -- (353.49046,81.45309)
  -- (353.51045,81.53309)
  -- (353.54045,81.42309)
  -- (355.11046,81.62309)
  -- (356.83046,81.55310)
  -- (357.61046,81.46310)
  -- (358.82047,81.63310)
  -- (359.63048,81.85310)
  -- (360.11046,81.86309)
  -- (360.79047,81.68308)
  -- (361.63048,81.35310)
  -- (362.39047,81.30310)
  -- (362.50047,81.34309)
  -- (362.55048,81.23309)
  -- (362.64047,81.34309)
  -- (362.67047,81.28309)
  -- (362.84047,81.34309)
  -- (362.89047,81.30310)
  -- (363.93047,81.46310)
  -- (365.42047,81.43308)
  -- (365.64047,81.51309)
  -- (366.26047,81.54308)
  -- (366.77048,81.56309)
  -- (367.22047,81.51309)
  -- (368.03047,81.58311)
  -- (369.32050,81.57310)
  -- (370.64047,81.69311)
  -- (371.06047,81.62309)
  -- (371.68048,81.67310)
  -- (372.63050,81.59309)
  -- (373.76048,81.69311)
  -- (374.37048,81.64309)
  -- (374.46050,81.77310)
  -- (374.57050,81.71310)
  -- (374.60050,81.76309)
  -- (374.66049,81.62309)
  -- (374.71048,81.72310)
  -- (374.74050,81.65309)
  -- (375.08049,81.71310)
  -- (375.13050,81.77310)
  -- (375.19049,81.73309)
  -- (375.27050,81.82310)
  -- (375.33049,81.74310)
  -- (375.41049,81.78310)
  -- (375.64049,81.69311)
  -- (375.72049,81.75309)
  -- (375.84048,81.73309)
  -- (375.92049,81.81309)
  -- (376.09048,81.74310)
  -- (376.23048,81.80311)
  -- (377.01048,81.77310)
  -- (377.04048,81.81309)
  -- (377.18050,81.74310)
  -- (377.30049,81.81309)
  -- (377.44049,81.71310)
  -- (377.49051,81.77310)
  -- (377.63050,81.71310)
  -- (377.74050,81.77310)
  -- (378.11049,81.70309)
  -- (378.31049,80.62309)
  -- (378.39049,80.91310)
  -- (378.42049,80.82310)
  -- (378.45049,80.86309)
  -- (378.61049,81.77310)
  -- (378.67050,81.69311)
  -- (378.98050,81.88310)
  -- (379.09050,81.80311)
  -- (379.15048,81.86309)
  -- (379.29050,81.57310)
  -- (379.37048,80.84309)
  -- (379.40048,80.96310)
  -- (379.46050,80.75309)
  -- (379.77050,82.08310)
  -- (379.93048,81.71310)
  -- (379.96051,81.75309)
  -- (380.02050,81.37309)
  -- (380.05050,81.59309)
  -- (380.19049,81.08310)
  -- (380.30049,81.50309)
  -- (380.50049,81.87310)
  -- (380.80050,81.29310)
  -- (381.17049,81.75309)
  -- (381.51048,81.33310)
  -- (381.84048,81.75309)
  -- (382.21051,81.34309)
  -- (382.55049,81.73309)
  -- (382.85051,81.38311)
  -- (383.16050,81.66310)
  -- (383.25050,81.67310)
  -- (383.61050,81.44310)
  -- (384.01050,81.62309)
  -- (384.37050,81.44310)
  -- (384.68050,81.64309)
  -- (384.76050,81.64309)
  -- (385.02050,81.43308)
  -- (385.41050,81.63310)
  -- (385.77051,81.47311)
  -- (386.06050,81.59309)
  -- (386.59050,81.50309)
  -- (386.90050,81.60311)
  -- (387.23050,81.47311)
  -- (387.60052,81.61309)
  -- (387.91050,81.48309)
  -- (388.19050,81.59309)
  -- (388.61050,81.52310)
  -- (388.95050,81.56309);

